The $q_{\mathrm{T}}$ and $\Delta\phi_{t\bar{t}}$ spectra in top-antitop hadroproduction at NNLL+NNLO: the interplay of soft-collinear resummation and Coulomb singularities

In this paper, we present the resummation-improved differential transverse momentum and azimuthal decorrelation cross sections, $d\sigma_{t\bar{t}}/dq_{\mathrm{T}}$ and $d\sigma_{t\bar{t}}/d\Delta\phi_{t\bar{t}}$, in top-antitop pair production at the LHC. Our calculation is based on the observation that both cross sections are dominated by topologies where the top-quark pair is well separated, expressed in their relative velocity $\beta_{t\bar{t}}\sim\mathcal{O}(1)$, at colliding energies of $\sqrt{s}=13\,\text{TeV}$ or higher. Therefore, the asymptotic behaviour in the limits $q_{\mathrm{T}}\to0$ and $\Delta\phi_{t\bar{t}}\to0$ can mostly be captured by the soft and collinear resummation in the HQET$+$SCET framework. Nevertheless, starting at NNLL, Coulomb singularities emerge in the threshold regime, $\beta_{t\bar{t}}\to0$, in both the hard sector and its evolution kernels, leading to unphysical results upon integration over the entire $\beta_{t\bar{t}}$ range. To this end, two prescriptions, dubbed the D- and R-prescription, are introduced to regularise these Coulomb singularities. They embody two fundamentally different methods to truncate the threshold enhanced terms, rendering their contribution finite. In the absence of a combined threshold and small-transverse-momentum resummation, we present a quantitative assessment of the ambiguity introduced by the choice of prescription, itself a test of the sensitivity of our calculation to such threshold enhancements, for both the $d\sigma_{t\bar{t}}/dq_{\mathrm{T}}$ and $d\sigma_{t\bar{t}}/d\Delta\phi_{t\bar{t}}$ spectra.

==> text/ref_generator.tex <==
\section{Introduction} \label{sec:intro} The investigation of top-antitop pair (\ttbar) production at hadron colliders has drawn both experimental and theoretical attention in the past decades. This has facilitated the precise determination of the top quark mass $m_t$ as an input parameter of the Standard Model (SM) as well as the exploration of many possible new physics scenarios. In the recent experiments carried out at Large Hadron Collider (LHC), the total cross sections of the top-antitop pair hadroproduction has been measured at a variety of colliding energies, for instance, $\sqrt{s}=5.02\,\text{TeV}$~\cite{ATLAS:2022jbj,CMS:2017zpm, ATLAS:2021xhc,CMS:2021gwv}, $7\,\text{TeV}$~\cite{CMS:2013yjt,ATLAS:2014nxi,ATLAS:2012ptu, CMS:2016yys,CMS:2016csa,CMS:2012hcu,LHCb:2015nta, ATLAS:2022aof}, $8\,\text{TeV}$~\cite{ATLAS:2019guf,ATLAS:2016pal,CMS:2016poo, CMS:2015auz,ATLAS:2014nxi,CMS:2016yys,CMS:2016csa,LHCb:2015nta, ATLAS:2022aof}, ~$13\,\text{TeV}$~\cite{ATLAS:2023gsl,CMS:2015yky,LHCb:2018usb, ATLAS:2016qjg,ATLAS:2019hau,ATLAS:2020aln,CMS:2019snc, CMS:2016rtp,CMS:2018fks}, and~$13.6\,\text{TeV}$~\cite{CMS:2022elr,ATLAS:2023slx}. In addition, many properties of the final state have been measured in single and double-differential distributions \cite{ATLAS:2012vvt,CMS:2012hkm,ATLAS:2014ipf,ATLAS:2015dbj, ATLAS:2016pal,CMS:2017iqf,CMS:2016poo,CMS:2015rld, ATLAS:2015lsn,ATLAS:2015mip,CMS:2024ybg,CMS:2022uae, ATLAS:2023gsl,CMS:2016oae,ATLAS:2016pbv,CMS:2017xio, ATLAS:2019hau,CMS:2019esx,CMS:2020tvq,ATLAS:2020ccu, ATLAS:2022xfj,ATLAS:2022mlu,CMS:2021vhb,CMS:2018htd, CMS:2018adi,ATLAS:2019hxz}, among them the transverse momentum \qT\ of the \ttbar\ system, its invariant mass \Mttbar\ or the separation in the azimuthal plane \dPhittbar. Simultaneously, precise theoretical predictions were developed and the first \NLO\ accurate calculations, including first-order QCD corrections, became available over 30 years ago \cite{Nason:1987xz,Beenakker:1988bq,Beenakker:1990maa,Mangano:1991jk}. More recently, the precision of the theoretical predictions has been further increased by including second-order corrections at \NNLO\ accuracy in QCD \cite{Czakon:2013goa,Czakon:2015owf,Czakon:2016ckf, Czakon:2017dip,Czakon:2017wor,Catani:2019iny,Catani:2020tko, Czakon:2020coa,Czakon:2021ohs,Catani:2019hip,Garzelli:2023rvx} and first-order \NLO\ electroweak (EW) effects \cite{Bernreuther:2010ny,Kuhn:2006vh,Bernreuther:2006vg, Kuhn:2013zoa,Hollik:2011ps,Pagani:2016caq,Gutschow:2018tuk, Denner:2016jyo,Czakon:2017wor,Bernreuther:2024ltu,Frederix:2021zsh}. Alongside, corrections to top-quark decays and off-shell corrections were included \cite{Gao:2012ja,Brucherseifer:2013iv, Catani:2019hip,Behring:2019iiv,Czakon:2020qbd, Stremmer:2024ecl,Ablat:2023tiy,Meng:2022htg}. Even though these fixed-order results are able to describe the production cross sections in the majority of the phase space, considerable corrections can emerge in particular kinematic limits from all orders in the perturbative series underpinning these calculations, calling for resummation techniques to improve the perturbative convergence and, in turn, provide reliable theoretical predictions. Existing research in this context comprises soft-gluon resummation in \ttbar\ production \cite{Kidonakis:2014pja,Kidonakis:2023juy,Kidonakis:2010dk, Kidonakis:2009ev,Kidonakis:2014isa,Kidonakis:2019yji, Ahrens:2010zv,Ferroglia:2012ku,Ferroglia:2013awa,Pecjak:2016nee, Czakon:2018nun,Almeida:2008ug,Pecjak:2018lif}, the Coulomb resummation around $\Mttbar\to2m_t$ \cite{Hagiwara:2008df,Kiyo:2008bv, Ju:2020otc,Ju:2019mqc} with a generic transverse recoil against the $\ttbar$ system, the combined resummation of Coulomb and soft-gluon corrections \cite{Beneke:2009ye,Beneke:2010da,Beneke:2011mq, Cacciari:2011hy,Piclum:2018ndt}, and the resummation of soft and collinear parton emissions \cite{Zhu:2012ts,Li:2013mia,Catani:2014qha,Catani:2017tuc, Catani:2018mei,Alioli:2021ggd,Ju:2022wia} in the small transverse recoil region. Parton-shower matched predictions at the highest fixed-order precision can be found in \cite{Mazzitelli:2020jio, Mazzitelli:2021mmm,Jezo:2023rht}. In this work we will continue to study the resummation of \changed{QCD} logarithms in the process $pp\to\ttbar+X$ and put particular emphasis on the asymptotic regions $\qT\to0$ and $\dPhittbar\to\pi$. The \changed{azimuthally averaged} distribution $\done\sigma_{\ttbar}/\done\qT$ \changed{is an observable that is free of any azimuthally asymmetric divergences \cite{Catani:2017tuc}.} It thus allows for a systematic resummation of the asymptotic behaviour of each perturbative order by means of exponentiating the logarithmic contributions in impact-parameter space, akin to the corresponding procedure in the Drell-Yan process \cite{Collins:1984kg,Becher:2010tm,Bozzi:2010xn, GarciaEchevarria:2011rb,Becher:2011xn,Banfi:2011dx, Banfi:2011dm,Banfi:2012du,Catani:2015vma,Scimemi:2017etj, Bizon:2018foh,Bacchetta:2019sam,Bizon:2019zgf,Becher:2020ugp, Ebert:2020dfc,Re:2021con,Camarda:2021ict,Ju:2021lah, Camarda:2023dqn,Neumann:2022lft,Moos:2023yfa} or Higgs hadroproduction \cite{Belyaev:2005bs,Bozzi:2005wk,Bozzi:2007pn, Monni:2016ktx,Becher:2020ugp,Becher:2012yn,Neill:2015roa, Bizon:2017rah,Chen:2018pzu,Bizon:2018foh, Gutierrez-Reyes:2019rug,Harlander:2014hya,Billis:2021ecs, Cal:2023mib}. In the existing literature, focusing on the leading singular contributions \changed{in low \qT\ domain}, such a logarithmic exponentiation has been presented in \cite{Zhu:2012ts,Li:2013mia}, through a combination of the Soft-Collinear Effective Theory (SCET) \cite{Bauer:2001yt, Bauer:2001ct,Bauer:2000yr,Bauer:2000ew,Bauer:2002nz, Beneke:2002ph,Beneke:2002ni,Bauer:2002aj,Lange:2003pk, Beneke:2003pa} with the Heavy-Quark Effective Theory (HQET)~\cite{Eichten:1989zv,Georgi:1990um,Grinstein:1990mj, Neubert:1993mb}, as well as using a generalised CSS approach in \cite{Catani:2014qha,Catani:2017tuc,Catani:2018mei}. \changed{ Moreover, a second class of observables, the projected transverse momentum spectra $\done\sigma_{\ttbar}/\done q_{\tau}$, were proposed in \cite{Ju:2022wia} to remove any azimuthally asymmetric contributions, where $q_{\tau}\equiv |\qTvec \cdot \vec{\tau}|$ represents the magnitude of the projection of \qTvec\ onto a reference unit vector $\vec{\tau}$ in the transverse plane. Choosing this reference vector $\vec{\tau}$ perpendicular to the top quark spatial momentum, $\done\sigma_{\ttbar}/\done q_{\tau}$ can be related to the azimuthal decorrelation $\done\sigma_{\ttbar}/\done\dPhittbar$ between the top and antitop quarks. This observable has been of particular interest in recent measurements at the LHC \cite{CMS:2022uae,CMS:2024ybg}, where it was observed that fixed-order calculations generally exhibited significant theoretical uncertainties in the vicinity of $\dPhittbar\to\pi$, demanding the inclusion and resummation of the dominant higher-order corrections. } \changed{ In addition, Coulomb divergences appear in the physical region of top-quark pair production in the vicinity of their production threshold \cite{Hagiwara:2008df,Kiyo:2008bv, Ju:2020otc,Ju:2019mqc,Beneke:2009ye,Beneke:2010da,Beneke:2011mq, Cacciari:2011hy,Piclum:2018ndt}, characterised through $\betattbar=0$ or $\dEttbar=0$, with the relative velocity $\betattbar\equiv\sqrt{1-4m_t^2/M^2_\ttbar}$ and the energy separation $ \dEttbar\equiv \Mttbar-2m_t$. This Coulomb divergence has the potential to formally spoil the perturbative convergence of the above SCET+HQET resummed calculation. In \cite{Ju:2022wia}, in order to remove the thus afflicted region from our consideration, a lower bound on the top-antitop-pair invariant mass, $\Mttbar\ge400\,\text{GeV}$, was introduced. In the following, we will explore methods to lift this kinematic constraint, so as to extend our resummation to encompass the whole $\ttbar$ production phase space. Meanwhile, as the leading singular terms as $\qT\to0$ and $\dPhittbar\to\pi$ are driven by the same dynamic modes, we will also generalise the resummation formalism in \cite{Ju:2022wia} through an adapted multipole expansion procedure to access $\done\sigma_{\ttbar}/\done\qT$ itself. } \changed{ Ideally, the overlap of Coulomb divergences and divergences of soft-collinear origin calls for a combined resummation to study the $\qT$ and $\dPhittbar$ spectra near the threshold regime. In terms of combining SCET and potential non-relativistic QCD (pNRQCD) \cite{Pineda:1997bj,Brambilla:1999xf,Beneke:1999zr, Beneke:1999qg} (or, alternatively, velocity non-relativistic QCD, vNRQCD \cite{Luke:1999kz,Manohar:1999xd,Manohar:2000hj, Manohar:2000kr,Hoang:2002ae}), such a resummation at leading-logarithmic (LL) accuracy primarily entails the products of LO Green function \cite{Beneke:1999qg,Beneke:1999zr, Pineda:2006ri,Beneke:2011mq}, the tree-level amplitudes for the hard processes, and the Sudakov factor consisting of the cusp anomalous dimensions at LO. Even though the leading threshold enhancements induced by Coulomb interactions can be resummed at such an accuracy, it limits the perturbative corrections of soft and collinear radiation to its lowest order at leading power, thereby neglecting crucial known higher-order corrections that have been embedded in the earlier works \cite{Zhu:2012ts,Li:2013mia,Ju:2022wia}. Owing to the superrenormalisable nature of the Coulomb vertices \cite{Beneke:2009ye,Pineda:2000gza}, beyond-LL precision involves both leading and sub-leading power perturbative contributions from the soft-collinear sector, in analogy with the combination of soft and Coulomb resummation \cite{Beneke:2010da,Beneke:2011mq,Piclum:2018ndt,Ju:2019lwp}. In recent years, a lot of effort has been devoted to calculate subleading power contributions to the \qT\ spectrum in colour-singlet hadroproduction \cite{Balitsky:2017gis,Balitsky:2020jzt,Balitsky:2021fer, Balitsky:2017flc,Vladimirov:2021hdn,Ebert:2021jhy, Gamberg:2022lju,Rodini:2022wic,Rodini:2023plb, Vladimirov:2023aot,Rodini:2023mnh,Ebert:2018gsn, Inglis-Whalen:2021bea,Inglis-Whalen:2022vyn,Ferrera:2023vsw, Campbell:2024hjq}, while results for coloured heavy partons processes have still to appear. Up to now, the discussions are focussed on the on-shell production of a top-antitop quark pair. Once the region $M_\ttbar\le 2m_t$ is of one's concern, the non-resonance contribution will come into play. In spite of the fact that this kind of contributions has been investigated at leptonic collider in the vicinity of production threshold \cite{Beneke:2003xh,Beneke:2004km,Hoang:2004tg,Hoang:2006pd,Beneke:2010mp,Penin:2011gg,Jantzen:2013gpa,Beneke:2017rdn}, generalizing their calculation to hadron collider invokes extra complexity due to the event selection. Especially, in the case that jet algorithm is introduced to target the event and maintain the IRC finiteness of the decay products, the non-global dynamics \cite{Becher:2023vrh,Becher:2023mtx,Becher:2024nqc} will bring structural alteration to the factorization formulae derived in \cite{Ju:2022wia}. } \changed{ Therefore, choosing a pragmatic approach aiming for a phenomenological appraisal of both the \qT\ and \dPhittbar\ spectra, we will employ ad hoc prescriptions to achieve a meaningful soft-collinear resummation in the presence of Coulomb divergences. The expectation is that for the process $pp\to\ttbar+X$ taking place measured at a colliding energy $\sqrt{s}=13\,\text{TeV}$, the bulk of events are produced well above the \ttbar\ production threshold in the domain $\Mttbar\ge400\,\text{GeV}$ where $\betattbar\sim\order(1)$ or $\dEttbar\sim\order(m_t)$. Here, the top and antitop quarks are kinematically well separated and the dynamics behind the asymptotic behaviour are captured entirely by SCET and HQET. Then, extending the coverage of the QCD resummation established in this domain to the whole phase space including the threshold region, using such an ad hoc prescription, can serve as a rapid and reasonable estimation for the single differential observables $\done\sigma_{\ttbar}/\done\qT$ and $\done\sigma_{\ttbar}/\done\dPhittbar$ without its details having a major impact when integrated over the entire invariant mass range. Such a methodology has been extensively applied in existing calculations on the total cross section of the processes $pp\to t\bar{t}+X$ \cite{Kidonakis:1997gm,Bonciani:1998vc, Kidonakis:2001nj,Ahrens:2010zv,Czakon:2018nun}, $pp\to t\bar{t} B(B=H,Z,W^{\pm})+X$ \cite{Broggio:2015lya, Broggio:2016lfj,Broggio:2017kzi,Kulesza:2017ukk, Kulesza:2017jqv,Kulesza:2018tqz}, and $pp\to t\bar{t}t\bar{t}+X$~\cite{vanBeekveld:2022hty}. } \changed{ However, extending the resummation phase space to include the threshold regime, $\Mttbar\ge 2m_t$, is not always straightforward in a SCET$+$HQET based resummation. To be precise, the resummation in the well-separated region \cite{Ju:2022wia} features the products of the fixed-order sectors, including hard, soft, and beam-collinear functions, as well as their corresponding scale evolution kernels. In this work, we will demonstrate that, starting from next-to-next-to leading logarithmic order (\NNLL), taking the threshold limit $\beta_{\ttbar}\to0$ of those ingredients will develop cubic and quadratic divergences in the triple differential cross sections $\done^3\sigma_{\ttbar}/(\done\betattbar\done\Yttbar\done\qT)$ and $\done^3\sigma_{\ttbar}/(\done\betattbar\done\Yttbar\done\dPhittbar)$, respectively. This, in turn, leads to a diverging phase space integration in evaluating $\done\sigma_{\ttbar}/\done\qT$ and $\done\sigma_{\ttbar}/\done\dPhittbar$ without further regularisation on the threshold enhancements. } % %In this work we will continue to study the resummation of logarithms %of soft-collinear origin in the process $pp\to t\bar{t} +X$ with a %particular emphasis on the asymptotic regions $\qT\to0$ and %$\dPhittbar\to\pi$. %The single differential distributions $\done\sigma_{\ttbar}/\done\qT$ %and $\done\sigma_{\ttbar}/\done\dPhittbar$ are two observables that %are free of any azimuthal asymmetric divergences %\cite{Catani:2017tuc,Ju:2022wia}. %It thus allows for a systematic resummation of the asymptotic behaviour %of each perturbative order by means of %exponentiating the logarithmic contributions in impact-parameter space, %akin to the corresponding procedure in the Drell-Yan processes %\cite{Collins:1984kg,Becher:2010tm,Bozzi:2010xn, % GarciaEchevarria:2011rb,Becher:2011xn,Banfi:2011dx, % Banfi:2011dm,Banfi:2012du,Catani:2015vma,Scimemi:2017etj, % Bizon:2018foh,Bacchetta:2019sam,Bizon:2019zgf,Becher:2020ugp, % Ebert:2020dfc,Re:2021con,Camarda:2021ict,Ju:2021lah, % Camarda:2023dqn,Neumann:2022lft,Moos:2023yfa} or Higgs %hadroproduction \cite{Belyaev:2005bs,Bozzi:2005wk,Bozzi:2007pn, % Monni:2016ktx,Becher:2020ugp,Becher:2012yn,Neill:2015roa, % Bizon:2017rah,Chen:2018pzu,Bizon:2018foh, % Gutierrez-Reyes:2019rug,Harlander:2014hya,Billis:2021ecs, % Cal:2023mib}. %In the existing literature, focusing on singular contributions %induced by soft and beam-collinear radiation, %such a logarithmic exponentiation has been presented in %\cite{Zhu:2012ts,Li:2013mia,Ju:2022wia}, through a combination %of the Soft-Collinear Effective Theory (SCET) \cite{Bauer:2001yt, % Bauer:2001ct,Bauer:2000yr,Bauer:2000ew,Bauer:2002nz, % Beneke:2002ph,Beneke:2002ni,Bauer:2002aj,Lange:2003pk, % Beneke:2003pa} with the Heavy-Quark Effective %Theory (HQET)~\cite{Eichten:1989zv,Georgi:1990um,Grinstein:1990mj, % Neubert:1993mb}, as well as using a generalised CSS approach %in \cite{Catani:2014qha,Catani:2017tuc,Catani:2018mei}. %Even though the soft and beam-collinear modes %can accurately describe the leading asymptotic behaviour as %$\qT\to0$ or $\dPhittbar\to\pi$ in the domain where the top-antitop quark pair %is well-separated, characterised through their relative velocity %$\betattbar\equiv\sqrt{1-4m_t^2/M^2_\ttbar}$ being of $\order(1)$ \changed{or equivalently $ \dEttbar\equiv \Mttbar-2m_t\sim\order(m_t)$}, %more consideration is still needed in %extrapolating the methods of \cite{Zhu:2012ts,Li:2013mia, % Catani:2014qha,Catani:2017tuc,Catani:2018mei,Ju:2022wia} to %the threshold regime $\betattbar\to0$ as a new %dynamic region emerges through the presence of Coulomb interactions. %At variance with the logarithmic singularity of soft and beam-collinear %origin, these Coulomb interactions generate power-like divergences order %by order. %They can, therefore, render the phase-space integral ill-defined when %the entire \Mttbar\ spectrum is inclusive, e.g.\ in evaluating the single %differential observables $\done\sigma_{\ttbar}/\done\qT$ and %$\done\sigma_{\ttbar}/\done\dPhittbar$. % %Addressing these considerations, this paper will revisit the %resummation of the $\done\sigma_{\ttbar}/\done\qT$ and %$\done\sigma_{\ttbar}/\done\dPhittbar$ spectra and thereby develop %a consistent extension of our previous result in \cite{Ju:2022wia}. %Focusing on the well-separated region in our previous paper %\cite{Ju:2022wia}, we have derived the factorisation of %soft and beam-collinear radiation in the $\dPhittbar\to\pi$ %limit by means of the decoupling properties~\cite{Bauer:2001yt, % Beneke:2010da} in the leading power SCET and HQET, from %which the scale evolution method---the renormalisation group %equations (RGE) and the rapidity renormalisation group equations %(RaGE)---was applied to accomplish the logarithmic exponentiations %\cite{Chiu:2011qc,Chiu:2012ir,Li:2016axz,Li:2016ctv} and, %in turn, the QCD resummation. %In view of the common momentum modes that drive the leading singular %terms in the $\qT\to0$ and $\dPhittbar\to\pi$ limits, the resummation %formalism in \cite{Ju:2022wia} is convertible to the case %$\done\sigma_{\ttbar}/\done\qT$ upon an appropriate adaptation of %the multipole expansion procedure. %In this paper, we will analyse the threshold behaviour of each %arising sector in the $\dPhittbar$ and \qT\ resummation up to \NNLL. %The asymptotic behaviour of the beam-collinear, soft, and resummation %kernels in the limit of $\betattbar\to0$ will be derived from their %analytic expressions, while to address the hard sector, potential %non-relativistic QCD (pNRQCD) \cite{Pineda:1997bj,Brambilla:1999xf, % Beneke:1999zr,Beneke:1999qg} will be used to extract the leading %threshold enhanced terms from the relevant partonic amplitudes at the %one-loop level. %Combining the leading contributions of all sectors, we will demonstrate %that the triple differential cross sections %$\done^3\sigma_{\ttbar}/(\done\betattbar\done\Yttbar\done\qT)$ and %$\done^3\sigma_{\ttbar}/(\done\betattbar\done\Yttbar\done\dPhittbar)$ %approach constants at \NLL\ but develop cubic and quadratic divergences %at \NNLL\ as $\betattbar\to0$. %This phenomenon indicates that a literal implementation of the framework %in \cite{Ju:2022wia} to the resum $\done\sigma_{\ttbar}/\done\qT$ or %$\done\sigma_{\ttbar}/\done\dPhittbar$ over the full \Mttbar\ phase space %is only possible at \NLL. %At higher orders it inevitably incurs power-like divergences in %\betattbar\ in the threshold domain, leading to divergent integrals over %\betattbar\ or \Mttbar, respectively. % % % {\color{blue} ---------------------------------------------------------------------------------} \changed{To this end, in this paper, we introduce two ad hoc prescriptions to treat this problem.} Their derivation is based on the observation that in using the expanded solution of the hard RGE~\cite{Buras:1991jm,Buchalla:1995vs} the main driver for the threshold divergences are the non-logarithmic products of the hard scale evolution kernels, contributing $\mathcal{O}(\betattbar^{-4})$ in the limit of $\betattbar\to0$. Ideally, this behaviour can be mitigated by implementing the exact solution of the hard RGE. However, in presence of soft colour correlations, such an exact solution necessitates the path-ordered integration over a set of threshold-enhanced colour matrices. Unfortunately, neither an analytically compact expression nor a numerical approximation via Taylor expansion is straightforward. Hence, \changed{akin to \cite{Kulesza:2017ukk,Alioli:2021ggd, Ahrens:2010zv,Zhu:2012ts,Li:2013mia}}, we first introduce the ``decomposition (D) \changed{prescription}'', in which the threshold-singular contributions at \NNLL\ are, in part, shifted to a higher logarithmic accuracy at the cost of mild corrections in the domain $\betattbar\sim\mathcal{O}(1)$. \changed{It} allows a smooth and consistent extrapolation to the threshold area $\betattbar\to0$. On the other hand, we will also introduce the ``re-exponentiation (R) \changed{prescription}''. In spite of the difficulties in determining a rigorous solution of hard RGE for a generic \betattbar, we will demonstrate that solving hard RGE can be substantially simplified in the vicinity of $\betattbar=0$. This is thanks to the fact that up to two-loop level the leading threshold divergences all reside in the diagonal entries of the hard anomalous dimensions~\cite{Ferroglia:2009ii,Ferroglia:2009ep}. Consequently, the leading singular behaviour of the hard anomalous dimensions can be exponentiated by solving an approximate hard RGE. The resulting resummation kernels in the R-\changed{prescription} present intensively oscillatory but integrable behaviour in the limit $\betattbar\to0$. \changed{Due to the fact that in these prescriptions, the threshold enhanced series are truncated in two radically different approaches, comparing their outcome can deliver a quantitative assessment on the dependence of $\done\sigma_{\ttbar}/\done\qT$ and $\done\sigma_{\ttbar}/\done\dPhittbar$ on the ad hoc prescriptions and in turn unveil their sensitivity to the higher order Coulomb interactions.} %By means of a numerical implementation, we will compare the results of both schemes and thereby deliver a quantitative assessment of the theoretical uncertainty caused by perturbative truncation in the threshold enhanced contribution. %%%%%%%%%%%%%%%%%%%%%%%%%%%% % memo % a) The S.Catani's resummation framework is argued to be valid up to N2LL in \cite{Catani:2014qha} but in practice only NLL \cite{Catani:2017tuc,Catani:2018mei} is hitherto published. % b) G.Sterman's paper 0805.1885/{Almeida:2008ug} focuses on NLL with the numeric exponentiation where hard anomalous is harmless since the Coulomb divergence only participate into imaginary parts which will drop out when evaluating the product of V and V^dagger %%%%%%%%%%%%%%%%%%%%%%%%%%%% %{\color{blue} ---------------------------------------------------------------------------------} % %\changed{I plan to remove the following discussions since they look pointless. The reason I added them was because I was not clear how Pacjack dealt with such a threshold divergences but now I see. } % %Finally, it should be noted that there already exists a partial %solution to the problem of extending a QCD resummation into the %threshold region, as %suggested in the soft \cite{Kulesza:2017ukk} and zero-jettiness %\cite{Alioli:2021ggd} resummations. %The therein proposed solution is in practice equivalent to the %D-scheme in this work and able to circumvent the threshold divergences %at \NNLL\ in a similar manner.\footnote{ % An equivalent method has also been embedded into the in-house % numerical programs of the \qT\ \cite{Zhu:2012ts,Li:2013mia} % and threshold \cite{Ahrens:2010zv} resummations for achieving % \NNLL\ precisions. %} % % %However, to our best knowledge, the motives to introduce such a %prescription in place of the original one in~\cite{Buras:1991jm, % Buchalla:1995vs} and its arising theoretical uncertainties in %the respective \Mttbar\ regions are rarely discussed in the existing %literature. %Decoding these theoretical subtleties will be helpful to interpret %the restriction of current resummation formalisms and will also help %to facilitate the comparison between the best QCD predictions and %the latest experimental measurements \cite{CMS:2024ybg,CMS:2022uae} %for both single and double differential distributions, %$\done\sigma_\ttbar/\done\mathcal{Q}$ and %$\done^2\sigma_\ttbar/(\done\Mttbar\done\mathcal{Q})$ with %$\mathcal{Q}$ denoting \qT\ or \dPhittbar. %%%%%%%%%%%%%%%%%%%%%%%%%%%% % memo % please note in DGLAP evolution and weak wilson evolution the product of $J$ has been taken into account +add references %%%%%%%%%%%%%%%%%%%%%%%%%%%% The paper is structured as follows. In Sec.~\ref{sec:methods} we start with a brief review of the soft-collinear resummation on the \qT\ and \dPhittbar\ spectra for the well-separated region, thereby specifying the fixed-order ingredients and anomalous dimensions comprised up to \NNLL. Then, Sec.~\ref{sec:sigma:thr:hqet} is devoted to an analysis of the asymptotic behaviour of \changed{HQET and SCET based resummation} %$\done^3\sigma_{\ttbar}/(\done\betattbar\done\Yttbar\done\qT)$ and $\done^3\sigma_{\ttbar}/(\done\betattbar\done\Yttbar\done\dPhittbar)$ in the vicinity of $\betattbar\to0$, from which we raise the concern over the integrability of the resummation kernel at \NNLL. In turn, we propose the two \changed{ad hoc} prescriptions discussed above in Sec.~\ref{sec:thr:div:extrap} to mitigate the arising threshold singularities before we match the resummed \qT\ and \dPhittbar\ distributions to the exact fixed-order calculations in Sec. \ref{sec:mat}. With our framework in place, we deliver a numeric evaluation in Sec.~\ref{sec:results}. Therein, we will at first validate the perturbative expansion of our resummed results by comparing against the \qT\ and \dPhittbar\ distribution computed in the full theory in three different \Mttbar\ slices, i.e.\ the threshold domain $\Mttbar\in[2m_t, 360]\,\text{GeV}$, the transitional region $\Mttbar\in[360,400]\,\text{GeV}$, and the well-separated realm $\Mttbar\ge400\,\text{GeV}$. Finally, we present our final resummation improved \qT\ and \dPhittbar\ distributions at \NNLLNNLO\ accuracy using both the D- and R-schemes before concluding this work in Sec.~\ref{sec:conclusions}. \section{Theoretical details} \label{sec:methods} \subsection{Soft and collinear resummation in the domain \texorpdfstring{$\dEttbar\sim\mathcal{O}(m_t)$}{Delta E of O(mt)}} \label{sec:methods:domains} From the QCD factorisation theorem~\cite{Collins:1989gx}, the differential cross section of a generic observable $\mathcal{Q}$ for the process $pp\to \ttbar+X$ can be expressed as, \begin{equation}\label{eq:QCDF} \begin{split} \frac{\done^3{\sigma_{\ttbar}}} {\done \Mttbar^2\, \done \Yttbar\,\done \mathcal{Q}} \,=\;& \sum_{\mathrm{sign}[P_{t}^{z}]}\frac{1}{16s\,(2\pi)^6 } \int \done^2\vec{P}_{t}^{\perp}\,\done^2 \qTvec\; \delta\Big[\mathcal{Q}-\mathcal{F}_{\mathcal{Q}}\Big]\; \frac{\Sigma_{\ttbar}}{\MTttbar\,|P_{t}^{z}|}\,, \end{split} \end{equation} where $s$ denotes collider energy and will be taken to be $13\,\text{TeV}$ throughout our investigation. $\vec{P}_{t}^{\perp}$ stands for the transverse momentum of the top quark measured in the laboratory reference frame (LRF), while $ P_{t}^{z}$ marks its longitudinal components detected from the $z$-direction rest frame ($z$RF) of the top-antitop pair. Further, $\qTvec$, $\Mttbar$, and $\Yttbar$ represent the transverse momentum, invariant mass and pseudo-rapidity of the $\ttbar$ system in LRF, respectively, from which the transverse mass of the top-antitop pair can be expressed as \begin{align} \Mttbar^{\mathrm{T}}=\sqrt{\Mttbar^2+\qT^2}. \end{align} $\mathcal{Q}$ in Eq.~\eqref{eq:QCDF} refers to the observable, which can be evaluated via its definition function $\mathcal{F}_{\mathcal{Q}}$. $\mathcal{F}_{\mathcal{Q}}$ takes the following form for the observables of interest in the present paper, \begin{align} \label{eq:meas:func:qT_dphi} \begin{split} \mathcal{Q}&=\qT\,,\quad\quad\quad\quad\quad\quad \quad\quad ~~~~\mathcal{F}_{\mathcal{Q}}=\changed{\left|\qTvec\right|}\,,\\ \mathcal{Q}&= \Delta\phi_{\ttbar}\equiv\pi-\Delta\Phi_{\ttbar} \,,\quad\quad\quad \mathcal{F}_{\mathcal{Q}}=\pi-\arccos \left[\frac{\vec{P}^{\bot}_t\cdot \vec{P}^{\bot}_{ \tbar}}{ |\vec{P}^{\bot}_t | |\vec{P}^{\bot}_{ \tbar} |}\right]\,. \end{split} \end{align} Here, $\vec{P}^{\bot}_{\tbar}$ stands for the transverse momenta of the antitop quark in the LRF, satisfying $\vec{P}^{\bot}_{\tbar}=\qTvec-\vec{P}^{\bot}_{t}$. $\Delta\Phi_{\ttbar}$ measures the azimuthal separation of the top and antitop quarks in the transverse plane. At last, ${\Sigma_{\ttbar}}$ in Eq.~\eqref{eq:QCDF} collects the contributions from all participating partonic processes, \begin{align}\label{eq:def:QCD:parton} \begin{split} {\Sigma_{\ttbar}} \,=&\; \sum_{i,j} \int^1_0 \frac{\done x_n}{x_n}\, \frac{\done x_{\nbar}}{x_{\nbar}}\, f_{i/N}(x_n)\,f_{j/\bar{N}}(x_{\nbar})\, \sum_{r\changed{=0}}^{\changed{\infty}}\,\int\, \left[\prod_{m\changed{=1}}^r \frac{\done^3 \vec{k}_m}{(2\pi)^3\,2E_{k_m}}\right] \overline{\sum_{\mathrm{hel, col}}} \left|\mathcal{M}(i+j\to t+\tbar+ X ) \right|^2\\ &\hspace*{70mm} \times\; (2\pi)^4\;\delta^4\left(p_i+p_{j}-P_{t}-P_{\tbar}-\sum_{m\changed{=0}}^{\changed{r}} k_m\right)\,, \end{split} \end{align} where the $f_{i/N}(x)$ is the parton distribution function (PDF) for parton $i$ with the momentum fraction $x$ from proton $N$, and $E_{k_m}$ and $\vec{k}_{m}$ are the energy and spatial momentum of the $m$-th emitted parton, respectively. $\mathcal{M}$ evaluates the transition amplitude of the occurring partonic scattering $i+j\to t+\tbar+X$, with $\{i,j\}\in[u,\bar{u},d,\bar{d},s,\bar{s},c,\bar{c},b,\bar{b},g]$, in line with the $5$ active flavour scheme. Substituting Eq.\ \eqref{eq:def:QCD:parton} into Eq.\ \eqref{eq:QCDF}, we can now appraise the $\qT$ and $\Delta\phi_{\ttbar}$ spectra on the fixed-order level. Although such a calculation delivers satisfactory predictions in most phase space regions, it converges poorly as $\qT\to0$ or $\dphittbar\to0$ due to the occurrence of large logarithmic corrections to all orders. Thus, a resummation of this asymptotic behaviour is mandated. In the domain where the top and antitop quarks are kinematically well-separated, i.e.\ \begin{align}\label{eq:defdE} \dEttbar\equiv \Mttbar-2m_t\sim\order(m_t)\,, \end{align} the factorisation and resummation of the azimuthally averaged distribution $\done{\sigma_{\ttbar}}/\done\qT$ have been investigated in different approaches, including the EFT-based analysis~\cite{Zhu:2012ts,Li:2013mia} and the generalized CSS framework~\cite{Catani:2014qha,Bonciani:2015sha, Catani:2017tuc,Catani:2018mei}. It is demonstrated that (at least) the leading singular behaviour of the \qT\ distribution is predominantly driven by the hard, soft and beam-collinear domains in the loop and phase space integrations. This conclusion has been extensively applied in fixed order calculations \cite{Bonciani:2015sha,Catani:2019iny,Catani:2019hip,Catani:2020tko,Garzelli:2023rvx,Catani:2021cbl,Catani:2022mfv,Buonocore:2022pqq,Catani:2020kkl,Buonocore:2023ljm} and also their combination with parton showers \cite{Mazzitelli:2020jio,Mazzitelli:2021mmm,Mazzitelli:2023znt,Mazzitelli:2024ura}. Recently, to further investigate the top-antitop-pair dynamics, the differential distribution of the projected transverse momentum $\done{\sigma_{\ttbar}}/\done q_{\tau}$ was computed in \cite{Ju:2022wia}, where $q_{\tau}$ signifies the projection of $\qTvec$ onto a reference unit vector $\vec{\tau}$ on the azimuthal plane, from which the $\Delta\phi_{\ttbar}$ spectrum can be derived by choosing $\vec{\tau}$ perpendicular to the flight direction of (anti)top quark. At variance with the small \qT\ region, which imposes constraints on both components of $\qTvec$, the asymptotic regime $q_{\tau}\to0$ or $\Delta\phi_{\ttbar}\to0$ concerns only the longitudinal projection $q_{\tau}=|\qTvec\cdot \vec{\tau}|$, leaving the transverse part unresolved. To probe the dynamic modes for the transverse component, in \cite{Ju:2022wia}, employing the method of expansion of dynamic regions \cite{Beneke:1997zp,Smirnov:2002pj,Smirnov:2012gma, Jantzen:2011nz} as well as the SCET formalism \cite{Bauer:2001yt, Bauer:2001ct,Bauer:2000yr,Bauer:2000ew,Bauer:2002nz, Beneke:2002ph,Beneke:2002ni,Bauer:2002aj,Lange:2003pk, Beneke:2003pa}, we enumerate the possible regions that can prompt energetic recoil against the top-antitop system, finding that assigning the label momenta to the transverse direction will incur an additional suppression from the phase space by at least one power of $\lambda_{\tau}\equiv q_{\tau}/\Mttbar$, such that the leading singular behaviour of $\done{\sigma_{\ttbar}}/\done q_{\tau}$ is also captured by the hard, soft and beam-collinear regions, akin to the \qT\ resummation in \cite{Zhu:2012ts,Li:2013mia,Catani:2014qha}. Given their common dynamic regions that preside over the leading singular contributions \footnote{% As far as we know, this coincidence only takes place in the leading power factorisation and resummation, since without accidental cancellations the central collinear mode can be relevant for $\done\sigma_{\ttbar}/\done\Delta\phi_{\ttbar}$ starting from the subleading power~\cite{Ju:2022wia}, whereas its participation in $\done\sigma_{\ttbar}/\done\qT$ is postponed to the sub-subleading power by its kinematics \cite{Collins:1980ui,Collins:1981uk,Ju:2022wia}. Analogously, structural similarities between Eqs.~(\ref{eq:LP:res}-\ref{eq:LP:res:gg}) and those governing resummation-improved azimuthal decorrelation of the jet-boson~\cite{Chien:2019gyf,Chen:2018fqu,Chien:2020hzh, Bouaziz:2022tik,Chien:2022wiq} and dijet \cite{delCastillo:2021znl,Banfi:2008qs,Zhang:2022wvs, Gao:2023ulg} processes may also be limited to leading power, especially when the jets therein are defined exclusively. }, we can utilise a uniform framework to compute the resummed expressions for both the $\qT$ and $\Delta\phi_{\ttbar}$ distributions. Within the context of \SCETII~\cite{Bauer:2002aj,Lange:2003pk, Beneke:2003pa} and HQET~\cite{Eichten:1989zv,Georgi:1990um, Grinstein:1990mj,Neubert:1993mb}, both of them comprise the resummed partonic function, \begin{align}\label{eq:LP:res} \Sigma_{\ttbar }^{\mathrm{res}} =&\; \frac{8\pi^2}{\Mttbar^2}\, \sum_{\kappa}\, \int {\done^2\bTvec}\,\exp\left(\mathrm{i}\,\bTvec \cdot\qTvec \right)\, \widetilde{\Sigma}_{\ttbar}^{\mathrm{res}, [\kappa]} (\bTvec,\Yttbar, \Mttbar,\Omega_t)\,, \end{align} where $\kappa$ runs over $\{g_{n}g_{\nbar},q^i_{n}\qbar^j_{\nbar},q^i_{\nbar}\qbar^j_{n}\}$, enumerating the active initial-state parton-pairs contributing to the hard kernels, with $i,j\in\{u,d,c,s,b\}$ specifying the flavour of the quark fields. $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$ collects the partonic contribution after Fourier transforming it into impact-parameter space, which is in general a function of the impact parameter $\bTvec$, the pseudorapidity $\Yttbar$, the invariant mass $\Mttbar$, and the solid angle $\Omega_t$ of the top quark measured in the rest reference frame of $\ttbar$ system. $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$ is formally related to the choice of the scheme regularising the rapidity divergences. In the following, we will use the soft and beam functions evaluated within the exponential regulator as proposed in \cite{Li:2016axz,Li:2016ctv}. Alternative choices can also be found in \cite{Zhu:2012ts, Li:2013mia,Angeles-Martinez:2018mqh,Gehrmann:2012ze, Gehrmann:2014yya} calculated via analytic rapidity regulator \cite{Becher:2011dz}, and in \cite{Catani:2011kr,Catani:2021cbl,Catani:2022sgr,Catani:2023tby} using a generalised CSS method~\cite{Catani:2014qha}. It follows that, \begin{align} \label{eq:LP:res:qqbar} \begin{split} &\hspace*{-5mm} \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[q^i_{n}\qbar^j_{\nbar}]} (\bTvec,\Yttbar, \Mttbar,\Omega_t)\\ \,=&\; \left(\frac{1}{2N_c}\right)^2\, \mathcal{D}^{\mathrm{res}}_{[q^i_{n}\qbar^j_{\nbar}]} (\bT,\Mttbar,\mu_h,\mu_b,\mu_s,\nu_b,\nu_s)\, \mathcal{B}_{n}^{[q_n^i]}(\eta_n,\bT,\mu_b,\nu_b)\, \mathcal{B}_{\nbar}^{[\qbar_\nbar^j]}(\eta_{\nbar},\bT,\mu_b,\nu_b) \, \\ & \sum_{\{\alpha,\beta,h\}}\Bigg\{ \mathcal{S}^{\alpha_1\beta_1}_{[q_{n}\qbar_{\nbar}]}(\bTvec,v_{t},v_{\tbar},\mu_s,\nu_s) \left[\mathcal{V}^{[q_{n}\qbar_{\nbar}]}_{\alpha_1\alpha_2}(v_{t},v_{\tbar},\mu_s,\mu_h) \mathcal{C}^{[q^i_{n}\qbar^j_{\nbar}]}_{\alpha_2;h_nh_{\nbar}h_th_{\tbar}} \right]^*\, \mathcal{V}^{[q_{n}\qbar_{\nbar}]}_{\beta_1\beta_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \\ & \mathcal{C}_{\beta_2;h_nh_{\nbar}h_th_{\tbar}}^{[q^i_{n}\qbar^j_{\nbar}]}\, \Bigg\}\,, \end{split} \end{align} and \begin{align} \label{eq:LP:res:gg} \begin{split} &\hspace*{-5mm} \widetilde{\Sigma}_{\ttbar }^{\mathrm{res},[g_{n}g_{\nbar}]} (\bTvec,\Yttbar, \Mttbar,\Omega_t)\\ \,=&\; \left(\frac{1}{N^2_c-1}\right)^2\, \mathcal{D}^{\mathrm{res}}_{[g_{n}g_{\nbar}]} (\bT,\Mttbar,\mu_h,\mu_b,\mu_s,\nu_b,\nu_s)\, \sum_{\{\alpha,\beta, h,h'\}} \Bigg\{ \mathcal{S}^{\alpha_1\beta_1}_{[g_ng_{\nbar}]}(\bTvec,v_{t},v_{\tbar},\mu_s,\nu_s)\, \\ &\times\, \mathcal{B}^{[g_n]}_{n,h_n'{h_n}}(\eta_n,\bTvec,\mu_b,\nu_b)\, \mathcal{B}^{[g_{\nbar}]}_{\nbar,h_{\nbar}'{h_{\nbar}}}(\eta_{\nbar},\bTvec,\mu_b,\nu_b) \, \left[\mathcal{V}^{[g_{n}g_{\nbar}]}_{\alpha_1\alpha_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\mathcal{C}^{[g_{n}g_{\nbar}]}_{\alpha_2;h'_nh'_{\nbar}h_th_{\tbar}}\right]^*\, \\ &\times \mathcal{V}^{[g_{n}g_{\nbar}]}_{\beta_1\beta_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}_{\beta_2;h_nh_{\nbar}h_th_{\tbar}}^{[g_ng_{\nbar}]}\, \Bigg\}\,, \end{split} \end{align} where the soft function is given by $\mathcal{S}^{\alpha\beta}_{[\kappa]}$ as a function of the impact parameter $\bTvec$, the velocity $v_{t(\tbar)}$ of the (anti)top quark, and the soft virtuality (rapidity) scale $\mu_s(\nu_s)$. To facilitate our calculations, we have projected the colour states of the soft function onto the orthonormal bases $c_{\{a_i\}}^{qq}$ and $c_{\{a_i\}}^{gg}$ of \cite{Beneke:2009rj}, leading to the colour indices $\{\alpha,\beta\}$ emerging as superscripts. \changed{Their expressions are presented in App.~\ref{app:def:col:spin}.} It is important to note that, heretofore, while the azimuthally averaged soft function have been calculated up to \NNLO~\cite{Angeles-Martinez:2018mqh,Catani:2023tby}, its fully azimuthal-angle-dependent form that are essential to compute the $\phi_{\ttbar}$ resummation are only available at \NLO~\cite{Catani:2021cbl,Ju:2022wia}. Furthermore, Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg} include the hard functions $\mathcal{C}_{\alpha;h_nh_{\nbar}h_th_{\tbar}}^{[q^i_{n}\qbar^j_{\nbar}]}$ and $\mathcal{C}_{\beta;h_nh_{\nbar}h_th_{\tbar}}^{[g_ng_{\nbar}]}$ which consist of the UV-renormalized and IRC-subtracted amplitudes of the relevant hard partonic processes. Again, the $\{\alpha,\beta\}$ encode the colour states as in the soft function, while the tuple $\{h_{n},h_{\nbar},h_t,h_{\tbar}\}$ is introduced to specify the helicity states of the external particles. Throughout this work, the helicity bases of \cite{Actis:2012qn,Actis:2016mpe} are taken as our default choice to evaluate the helicity projections \changed{ and we present their expression in App.~\ref{app:def:col:spin}.} In calculating $\mathcal{C}_{\alpha;h_nh_{\nbar}h_th_{\tbar}}^{[q^i_{n}\qbar^j_{\nbar}]}$ and $\mathcal{C}_{\beta;h_nh_{\nbar}h_th_{\tbar}}^{[g_ng_{\nbar}]}$, the \MSbar\ scheme is utilised to renormalise the UV divergences associated with the massless partons and the zero-momentum subtraction prescription \cite{Beenakker:2002nc} is employed to cope with those pertaining to the (anti)top quarks. The remaining IRC singularities are removed following the procedures in \cite{Ferroglia:2009ii}. Up to \NLO, the automated program \Recola~\cite{Actis:2012qn,Actis:2016mpe} is employed in this paper to extract the amplitudes of $\qqbar\to\ttbar$ and $gg\to\ttbar$ in all the helicity and colour configurations. The \NNLO\ calculation are more involved. For now, the grid-based numerical results have been presented in \cite{Chen:2017jvi}, while the progress towards the full analytic evaluations are made in \cite{DiVita:2019lpl,Badger:2021owl,Mandal:2022vju,Wang:2023qbf}. Next, Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg} also comprise the beam functions $\mathcal{B}_{n(\nbar)}^{[q_{n(\nbar)}^i]}$ and $\mathcal{B}^{[g_{n(\nbar)}]}_{n(\nbar)}$ governing the beam-collinear contributions along the $n(\nbar)$-direction. They are the functions of the virtuality (rapidity) scale $\mu_b(\nu_b)$ and the momentum fractions $\eta_n={\Mttbar\,e^{\Yttbar}}/{\sqrt{s}}$ and $\eta_\nbar={\Mttbar\,e^{-\Yttbar}}/{\sqrt{s}}$. In comparison with the quark beam function $\mathcal{B}_{n(\nbar)}^{[q_{n(\nbar)}^i ]}$, the gluon case additionally depends on the gluon helicities $\{h_{n(\nbar)},h_{n(\nbar)}'\}\in\{+,-\}$ to accommodate the helicity-flipping and helicity-conserving contributions. At present, the quark beam function, $\mathcal{B}_{n(\nbar)}^{[q_{n(\nbar)}^i]}$, and the helicity-conserving components of the gluon beam function, $\mathcal{B}_{n(\nbar),++}^{[g_{n(\nbar)}]}$ and $\mathcal{B}_{n(\nbar),--}^{[g_{n(\nbar)}]}$, have been calculated up to \NNNLO\ \cite{Luo:2020epw,Luo:2019szz,Luo:2019bmw,Luo:2020epw}, while the helicity-flipping entries $\mathcal{B}_{n(\nbar),+-}^{[g_{n(\nbar)}]}$ and $\mathcal{B}_{n(\nbar),-+}^{[g_{n(\nbar)}]}$ are only know on the \NNLO\ level \cite{Luo:2019bmw,Gutierrez-Reyes:2019rug,Catani:2022sgr}. Finally, in addition to the above fixed-order contributions, Eqs.\ \eqsref{eq:LP:res:qqbar}{eq:LP:res:gg} contains the evolution kernels $\mathcal{D}^{\mathrm{res}}_{[\kappa]}$ and $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ as well. They bridge the gap between the intrinsic scales in the hard, soft, and beam-collinear contributions by resumming the occurring large logarithms and are derived by solving the respective R(a)GEs of the corresponding constituents \cite{Chiu:2011qc,Chiu:2012ir,Li:2016axz,Li:2016ctv}. For instance, $ \mathcal{D}^{\mathrm{res}}_{[\kappa]}$ consists of the solutions of the beam-collinear R(a)GEs and the diagonal part of the hard RGEs, see~\cite{Ju:2022wia}, \begin{align} \label{eq:def:Dres} &\ln\mathcal{D}^{\mathrm{res}}_{[\kappa]} (\bT,\Mttbar,\mu_h,\mu_b,\mu_s,\nu_b,\nu_s) \nnb\\ &\,=\; \int^{\mu^2_s}_{\mu^2_b} \, \frac{\done\bar{\mu}^2}{\bar{\mu}^2}\, \Bigg\{ C_{[\kappa]}\, \Gamma_{\mathrm{cusp}}\big[\alpha_s(\bar{\mu}) \big]\, \ln\bigg[ \frac{\nu_b^2}{\Mttbar^2}\bigg] +2\,\gamma^{[\kappa]}_b\big[\alpha_s(\bar{\mu}) \big]\, \Bigg\} -\int^{\mu_s^2}_{\mu_h^2}\frac{\done \bar{\mu}^2}{\bar{\mu}^2}\, \bigg\{ {C_{[\kappa]}}\, \Gamma_{\mathrm{cusp}}\big[\alpha_s(\bar{\mu}) \big]\, \ln\left[\frac{\bar{\mu}^2}{\Mttbar^2}\right]\,\bigg\}\nnb \\ &\,\phantom{=}\;{} +C_{[\kappa]}\, \ln\bigg[\frac{\nu_s^2}{\nu_b^2}\bigg]\, \int_\frac{b_0^2}{\bT^2}^{\mu_s^2}\, \frac{\done\bar{\mu}^2}{\bar{\mu}^2}\, \Gamma_{\mathrm{cusp}}\big[\alpha_s(\bar{\mu}) \big]\, -C_{[\kappa]}\, \ln\bigg[\frac{\nu_s^2}{\nu_b^2}\bigg]\, \gamma_r \bigg[\alpha_s\left(\frac{b_0}{\bT}\right)\bigg]\,. \end{align} Therein, $\Gamma_{\mathrm{cusp}}$, $\gamma^{[\kappa]}_b$, and $\gamma_r$ denote the cusp anomalous dimension, the non-cusp anomalous dimension associated with the virtuality divergences in the beam functions, and the non-cusp anomalous dimension of the rapidity renormalisation. All their expressions up to \NNNNLO\ are already available in the literature \cite{Moch:2004pa,Henn:2019swt,vonManteuffel:2020vjv,Herzog:2018kwj} and \cite{Li:2016axz,Luo:2019bmw,Luo:2019hmp,Li:2016ctv, Vladimirov:2016dll,Luo:2020epw,Ebert:2020yqt,Luo:2019szz, Das:2019btv,Duhr:2022cob,Duhr:2022yyp,Moult:2022xzt}, respectively. In writing Eq.~\eqref{eq:def:Dres}, the following abbreviations are employed for the corresponding colour factor in QCD, \begin{align} \kappa\in\{g_{n}g_{\nbar}\}\,:\; C_{[\kappa]}=C_A\;,\qquad\qquad \kappa\in\{q^i_{n}\qbar^j_{\nbar},q^i_{\nbar}\qbar^j_{n}\}\,:\; C_{[\kappa]}=C_F\,, \end{align} as well as the non-cusp anomalous dimensions, \begin{equation} \kappa\in\{g_{n}g_{\nbar}\}\,:\; \gamma_b^{[\kappa]}=\gamma_b^{[g]}\,, \qquad\qquad \kappa\in\{q^i_{n}\qbar^j_{\nbar},q^i_{\nbar}\qbar^j_{n}\}\,:\; \gamma_b^{[\kappa]}=\gamma_b^{[q]}\,. \end{equation} Complementarily, the $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ are in charge of the non-cusp hard anomalous dimension $\gamma^{[\kappa]}_h$ \cite{Ferroglia:2009ii,Ferroglia:2009ep}. Up to \NLL, the $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ can be derived by solving the RGE of the hard function in the diagonal colour space \cite{Buras:1991jm,Buchalla:1995vs,Ahrens:2010zv}, \begin{align}\label{eq:def:Vres:NLL} \mathbf{V}_h^{[\kappa]}(v_t,v_{\tbar},\mu_s,\mu_h)\Bigg|_{\mathrm{NLL} } \,=\; \mathbf{R}^{-1}_{[\kappa]}\, \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \mathbf{R}_{[\kappa]}\,, \end{align} where $\mathbf{V}_h^{[\kappa]}$ is the matrix representation of $\mathcal{V}^{[\kappa]}_{\alpha\beta}$. $\mathbf{r}^{[\kappa],(0)}_{h}$ stands for the diagonalised one-loop non-cusp anomalous dimension of the hard function, by means of the invertible transformation matrix $\mathbf{R}_{[\kappa]}$. $\alpha_s$ denotes the strong coupling evaluated in the $N_F=5$ flavour scheme, with the according anomalous dimension $\beta_k$ at $(k+1)$-loop accuracy. This approach can also been generalized to \NNLL\ by including the off-diagonal entries of the two-loop hard anomalous dimensions as appropriate \changed{\cite{Buras:1991jm,Buchalla:1995vs}}, i.e., \begin{align}\label{eq:def:Vres:N2LL} \begin{split} &\mathbf{V}_h^{[\kappa]}(v_t,v_{\tbar},\mu_s,\mu_h)\Bigg|_{\NNLL} \\ &\,=\; \mathbf{R}^{-1}_{[\kappa]}\, \bigg[\mathbf{I}+\frac{\alpha_s(\mu_s)}{4\pi}\mathbf{J}^{[\kappa]}\bigg]\, \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \bigg[ \mathbf{I}-\frac{\alpha_s(\mu_h)}{4\pi}\mathbf{J}^{[\kappa]} \bigg]\, \mathbf{R}_{[\kappa]}\,, \end{split} \end{align} where the matrix $\mathbf{J}^{[\kappa]}$ is introduced here to take in the two loop ingredients, \begin{align} \label{eq:def:Vres:N2LL:Jmax} \mathbf{J}^{[\kappa]}_{ij} \,=\; \mathbf{r}^{{[\kappa]},(0)}_{h,ii}\; \delta_{ij}\,\frac{\beta_1}{2\beta^2_0} -\frac{\mathbf{r}^{{[\kappa]},(1)}_{h,ij}} {2\beta_0+\mathbf{r}^{{[\kappa]},(0)}_{h,ii} -\mathbf{r}^{{[\kappa]},(0)}_{h,jj}}\,, \end{align} Herein, $\delta_{ij}$ represents the Kronecker delta function carrying the indices $\{i,j\}\in\{1,2\}\;(\{1,2,3\}$) for the quark (gluon) channel. $\mathbf{r}^{{[\kappa]},(1)}_{h}$ is defined analogously to $\mathbf{r}^{{[\kappa]},(0)}_{h}$ in terms of the two-loop non-cusp anomalous dimension $\gamma^{(1)}_h$ within the diagonal space of $\gamma^{(0)}_h$. %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% % memo % it would be good to spell out the counting rule %\begin{equation}\label{eq:intro:def_res_order} % \begin{split} % \frac{ \done{\sigma}_{\ttbar}} {\done q_{\tau} } % \sim&\; % \sigma^\text{Born}_{\ttbar} % \, % \exp\bigg[\; % \underbrace{L_{\mathrm{M}}\, f_0(\alpha_sL_{\mathrm{M}})}_{(\text{LL})} % +\underbrace{f_1(\alpha_sL_{\mathrm{M}})}_{(\text{NLL,NLL$'$})} % +\underbrace{\alpha_s\, f_2(\alpha_sL_{\mathrm{M}})}_{(\text{N$^2$LL,N$^2$LL$'$})} % +\underbrace{\alpha^2_s\, f_3(\alpha_sL_{\mathrm{M}})}_{(\text{N$^3$LL,N$^3$LL$'$})} % +\ldots\; % \bigg] \\ % &\quad\times % \bigg\{ % 1 (\text{LL,NLL})+ % \alpha_s (\text{NLL$'$,N$^2$LL})+ % \alpha_s^2 (\text{N$^2$LL$'$,N$^3$LL})+ % \alpha_s^3 (\text{N$^3$LL$'$,N$^4$LL})+ % \ldots % \bigg\} \, . % \end{split} %\end{equation} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Reinserting the results of Eqs.\ \eqsref{eq:LP:res:qqbar}{eq:LP:res:gg} into Eq.~\eqref{eq:QCDF} and expanding the kinematic variables to leading power, we arrive at the resummed \qT\ and \dphittbar\ spectra~\cite{Ju:2022wia}, %\commentWJ{Checked!} \begin{align}\label{eq:methods:res:qT_dphi} \begin{split} \frac{\done{\sigma^{\mathrm{res}}_{\ttbar}}} {\done \qT} \,=\;& \changed{ \frac{\qT}{64\pi^3\,s} \sum_{\kappa,\mathrm{sign}[\widetilde{P}^z_{t}]} \int\done\Mttbar^2\,\done\Yttbar\,\done^2\widetilde{P}_{t}^{\perp}\; \frac{\theta(M_\ttbar-\Mttbar^\text{min})} {\Mttbar^3\;|\widetilde{P}^z_{t}|}} \int{\done^2\bTvec}\,J_{0}(\bT\qT)\, \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]} (\bTvec,\Yttbar,\Mttbar,\Omega_t)\,,\hspace*{-20mm}\\ \frac{\done{\sigma^{\mathrm{res}}_{\ttbar}}} {\done \dphittbar} \,=\;& %============================ % memo: noting that \vec{\tau} can point towards either \vec{n}\times\vec{P}^{\bot}_{t} or the opposite % the results should be same for LHC since the beams are symmetric %============================ \changed{ \frac{1}{32\pi^3\,s} \sum_{\kappa,\mathrm{sign}[\widetilde{P}^z_{t} ]} \int\done\Mttbar^2\,\done\Yttbar\,\done^2\widetilde{P}_{t}^{\perp}\; \frac{\theta(M_\ttbar-\Mttbar^\text{min})}{\Mttbar^3}\, \frac{|\widetilde{P}_{t}^{\perp}|}{|\widetilde{P}^z_{t}|}\;}\\ &\hspace*{60mm}\times\; \int{\done b_{\tau}}\, \cos(b_{\tau}\,|\widetilde{P}_{t}^{\perp}|\,\dphittbar)\, \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]} (\vec{b}^{\|}_{\tau},\Yttbar,\Mttbar,\Omega_t)\,,\hspace*{-20mm} \end{split} \end{align} where $\widetilde{P}^z_{t}$ and $\widetilde{P}_{t}^{\perp}$ are the longitudinal and transverse momenta of the top quark measured in the rest frame of the top and antitop pair. \changed{A lower cutoff $\Mttbar^\text{min}$, which was chosen to be $400\,\text{GeV}$ in~\cite{Ju:2022wia}, is introduced avoid any threshold enhanced contributions, thereby ensuring the applicability of HQET. } % $J_0(x)$ represents the zeroth-rank Bessel function. $\vec{b}_{\tau}$ refers to the projected component of the impact parameter $\bTvec$, \begin{align} \bTvec =\vec{b}_{\tau}^{\perp}+ \vec{b}_{\tau}^{\|} \equiv b_{\tau}^{\perp}\vec{\tau}\times\vec{n}+ b_{\tau}\vec{\tau}\,. \end{align} Here $\vec{n}$ stands for a unit vector pointing to one of beam directions in the laboratory reference frame, whilst in calculating $\dphittbar$ distribution, $\vec{\tau}$ is always chosen to be perpendicular to the flight direction of top quark. Before closing this subsection, we want to discuss the choice of the auxiliary scales in Eqs.\ \eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}. Therein, two sets of auxiliary scales $\{\mu_h,\mu_b,\mu_s\}$ and $\{\nu_b,\nu_s\}$ are introduced during the virtuality and rapidity renormalisation in the relevant sectors. An appropriate choice of their values can minimise the logarithmic dependences in the fixed-order functions, and in turn improve the convergence of the resummation. To this end, the following values will be taken by default in this paper~\cite{Chiu:2012ir,Neill:2015roa,Ju:2022wia}, \begin{align}\label{eq:scale:nat:qT_dphi} \begin{split} \mathcal{Q}&=\qT\,,\quad\quad\quad\quad \mu^{\mathrm{def}}_h=\nu^{\mathrm{def}}_{b}=\Mttbar\,,\quad\quad\quad \mu^{\mathrm{def}}_b= \mu^{\mathrm{def}}_s=\nu^{\mathrm{def}}_s= b_0/\bT\,,\\ \mathcal{Q}&=\dphittbar\,,\quad\quad\quad \mu^{\mathrm{def}}_h=\nu^{\mathrm{def}}_{b}=\Mttbar\,,\quad\quad\quad \mu^{\mathrm{def}}_b= \mu^{\mathrm{def}}_s=\nu^{\mathrm{def}}_s= b_0/b_{\tau}\,, \end{split} \end{align} where $b_0=2\exp(-\gamma_{\mathrm{E}})$ with $\gamma_{\mathrm{E}}$ being the Euler constant. With the choice of Eq.~\eqref{eq:scale:nat:qT_dphi}, the evaluation of Eq.~\eqref{eq:methods:res:qT_dphi} can encounter the Landau singularity of the strong coupling $\alpha_s$ during the impact parameter space integration, which we regularise using the cutoff prescription proposed in \cite{Neill:2015roa}. \subsection{\changed{Extending the resummation region -- properties and caveats}} %\subsection{Asymptotic behaviour in the threshold regime \texorpdfstring{$\dEttbar\to0$}{Delta E to 0}} \label{sec:sigma:thr:hqet} In the last subsection, we introduced the resummed \qT\ and \dphittbar\ spectra in the domain where the top and antitop quarks are kinematically well-separated, i.e.\ $\dEttbar\sim\mathcal{O}(m_t)$ or larger. In this regime, thanks to HQET~\cite{Eichten:1989zv, Georgi:1990um,Grinstein:1990mj,Neubert:1993mb}, the (anti)top quark field will not interact with the other particles at leading power accuracy after applying the decoupling transformation \cite{Bauer:2001yt,Beneke:2010da}. In consequence, at least up to leading power, the hard, soft and beam-collinear regions are sufficient to describe the asymptotic behaviour of the $\qT$ and $\dphittbar$ spectra. % , by analogy to the % \qT\ resummation in the Drell-Yan processes \cite{Collins:1984kg, % Becher:2010tm,Bozzi:2010xn,GarciaEchevarria:2011rb, % Becher:2011xn,Banfi:2011dx,Banfi:2011dm,Banfi:2012du,Catani:2015vma, % Scimemi:2017etj,Bizon:2018foh,Bacchetta:2019sam,Bizon:2019zgf, % Becher:2020ugp,Ebert:2020dfc,Re:2021con,Camarda:2021ict,Ju:2021lah, % Camarda:2023dqn,Neumann:2022lft,Moos:2023yfa} and Higgs % production \cite{Belyaev:2005bs, % Bozzi:2005wk,Bozzi:2007pn,Monni:2016ktx,Becher:2020ugp, % Becher:2012yn,Neill:2015roa,Bizon:2017rah, % Chen:2018pzu,Bizon:2018foh,Gutierrez-Reyes:2019rug, % Harlander:2014hya,Billis:2021ecs,Cal:2023mib}. \changed{ We are now interested in exploring the possibility to lift this kinematic restriction, $\theta(M_\ttbar-\Mttbar^\text{min})$, in Eq.~\eqref{eq:methods:res:qT_dphi} and extend the single differential observables $\done\sigma_\ttbar/\done\qT$ and $\done\sigma_\ttbar/\done\Delta\phi_\ttbar$ over the full $\Mttbar$ range. Such an approach is motivated by the anticipation that for top-quark pair production at the LHC at 13\,TeV the kinematic region $\Delta E_\ttbar\sim\mathcal{O}(m_t)$ accounts for the bulk of the total production cross section. Hence, the asymptotic behaviour in the $\qT\to0$ and $\dphittbar\to0$ limits of the unconstrained cross section is expected to be mostly governed by the dynamics in HQET and SCET, in analogy to the methodology used in \cite{Kidonakis:1997gm,Bonciani:1998vc, Kidonakis:2001nj,Ahrens:2010zv,Czakon:2018nun, Broggio:2015lya,Broggio:2016lfj,Broggio:2017kzi, Kulesza:2017ukk,Kulesza:2017jqv,Kulesza:2018tqz, vanBeekveld:2022hty}. } \changed{ Nonetheless, we will discuss in the following the implications of removing the phase space restriction $\Mttbar^\text{min}$ in Eq.~\eqref{eq:methods:res:qT_dphi}. In particular, we will show that the integrand $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$, in particular the amplitudes $\mathcal{C}^{[\kappa]}_{\alpha;\{h_i\}}$ of the hard sector as well as the evolution kernels $\mathbf{V}_{h}^{[\kappa]}$ it comprises, develops power-like divergences $\sim(\alpha_s/\betattbar)^n$ as the Coulomb interactions manifest themselves in the threshold limit as $\dEttbar\to0$, or more conventionally } \begin{equation}\label{eq:defbeta} \betattbar\equiv\sqrt{1-\frac{4m_t^2}{\Mttbar^2}}\to0\,. \end{equation} % %In the last subsection, we introduced the resummed \qT\ and %\dphittbar\ spectra in the domain where the top and antitop %quarks are kinematically well-separated, i.e. %$\dEttbar\sim\mathcal{O}(m_t)$ %or larger. %In this regime, thanks to HQET~\cite{Eichten:1989zv, % Georgi:1990um,Grinstein:1990mj,Neubert:1993mb}, the %(anti)top quark field will not interact with the other particles %at leading power accuracy after applying the decoupling transformation %\cite{Bauer:2001yt,Beneke:2010da}. %In consequence, at least up to leading power, the hard, soft and %beam-collinear regions are sufficient to describe the asymptotic %behaviour of the \qT\ and $\dphittbar$ spectra, by analogy to the %\qT\ resummation in the Drell-Yan processes \cite{Collins:1984kg, % Becher:2010tm,Bozzi:2010xn,GarciaEchevarria:2011rb, % Becher:2011xn,Banfi:2011dx,Banfi:2011dm,Banfi:2012du,Catani:2015vma, % Scimemi:2017etj,Bizon:2018foh,Bacchetta:2019sam,Bizon:2019zgf, % Becher:2020ugp,Ebert:2020dfc,Re:2021con,Camarda:2021ict,Ju:2021lah, % Camarda:2023dqn,Neumann:2022lft,Moos:2023yfa} and Higgs % production \cite{Belyaev:2005bs, % Bozzi:2005wk,Bozzi:2007pn,Monni:2016ktx,Becher:2020ugp, % Becher:2012yn,Neill:2015roa,Bizon:2017rah, % Chen:2018pzu,Bizon:2018foh,Gutierrez-Reyes:2019rug, % Harlander:2014hya,Billis:2021ecs,Cal:2023mib}. %However, this strategy, cannot be employed over the entire %$\ttbar$ production phase space, including regions near %the $\ttbar$ threshold, $\dEttbar\ll m_t$, %rendering the application of Eq.~\eqref{eq:methods:res:qT_dphi} %onto the calculation of the differential observable %$\done\sigma^{\rm{res}}_{\ttbar}/\done\mathcal{Q}$ %beyond \NLL\ invalid. %This is since, starting at \NNLL\ accuracy, the partonic contributions in %Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg} develop quintic %divergences in the threshold limit as $\dEttbar\to0$, or more %conventionally %\begin{equation}\label{eq:defbeta} % \betattbar\equiv\sqrt{1-\frac{4m_t^2}{\Mttbar^2}}\to0\,, %\end{equation} %leading to diverging phase space integrals over $\Mttbar$. %In the following, we will elaborate on this point and its %solution. %We start with an analysis of the asymptotic properties of the %partonic contributions $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$. %As illustrated in Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}, %$\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$ contains %the fixed-order contribution functions %$\mathcal{B}_{n(\nbar)}^{[\kappa]}$, %$\mathcal{S}^{\alpha\beta}_{[\kappa]}$, and %$\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ as well as the evolution kernels %$\mathcal{D}^{\mathrm{res}}_{[\kappa]}$ and %$\mathcal{V}^{[\kappa]}_{\alpha\beta}$. In the following, their %scaling in the threshold limit will be investigated. \subsection*{Beam function and the evolution kernel \texorpdfstring{$\mathcal{D}^{\mathrm{res}}_{[\kappa]}$} {Dres}} As illustrated in Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}, $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$ contains the fixed-order contribution functions $\mathcal{B}_{n(\nbar)}^{[\kappa]}$, $\mathcal{S}^{\alpha\beta}_{[\kappa]}$, and $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ as well as the evolution kernels $\mathcal{D}^{\mathrm{res}}_{[\kappa]}$ and $\mathcal{V}^{[\kappa]}_{\alpha\beta}$. \changed{ Here, we start with an analysis of the threshold limit of the beam sector $\mathcal{B}_{n(\nbar)}^{[\kappa]}$ and the evolution kernel $\mathcal{D}^{\mathrm{res}}_{[\kappa]}$. Given the fact that both are functions of $\Mttbar$, $\Yttbar$, and the magnitude of impact parameters $\bT$ and $b_{\tau}$, taking the threshold limit is straightforward and does not incur any singular behaviour at any perturbative order.% } It follows that, \begin{align} \label{eq:bf:asy:thr} \mathcal{B}_{n(\nbar)}^{[\kappa]} & \xrightarrow[]{\betattbar\to0} \sum_{m=0}^{\infty}\left(\frac{\alpha_s(\mu_b)}{4\pi}\right)^m \underbrace{\mathcal{B}_{n(\nbar),\mathrm{thr}}^{[\kappa],{(m)}}}_{\mathcal{O}(\betattbar^0)} +\,\mathcal{O}(\betattbar)\,,\\ \label{eq:Dexp:asy:thr} \mathcal{D}^{\mathrm{res}}_{[\kappa]}& \xrightarrow[]{\betattbar\to0} \underbrace{\mathcal{D}^{\mathrm{res}}_{\mathrm{thr},[\kappa]}}_{\mathcal{O}(\betattbar^0)} +\,\mathcal{O}(\betattbar)\,. \end{align} Herein, to facilitate the later discussion, the functions $\mathcal{B}_{n(\nbar),\mathrm{thr}}^{[\kappa],{(m)}} $ and $\mathcal{D}^{\mathrm{res}}_{\mathrm{thr},[\kappa]}$, that represent leading contributions of the beam-collinear sector and the cusp evolution kernel in the vicinity of $\Mttbar=2m_t$, respectively, are introduced, with the corresponding scalings indicated in the underbraces. \subsection*{Hard function} Approaching the limit $\betattbar\to0$ can induce a distinct asymptotic behaviour in the hard function $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$. Within the context of the expansion by regions \cite{Beneke:1997zp,Smirnov:2002pj,Smirnov:2012gma,Jantzen:2011nz}, we can perform the asymptotic expansion of $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ in $\betattbar$ via a set of dynamic regions in the loop integrals, which in general includes the hard, collinear, soft, ultrasoft, and Coulomb regions~\cite{Beneke:2010da}. In the following, we will use the soft-collinear effective field theory (SCET) \cite{Bauer:2000ew,Bauer:2000yr,Bauer:2001yt, Beneke:2002ph,Beneke:2002ni} and potential non-relativistic QCD (pNRQCD) \cite{Pineda:1997bj,Brambilla:1999xf,Beneke:1999zr, Beneke:1999qg} frameworks to capture their contributions. At leading power, the SCET and pNRQCD effective Lagrangians can be expressed as \cite{Beneke:2002ph,Beneke:2002ni,Beneke:1999zr, Beneke:1999qg,Kniehl:2002br} \begin{align} \label{eq:L0SCET} \mathcal{L}_{\text{SCET}} &= \bar{\varphi}_n \Big( i n \cdot D_n + i \slashed{D}_{n\perp} \frac{1}{i \nbar \cdot D_n} i \slashed{D}_{n\perp} \Big) \frac{\slashed{\nbar}}{2} \varphi_n -\frac{1}{2} \mathrm{Tr} \Big\{ F^{\mu\nu}_n F_{\mu\nu}^n \Big\} + ( n \leftrightarrow \nbar ) - \frac{1}{2} \mathrm{Tr} \Big\{F^{\mu\nu}_{\text{us}} F_{\mu\nu}^{\text{us}}\Big\}\,, \\ \label{eq:L0pNRQCD} \mathcal{L}_{\text{pNR}} &= \psi^{\dag} \left( i \partial^0 +\frac{\vec{\partial}^2}{2m_t} \right) \psi + \chi^{\dag} \left( i \partial^0 - \frac{\vec{\partial}^2 }{2m_t} \right) \chi - \int \mathrm{d}^3\vec{r} \, \psi^{\dag} T^{a} \psi \big( x^0,\vec{x}+\vec{r} \big) \left( \frac{\alpha_s}{r} \right) \chi^{\dag} T^{a}\chi \big(x^0,\vec{x}\big) \,, \end{align} where $\varphi_{n}$ denotes the collinear quark field, while $F_{n}^{\mu\nu}$ is the collinear gluon field strength tensor. Likewise, $F_{\text{us}}^{\mu\nu}$ represents the field strength tensor for the ultrasoft gluons. $\psi^{\dagger}(\chi)$ stands for the \changed{heavy quark} field creating the (anti)top quark. The $T^a$ are the usual generators of QCD. In writing Eqs.~\eqref{eq:L0SCET} and~\eqref{eq:L0pNRQCD}, the decoupling transformation~\cite{Beneke:2010da} has been carried out on the collinear and heavy quark fields so as to remove all the ultrasoft-collinear and ultrasoft-heavy-quark interactions at leading power, respectively. We are now ready to appraise the leading contribution of $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ at each perturbative order. On the tree level, the leading terms of $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ are determined by the effective Hamiltonian constructed out of the SCET and pNRQCD fields above. To evaluate the amplitudes induced by this Hamiltonian, we match the QCD amplitudes evaluated at the threshold $\Mttbar=2m_t$ onto the effective field theories. During the calculation, we make use of the \texttt{Mathematica} packages \texttt{FeynArts} \cite{Hahn:2000kx}, \texttt{FeynCalc} \cite{Mertig:1990an,Shtabovenko:2016sxi, Shtabovenko:2020gxv}, and \texttt{FeynHelpers} \cite{Shtabovenko:2016whf} to generate the amplitudes for the individual partonic channels and then employ \texttt{FeynOnium} \cite{Brambilla:2020fla} to recast the Dirac spinors of the heavy quarks in terms of Pauli spinors. It follows that, \begin{align} \mathcal{C}^{[\kappa]}_{\alpha,\{h\}}\xrightarrow[]{\betattbar\to0} \sum^{\infty}_{n=0}\,\left(\frac{\alpha_s}{4\pi}\right)^{n+1}\mathcal{C}^{[\kappa],(n)}_{\mathrm{thr},\alpha,\{h\}}+\dots\,, \end{align} where $\mathcal{C}^{[\kappa],(n)}_{\mathrm{thr},\alpha,\{h\}}$ characterises the leading contribution in the threshold domain $\betattbar\to0$ at the $n$-th order. The LO results read, \begin{align} \label{eq:def:Chard:thr:qqb_qbq_gg:LO} \begin{split} \mathcal{C}^{[q_{n}\qbar_{\nbar}],(0)}_{\mathrm{thr},\{h\}}&= \begin{bmatrix} 0& \frac{4\mathrm{i}\sqrt{2}\pi^2}{m^2_t}\left(\xi_{t}^{\dagger}\vec{\sigma}\eta_{\tbar}\right)\!\cdot\!\left(\bar{v}_{\nbar}\vec{\gamma}_{\perp}u_{n}\right)\, \\ \end{bmatrix} ^{\mathbf{T}}\,, \\ \mathcal{C}^{[q_{\nbar}\qbar_{n}],(0)}_{\mathrm{thr},\{h\}}&= \begin{bmatrix} 0& \frac{4\mathrm{i}\sqrt{2}\pi^2}{m^2_t}\left(\xi_{t}^{\dagger}\vec{\sigma}\eta_{\tbar}\right)\!\cdot\!\left(\bar{v}_{{n}}\vec{\gamma}_{\perp}u_{\nbar}\right)\, \\ \end{bmatrix} ^{\mathbf{T}}\,, \\ \mathcal{C}^{[g_{n}g_{\nbar}],(0)}_{\mathrm{thr},\{h\}}&= \begin{bmatrix} -\frac{8\pi^2}{m_t}\sqrt{\frac{2}{3}}\,\xi_{t}^{\dagger}\eta_{\tbar}\,\varepsilon_{\perp}^{\epsilon_n\epsilon_{\nbar}}&0&-\frac{8\pi^2}{m_t}\sqrt{\frac{5}{3}}\,\xi_{t}^{\dagger}\eta_{\tbar}\,\varepsilon_{\perp}^{\epsilon_n\epsilon_{\nbar}} \\ \end{bmatrix} ^{\mathbf{T}}\,. \end{split} \end{align} Here, $\xi^{\changed{\dagger}}_{t}$ and $\eta_{\tbar}$ denote the Pauli spinors for the top and antitop quarks, respectively, \changed{resulting from the quantum field operators $\psi^{\dagger}$ and $\chi$ in Eq.~\eqref{eq:L0pNRQCD} acting on the external states $\langle\ttbar|$, with $\vec{\sigma}$ being a spatial vector consisting of the Pauli matrices.} Similarly, $u_{n(\nbar)}$ and $v_{n(\nbar)}$ denote the Dirac spinors of the incoming massless quark and antiquarks \changed{induced by the collinear field operator $\varphi_n$ in Eq.~\eqref{eq:L0SCET}}, while $\vec{\gamma}_\perp$ is the transverse component of the Dirac matrices. The contraction of the totally antisymmetric tensor and the polarisation vectors is abbreviated to $\varepsilon_{\perp}^{\epsilon_n\epsilon_{\nbar}}\equiv \varepsilon^{\mu\nu\rho\sigma}n_{\mu}\nbar_{\nu} \epsilon_{n,\rho}\epsilon_{\nbar,\sigma}$. \changed{ In writing Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:LO}, the bases $c_{\{a_i\}}^{qq}$ and $c_{\{a_i\}}^{gg}$ in Eq.~\eqref{eq:def:color:basis:qq_gg} are employed to project out the colour states of the hard amplitudes. % We then collect the contribution of each colour configuration in arrays. As shown in Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:LO}, $\mathcal{C}^{[q_{n}\qbar_{\nbar}],(0)}_{\mathrm{thr},\{h\}}$ and $\mathcal{C}^{[q_{\nbar}\qbar_{n}],(0)}_{\mathrm{thr},\{h\}}$ only include the colour-octet contributions as the LO partonic process $q\bar{q}\to\ttbar$ only contains colour-octet $s$-channel diagrams. This differs for $gg\to\ttbar$, where the $s$-channel and $u$-channel diagrams both contribute, leading to the presence of both colour-singlet and color-octet configurations in $\mathcal{C}^{[g_{n}g_{\nbar}],(0)}_{\mathrm{thr},\{h\}}$. } The leading contributions of $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ on the one-loop level is calculated with the amplitudes induced by the time product of the Coulomb vertex in Eq.~\eqref{eq:L0pNRQCD} and the tree-level Hamiltonian. To evaluate the ensuing loop integral, following the method in \cite{Smirnov:2002pj}, the residue theorem is first applied to integrate out the temporal component of the loop momentum, and the integration of the remaining spatial components can be completed via Feynman parameterisation. After removing the IRC poles within the \MSbar scheme \cite{Ferroglia:2009ii}, it yields, \begin{align} \label{eq:def:Chard:thr:qqb_qbq_gg:NLO} \begin{split} \mathcal{C}^{[q_{n}\qbar_{\nbar}],(1)}_{\mathrm{thr},\{h\}}&= \begin{bmatrix} 0 & \frac{4\mathrm{i}\sqrt{2}\pi^2}{m^2_t}\left(\xi_{t}^{\dagger}\vec{\sigma}\eta_{\tbar}\right)\!\cdot\!\left(\bar{v}_{\nbar}\vec{\gamma}_{\perp}u_{n}\right) \left( -\frac{\pi ^2}{6 \betattbar}+\frac{i \pi \Lttbar }{3 \betattbar}\right) \\ \end{bmatrix} ^{\mathbf{T}}\,, \\ \mathcal{C}^{[q_{\nbar}\qbar_{n}],(1)}_{\mathrm{thr},\{h\}}&= \begin{bmatrix} 0 & \frac{4\mathrm{i}\sqrt{2}\pi^2}{m^2_t}\left(\xi_{t}^{\dagger}\vec{\sigma}\eta_{\tbar}\right)\!\cdot\!\left(\bar{v}_{{n}}\vec{\gamma}_{\perp}u_{\nbar}\right)\left( -\frac{\pi ^2}{6 \betattbar}+\frac{i \pi \Lttbar }{3 \betattbar}\right) \\ \end{bmatrix} ^{\mathbf{T}}\,, \\ \mathcal{C}^{[g_{n}g_{\nbar}],(1)}_{\mathrm{thr},\{h\}}&= \begin{bmatrix} -\frac{8\pi^2}{m_t}\sqrt{\frac{2}{3}}\,\xi_{t}^{\dagger}\eta_{\tbar}\,\varepsilon_{\perp}^{\epsilon_n\epsilon_{\nbar}}\left(\frac{4 \pi ^2}{3 \betattbar}-\frac{8 i \pi \Lttbar }{3 \betattbar} \right) & 0 & -\frac{8\pi^2}{m_t}\sqrt{\frac{5}{3}}\,\xi_{t}^{\dagger}\eta_{\tbar}\,\varepsilon_{\perp}^{\epsilon_n\epsilon_{\nbar}} \left( -\frac{\pi ^2}{6 \betattbar}+\frac{i \pi \Lttbar }{3 \betattbar}\right) \\ \end{bmatrix} ^{\mathbf{T}}\,, \end{split} \end{align} where $\Lttbar\equiv\ln\left(\frac{\mu}{2\betattbar m_t}\right)$% \changed{, using an analogous notation to Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:LO}.} We have verified that the logarithmic dependences in Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO} indeed satisfy the RGE suggested in \cite{Becher:2009cu,Ferroglia:2009ii} up to the power corrections \changed{of} $\mathcal{O}(\betattbar^0)$ and also that the non-logarithmic terms of Eq.\ \eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO} reproduce the NLO correction of the imaginary part of the pNRQCD Green function \cite{Beneke:1999qg,Beneke:1999zr,Pineda:2006ri, Beneke:2011mq}. \changed{ Comparing with the LO results of Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:LO}, we observe that the leading-power one-loop corrections of Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO} contain the same colour configurations only. This echoes the colour conservation in the leading-power Coulomb-gluon exchanges but might be broken when adding ultrasoft radiation at subleading power. } At last, it is worth noting that aside from the Coulomb exchanges, it is also possible to consider the collinear and hard contribution to the one-loop amplitude $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$. However, while the hard loop momenta can not generate any threshold enhanced contributions, according to Eq.~\eqref{eq:L0SCET}, the internal collinear propagators can only result in scaleless and thus vanishing loop integrals for on-shell amplitudes. Therefore, in deriving Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO}, we are only concerned with the contributions induced by the Coulomb potential. From Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:LO} and Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO}, we can determine the asymptotic behaviour of $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ in the threshold regime, \begin{align} \label{eq:chard:asy:thr:qq:gg} \mathcal{C}^{[\kappa]}_{\alpha,\{h\}}\xrightarrow[]{\betattbar\to0} \,\left(\frac{\alpha_s}{4\pi}\right)\Bigg\{\underbrace{\mathcal{C}^{[\kappa],(0)}_{\mathrm{thr},\alpha,\{h\}}}_{\sim\mathcal{O}(\betattbar^0)}+ \mathcal{O}(\betattbar)\Bigg\}+\left(\frac{\alpha_s}{4\pi}\right)^2\Bigg\{\underbrace{\mathcal{C}^{[\kappa],(1)}_{\mathrm{thr},\alpha,\{h\}}}_{\sim\mathcal{O}(\beta^{-1}_{\ttbar})}+ \mathcal{O}(\betattbar^0)\Bigg\}\dots\,, \end{align} Here we only present the results up to the one-loop level, which is sufficient for us to analyse the \NNLL\ resummation in $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$. The asymptotic expansion of $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ at the two loop accuracy and beyond can be carried out in an analogous manner, even including higher power correction in $\betattbar$. Further discussion can be found in \cite{Beneke:2009ye,Barnreuther:2013qvf}. \subsection*{Soft function} We now move onto the investigation of the behaviour of the soft function $\mathcal{S}^{\alpha\beta}_{[\kappa]}$ in the limit $\betattbar\to0$. In principle, the threshold limit of the HQET-based soft function could be extracted by comparison with the soft function in pNRQCD. However, due to the fact that HQET and pNRQCD follow a different sequence in performing the UV renormalisation and the asymptotic expansion---the threshold expansion of the soft function in HQET prioritises the UV renormalisation, whilst the soft sector in pNRQCD is derived by the $\betattbar$ expansion in the first place---this kind of comparison has to be delivered on the differential cross section level, rather than mapping the soft sectors between the two directly. One example to demonstrate the non-commutativity can be found in the inclusive soft functions~\cite{Czakon:2013hxa,Wang:2018vgu} for the threshold resummation. With this in mind, we will directly expand the analytic results for $\mathcal{S}^{\alpha\beta}_{[\kappa]}$ in the limit $\betattbar\to0$. Remaining at the \NNLL\ level in $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$, using Eqs.~(\ref{eq:LP:res:qqbar}-\ref{eq:LP:res:gg}), we only require the soft contribution up to the one-loop level, for which the analytic expression have been derived in \cite{Ju:2022wia} with the help of a Mellin-Barnes transformation \cite{Smirnov:1999gc,Tausk:1999vh}. Expanding those renormalised results in the small parameter $\betattbar$, it yields that \begin{align} \label{eq:sf:asy:thr} \mathcal{S}^{\alpha\beta}_{[\kappa]} \xrightarrow[]{\betattbar\to0} \delta^{\alpha\beta}+\left(\frac{\alpha_s}{4\pi}\right)\, \left[\mathcal{S}^{(1),\alpha\beta}_{\mathrm{thr},[\kappa]}+\mathcal{O}(\betattbar)\right]+\mathcal{O}(\alpha^2_s)\dots\,, \end{align} where %\commentWJ{already checked!} \begin{align} \begin{split} \mathcal{S}^{(1),\alpha\beta}_{\mathrm{thr},[q_n\qbar_{\nbar}]}&= \mathcal{S}^{(1),\alpha\beta}_{\mathrm{thr},[q_{\nbar}\qbar_n]}= \begin{bmatrix} \frac{16 L_{\nu } L_{\mathrm{T}}}{3}-\frac{8 L_{\mathrm{T}}^2}{3}-\frac{4 \pi ^2}{9} & 0 \\ 0& \frac{16 L_{\nu } L_{\mathrm{T}}}{3}-\frac{8 L_{\mathrm{T}}^2}{3}+6 L_{\mathrm{T}}-\frac{4 \pi ^2}{9} \end{bmatrix}\,, \\ \mathcal{S}^{(1),\alpha\beta}_{\mathrm{thr},[gg]}&= \begin{bmatrix} 12 L_{\nu } L_{\mathrm{T}}-6 L_{\mathrm{T}}^2-\pi ^2 & 0 &0 \\ 0& 12 L_{\nu } L_{\mathrm{T}}-6 L_{\mathrm{T}}^2+6 L_{\mathrm{T}}-\pi ^2 &0\\ 0& 0 &12 L_{\nu } L_{\mathrm{T}}-6 L_{\mathrm{T}}^2+6 L_{\mathrm{T}}-\pi ^2\\ \end{bmatrix}\,. \end{split} \end{align} Herein, we use the notations $L_{\nu}=\ln[\mu^2/\nu^2]$, $L_{\mathrm{T}}=\ln[\bT^2\mu^2/b_0^2]$, and $b_0=2\exp(-\gamma_{\mathrm{E}})$ with $\gamma_{\mathrm{E}}$ being again the Euler constant. From the results above, it is seen that no threshold enhanced behaviour emerges from the NLO soft function. We can therefore establish, \begin{align} \label{eq:soft:asy:thr:qq:gg} \mathcal{S}^{(1),\alpha\beta}_{\mathrm{thr},[\kappa]}\sim\mathcal{O}(1)\,. \end{align} \subsection*{Evolution kernel $\mathcal{V}^{[\kappa]}_{\alpha\beta}$} Finally, we investigate the behaviour of non-cusp resummation kernel $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ in the vicinity of the threshold. According to the definitions in Eqs.~\eqref{eq:def:Vres:NLL} and \eqref{eq:def:Vres:N2LL}, $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ comprises the exponential of the $\mathbf{r}^{{[\kappa]},(0)}_{h}$ matrices up to \NLL\ accuracy. Starting at \NNLL, however, they are supplemented with additional perturbative correction matrices, $\mathbf{J}^{[\kappa]}$, to accommodate the two-loop non-cusp anomalous dimension \cite{Ferroglia:2009ii,Ferroglia:2009ep}. Hence, the analysis of the threshold behaviour of $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ reduces to the expansion of $\mathbf{r}^{{[\kappa]},(0)}_{h}$, $\mathbf{J}^{[\kappa]}$, and the transformation matrices $\mathbf{R}_{[\kappa]}$ in $\betattbar$. The $\mathbf{r}^{{[\kappa]},(0)}_{h}$ matrices can be constructed from the eigenvalues of the one-loop non-cusp anomalous dimensions $\gamma_h^{[\kappa],(0)}$~\cite{Ferroglia:2009ii,Ferroglia:2009ep}, for which we solve the characteristic equations for the contributing partonic processes using \texttt{Mathematica}. Expanding in $\betattbar$, the leading and subleading power contributions read, \begin{align} \label{eq:rh:thr:exp} \mathbf{r}^{{[\kappa]},(0)}_{h} \xrightarrow[]{\betattbar\to0}\mathbf{r}^{{[\kappa]},(0)}_{h,\mathrm{thr}}+\mathcal{O}(\betattbar)\,, \end{align} where \begin{align} \label{eq:rh:thr:exp:qq_gg} \begin{split} \mathbf{r}^{{[q_n\qbar_{\nbar},\qbar_n{q}_{\nbar}]},(0)}_{h,\mathrm{thr}}=& \begin{bmatrix} -8-\frac{8 i \pi }{3 \betattbar}&0\\ 0&\frac{i \pi }{3 \betattbar}+6 i \pi -14\, \end{bmatrix} \,,\\ \mathbf{r}^{{[g_ng_{\nbar}]},(0)}_{h,\mathrm{thr}}=& \begin{bmatrix} -\frac{46}{3}-\frac{8 i \pi }{3 \betattbar}&0&0\\ 0&-\frac{64}{3}+\frac{i\pi }{3 \betattbar}+6i \pi&0\\ 0&0&-\frac{64}{3}+\frac{i\pi }{3 \betattbar}+6i \pi\\ \end{bmatrix} \,. \end{split} \end{align} Here, all terms suppressed by positive powers of $\betattbar$ are omitted as they are not related to the leading behaviour of the exponential function of Eq.~\eqref{eq:def:Vres:NLL} in the limit $\betattbar\to0$. Of the remaining expression, the threshold-enhanced imaginary parts echo the $\Lttbar$-dependences in Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO}, driven by Coulomb vertex in Eq.~\eqref{eq:L0pNRQCD}. To derive the diagonalisation matrix $\mathbf{R}_{[\kappa]}$, we solve for the eigenvectors of $\gamma_h^{[\kappa],(0)}$ with the diagonal entries of $\mathbf{r}^{{[\kappa]},(0)}_{h}$ and then fill the columns of $\mathbf{R}_{[\kappa]}$ with the resulting eigenvectors in line with the positions of their eigenvalues. There is, however, some arbitrariness involved in the solutions for the eigenvectors themselves. In this work, we require the eigenvectors constructing $\mathbf{R}_{[\kappa]}$ to, at most, be of $\mathcal{O}(\betattbar^0)$ in the threshold domain. Alternative choices of eigenvectors will lead to distinct expressions of $\mathbf{R}_{[\kappa]}$ as well as $\mathbf{J}^{[\kappa]}$, but do not alter the resulting $\mathcal{V}^{[\kappa]}_{\alpha\beta}$. To confirm this, we have compared the non-cusp kernel $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ evaluated by our $\mathbf{R}_{[\kappa]}$ and its inverse matrix with those generated by the program~\texttt{Diag}~\cite{Hahn:2006hr} and the built-in functions in \texttt{Mathematica}, finding numerical agreements in all three partonic channels at both \NLL\ and \NNLL\ accuracy. After carrying out the expansion in $\betattbar$, the leading terms from $\mathbf{R}_{[\kappa]}$ read, \begin{align} \mathbf{R}_{[\kappa]} \xrightarrow[]{\betattbar\to0} \mathbf{R}^{\mathrm{thr}}_{[\kappa]}+\mathcal{O}(\betattbar)\,, \end{align} where \begin{align} \begin{split} \mathbf{R}^{\mathrm{thr}}_{{[q_n\qbar_{\nbar},\qbar_n{q}_{\nbar}]}} = & \begin{bmatrix} 1&0\\ 0&1\, \end{bmatrix} \,,\\ \mathbf{R}_{{[g_ng_{\nbar}]}}^{\mathrm{thr}}=& \begin{bmatrix} 1&0&0\\ 0&1&\mathrm{sign}[\cos(\theta_t)]\\ 0&-\mathrm{sign}[\cos(\theta_t)]&1\\ \end{bmatrix} \,. \end{split} \end{align} Herein, the transformation matrices take diagonal form for the $\kappa=q_n\qbar_{\nbar}$ and $\kappa=\qbar_n{q}_{\nbar}$ channels in the threshold limit, while $\mathbf{R}_{{[g_ng_{\nbar}]}}^{\mathrm{thr}}$ comprises additional off-diagonal entries $\pm\mathrm{sign}[\cos(\theta_t)]$ in the colour-octet blocks. The reason for this phenomenon is that in the quark-antiquark initiated process, the eigenvalues for the one-loop anomalous dimensions differ from each other by $\mathcal{O}(\betattbar^{-1})$, but as for the $\kappa=g_ng_{\nbar}$ case, the eigenvalues accounting for colour-octet projections overlap with each other until $\mathcal{O}(\betattbar)$, which, in solving for their eigenvectors, can bring in additional contributions from the colour-octet blocks and in turn result in the appearances of $\pm\mathrm{sign}[\cos(\theta_t)]$ in $\mathbf{R}_{{[g_ng_{\nbar}]}}^{\mathrm{thr}}$. When applying $\mathbf{R}_{{[g_ng_{\nbar}]}}^{\mathrm{thr}}$ onto the diagonalisation, one encounters a change in sign when the scattering angle $\theta_t$ crosses $\pi/2$. This is caused by the small-$\betattbar$ expansion of the square root operation in the eigenvalues and is associated with the branch cuts therein. Equipped with the above transformation matrices and the two-loop anomalous dimensions~\cite{Ferroglia:2009ii,Ferroglia:2009ep}, we are now able to evaluate and expand the matrix $\mathbf{J}^{[\kappa]}$ via Eq.~\eqref{eq:def:Vres:N2LL:Jmax}, \begin{align} \mathbf{J}^{[\kappa]} \xrightarrow[]{\betattbar\to0} \mathbf{J}^{[\kappa]}_{\mathrm{thr}}+\mathcal{O}(\betattbar^0)\,, \end{align} where \begin{align} \label{eq:Jh:thr:exp:qq_gg} \begin{split} \mathbf{J}_{\mathrm{thr}}^{{[q_n\qbar_{\nbar},\qbar_n{q}_{\nbar}]}} = & \begin{bmatrix} -\frac{220 i \pi }{4761 \beta_\ttbar}&0\\ 0&\frac{55 i \pi }{9522\beta_\ttbar}\, \end{bmatrix} \,,\\ \mathbf{J}_{\mathrm{thr}}^{{[g_ng_{\nbar}]}}=& \begin{bmatrix} -\frac{220 i \pi }{4761 \beta_\ttbar}&0&0\\ 0&\frac{55 i \pi }{9522\beta_\ttbar}&0\\ 0&0&\frac{55 i \pi }{9522\beta_\ttbar}\\ \end{bmatrix} \,. \end{split} \end{align} Akin to Eq.~\eqref{eq:rh:thr:exp:qq_gg}, the expressions for $\mathbf{J}_{\mathrm{thr}}^{[\kappa]}$ contain the power-like divergence in the imaginary parts. Here, we only need to retain the leading singular terms. Substituting the expressions of Eq.~\eqref{eq:rh:thr:exp:qq_gg} into Eqs.~(\ref{eq:def:Vres:NLL}-\ref{eq:def:Vres:N2LL}), we arrive at the leading behaviour of the evolution kernel $\mathbf{V}_h^{[\kappa]}$ in the threshold domain, \begin{align} & \mathbf{V}_h^{[\kappa]} \Bigg|_{\mathrm{NLL}(')} \, \xrightarrow[]{\betattbar\to0}\; \mathbf{V}_{h,\mathrm{thr}}^{[\kappa],(0)} +\mathcal{O}(\betattbar^0) \,, \\ & \mathbf{V}_h^{[\kappa]} \Bigg|_{\mathrm{N}^2\mathrm{LL}(')} \, \xrightarrow[]{\betattbar\to0}\; \mathbf{V}_{h,\mathrm{thr}}^{[\kappa],(1)}+\mathcal{O}(\beta^{-1}_{\ttbar})\,, \end{align} where \begin{align} \label{eq:def:Vres:NLL:thr:qq_gg} \begin{split} &\mathbf{V}_{h,\mathrm{thr}}^{[q_n\qbar_{\nbar},\qbar_n{q}_{\nbar}],(0)} = \begin{bmatrix} \displaystyle\left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{-\frac{12}{23}-\frac{4 \mathrm{i} \pi }{23 \betattbar}}\, &0\\ 0&\displaystyle\left[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{\frac{\mathrm{i} \pi }{46 \betattbar}+\frac{9 \mathrm{i} \pi }{23}-\frac{21}{23}} \end{bmatrix} \,, \\ &\mathbf{V}_{h,\mathrm{thr}}^{[g_ng_{\nbar}],(0)} = \begin{bmatrix} \displaystyle\left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{-1-\frac{4\mathrm{i} \pi }{23 \betattbar} }\, &0&0\\ 0&\displaystyle\left[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{\frac{\mathrm{ i} \pi }{46 \betattbar}+\frac{9 \mathrm{ i} \pi }{23}-\frac{32}{23}}&0\\ 0&0&\displaystyle\left[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{\frac{\mathrm{ i} \pi }{46 \betattbar}+\frac{9 \mathrm{ i} \pi }{23}-\frac{32}{23}}\\ \end{bmatrix} \,, \end{split} \end{align} and \begin{align} \label{eq:def:Vres:N2LL:thr:qq_gg} \begin{split} &\mathbf{V}_{h,\mathrm{thr}}^{[q_n\qbar_{\nbar},\qbar_n{q}_{\nbar}],(1)} = \frac{\alpha_s(\mu_s)\alpha_s(\mu_h)}{\beta^2_{\ttbar}}\,\\ & \begin{bmatrix} \displaystyle \frac{3025}{22667121 } \, \left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{-\frac{12}{23}-\frac{4 \mathrm{i} \pi }{23 \betattbar}}\, &0\\ 0& \displaystyle \frac{3025}{1450695744 } \, \left[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{\frac{\mathrm{i} \pi }{46 \betattbar}+\frac{9 \mathrm{i} \pi }{23}-\frac{21}{23}} \end{bmatrix}\,, \\ &\mathbf{V}_{h,\mathrm{thr}}^{[g_ng_{\nbar}],(1)} = \frac{\alpha_s(\mu_s)\alpha_s(\mu_h)}{\beta^2_{\ttbar}}\,\\ & \begin{bmatrix} \displaystyle \frac{3025}{22667121 } \left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{-1-\frac{4\mathrm{i} \pi }{23 \betattbar} }\, &0&0\\ 0& \displaystyle \frac{3025}{1450695744 } \left[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{\frac{\mathrm{ i} \pi }{46 \betattbar}+\frac{9 \mathrm{ i} \pi }{23}-\frac{32}{23}}&0\\ 0&0& \displaystyle \frac{3025}{1450695744 }\left[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{\frac{\mathrm{ i} \pi }{46 \betattbar}+\frac{9 \mathrm{ i} \pi }{23}-\frac{32}{23}}\\ \end{bmatrix} .\hspace*{-20mm} \end{split} \end{align} Examining the above evolution kernels in detail, we observe an intensely oscillating behaviour in the diagonal entries at \NLL\ as $\betattbar\to0$, which is always bounded from above though and, thus, remains finite. The results at \NNLL\ accuracy, however, exhibits quadratic divergences that factorise from the matrix structure of the evolution kernel. These divergences are induced by the product of pairs of $\mathbf{J}_{\mathrm{thr}}^{[\kappa]}$ matrices, detailed in Eq.\ \eqref{eq:Jh:thr:exp:qq_gg}, when assembled according to Eq.~\eqref{eq:def:Vres:N2LL}. Comparing this result to the exact evolution function of Eqs.\ \eqsref{eq:def:Vres:NLL}{eq:def:Vres:N2LL}, we find that the expressions in Eqs.~\eqsref{eq:def:Vres:NLL:thr:qq_gg}{eq:def:Vres:N2LL:thr:qq_gg} can indeed replicate the desired asymptotic behaviour in the vicinity of $\beta_\ttbar=0$. More details on this numerical assessment can be found in App.~\ref{app:vali:Vthr}. \subsection*{Combined resummation} Summarising the scaling laws in Eqs.~\eqsref{eq:bf:asy:thr}{eq:Dexp:asy:thr}, Eq.~\eqref{eq:chard:asy:thr:qq:gg}, Eq.~\eqref{eq:soft:asy:thr:qq:gg}, and Eqs.~\eqsref{eq:def:Vres:NLL:thr:qq_gg}{eq:def:Vres:N2LL:thr:qq_gg}, we can determine the asymptotic behaviour of $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$ with the help of Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg},\footnote{ Please note that the coefficient functions at the given orders will have to be expanded for the appropriate order counting of the resummed cross section. In particular, $(\mathcal{C}^{[\kappa],(0)}_{\alpha,\{h'\}}+\frac{\alpha_s}{4\pi}\mathcal{C}^{[\kappa],(1)}_{\alpha,\{h'\}})^{\dagger} (\mathcal{C}^{[\kappa],(0)}_{\beta,\{h\}}+\frac{\alpha_s}{4\pi}\mathcal{C}^{[\kappa],(1)}_{\beta,\{h\}}) =\mathcal{C}^{[\kappa],(0),\dagger}_{\alpha,\{h'\}}\mathcal{C}^{[\kappa],(0)}_{\beta,\{h\}} +\frac{\alpha_s}{4\pi}(\mathcal{C}^{[\kappa],(0),\dagger}_{\alpha,\{h'\}}\mathcal{C}^{[\kappa],(1)}_{\beta,\{h\}}+\mathcal{C}^{[\kappa],(1),\dagger}_{\alpha,\{h'\}}\mathcal{C}^{[\kappa],(0)}_{\beta,\{h\}}) +\order(\alpha_s^2)$, etc. } \begin{align} \label{eq:def:sigma:res:NLL:N2LL:thr} \begin{split} \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}\Bigg|_{\NLL}\, \xrightarrow[]{\betattbar\to0}&\; \underbrace{\widetilde{\Sigma}_{\ttbar,\mathrm{thr}}^{\mathrm{res},[\kappa]}\Bigg|_{\NLL}}_{\mathcal{O}(\betattbar^{0})} +\,\mathcal{O}(\betattbar)\,,\\ \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}\Bigg|_{\NNLL}\, \xrightarrow[]{\betattbar\to0}&\; \underbrace{\widetilde{\Sigma}_{\ttbar,\mathrm{thr}}^{\mathrm{res},[\kappa]}\Bigg|_{\NNLL}}_{\mathcal{O}(\betattbar^{-5})} +\,\mathcal{O}(\betattbar^{-4}) \,, \end{split} \end{align} where \begin{align} \label{eq:NLL:res:qq_gg:thr} \begin{split} %%%%%%%%%%%%%%%%%%%%%%%%%%%% %NLL res function in threshold limit: qq \widetilde{\Sigma}_{\ttbar,\mathrm{thr}}^{\mathrm{res},[q^i_{n}\qbar^j_{\nbar}]}\Bigg|_{\mathrm{N}\mathrm{LL} }=&\; % scaling factor \frac{64 \pi ^2 \alpha^2_s(\mu_h) }{9} \, % non-cusp evolutoion \left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)}\right]^{-\frac{42}{23}}\, % cusp evolution \mathcal{D}^{\mathrm{res},(1)}_{\mathrm{thr},[q^i_{n}\qbar^j_{\nbar}]} \, % PDFs f_{q_n^i/N}(\tilde{\eta}_n,\mu_b) \,f_{\qbar_\nbar^j/\bar{N}}(\tilde{\eta}_\nbar,\mu_b) \,, \\[2mm] %%%%%%%%%%%%%%%%%%%%%%%%%%%% %NLL res function in threshold limit: gg \widetilde{\Sigma}_{\ttbar,\mathrm{thr}}^{\mathrm{res},[g_{n}g_{\nbar}]}\Bigg|_{\mathrm{N}\mathrm{LL} }=&\; % non-cusp evolutoion \Bigg\{ \frac{2 \pi ^2\alpha_s^2(\mu_h)}{3} \left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)}\right]^{-2} + \frac{5\pi ^2 \alpha_s^2(\mu_h)}{3}\left[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \right]^{-\frac{64}{23}} \Bigg\} % cusp evolution \\&\times\, \mathcal{D}^{\mathrm{res},(1)}_{\mathrm{thr},[g_{n}g_{\nbar}]}\, % PDFs f_{g/N}(\tilde{\eta}_n,\mu_b) \, f_{g/\bar{N}}(\tilde{\eta}_\nbar,\mu_b) \,, \end{split} \end{align} and \begin{align} \label{eq:N2LL:res:qq_gg:thr} \begin{split} %%%%%%%%%%%%%%%%%%%%%%%%%%%% %N2LL res function in threshold limit: qq \widetilde{\Sigma}_{\ttbar,\mathrm{thr}}^{\mathrm{res},[q^i_{n}\qbar^j_{\nbar}]}\Bigg|_{\mathrm{N}^2\mathrm{LL} }=&\; % scaling factor 1 -\frac{\alpha_s^5(\mu_h) \alpha_s^2(\mu_s) }{\betattbar^5}\, % scaling factor 2 \frac{9150625\,\pi^3}{3551374364050766592} % non-cusp evolutoion \left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)}\right]^{-\frac{42}{23}} % cusp evolution \\&\times\, \mathcal{D}^{\mathrm{res},(2)}_{\mathrm{thr},[q^i_{n}\qbar^j_{\nbar}]}\, % PDFs f_{q_i/N}(\tilde{\eta}_n,\mu_b) \,f_{\qbar_j/\bar{N}}(\tilde{\eta}_\nbar,\mu_b)\,,\hspace*{-20mm} \\[4mm] %%%%%%%%%%%%%%%%%%%%%%%%%%%% %N2LL res function in threshold limit: gg \widetilde{\Sigma}_{\ttbar,\mathrm{thr}}^{\mathrm{res},[g_{n}g_{\nbar}]} \Bigg|_{\mathrm{N}^2\mathrm{LL} }=&\; % scaling factor 1 \frac{\alpha_s^5(\mu_h)\alpha_s^2(\mu_s)}{ \betattbar^5}\, % scaling factor 2 \Bigg\{ \frac{36602500\,\pi^3}{4624185369857769 } \left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)}\right]^{-2} \!\!\!\!\!\! - \frac{45753125\,\pi^3}{75762653099749687296} \left[\frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)}\right]^{-\frac{64}{23}} \!\Bigg\}\hspace*{-20mm}\\ % cusp evolution &\times\, \mathcal{D}^{\mathrm{res},(2)}_{\mathrm{thr},[g_{n}g_{\nbar}]}\, % PDFs f_{g/N}(\tilde{\eta}_n,\mu_b) \, f_{g/\bar{N}}(\tilde{\eta}_\nbar,\mu_b) \,. \end{split} \end{align} Once again, we omit the expression for the $\kappa=\qbar^i_{n}q^j_{\nbar}$ case, for which the results at \NLL\ and \NNLL\ can be derived from the $\kappa=q^i_{n}\qbar^j_{\nbar}$ case by appropriately swapping the labels $n\leftrightarrow \nbar$. In Eqs.~\eqsref{eq:NLL:res:qq_gg:thr}{eq:N2LL:res:qq_gg:thr}, we have introduced the resummation kernels $\mathcal{D}^{\mathrm{res},(1,2)}_{\mathrm{thr},[\kappa]}$ to encode the contribution of Eq.~\eqref{eq:def:Dres} evaluated at threshold, $\Mttbar=2m_t$, with the superscripts $\{1,2\}$ denoting the logarithmic precision. For the \NLL\ results in Eqs.~\eqref{eq:NLL:res:qq_gg:thr}, due to the lack of perturbative corrections to the fixed-order ingredients, the soft function is equal to a unit matrix and the beam functions are reduced to the PDFs with the momentum fractions $\tilde{\eta}_n= {2m_te^{\Yttbar}}/{\sqrt{s}}$ and $\tilde{\eta}_\nbar={2m_te^{-\Yttbar}}/{\sqrt{s}}$. Conversely, evaluating the \NNLL\ expressions of Eq.~\eqref{eq:N2LL:res:qq_gg:thr}, we emphasise that the perturbative corrections, which comprise the hard contributions of Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO} and its complex conjugate as well as their non-cusp evaluations in Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, account for the leading singular behaviour of $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$. Using the results of Eqs.~\eqsref{eq:NLL:res:qq_gg:thr}{eq:N2LL:res:qq_gg:thr}, we note that while the \NLL\ resummation approaches a constant as $\betattbar\to0$, the \NNLL\ results display quintic divergences. To be precise, $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[q^i_{n}\qbar^j_{\nbar}]}$ approaches negative infinity in the limit $\betattbar\to0$, whereas the sign of the threshold limit of $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[g_{n}g_{\nbar}]}$ is subject to the competition between colour-singlet and colour-octet contributions, as shown in the first and second term in the curly brackets of Eq.~\eqref{eq:N2LL:res:qq_gg:thr}, respectively. Under regular LHC conditions and conventional scale definitions, the singlet term is by far dominant, though, inducing a positive overall sign.\footnote{ The difference in magnitude of the prefactors of the singlet and octet coefficients would have to be overcome by an extreme ratio of the strong couplings at the soft and hard scales, necessitating a soft scale choice extremely close to the $\Lambda_\text{QCD}$. } Combining the scalings of Eq.~\eqref{eq:def:sigma:res:NLL:N2LL:thr} with Eqs.~\eqref{eq:methods:res:qT_dphi}, we are able to establish the asymptotic properties of the resummed \qT\ and \dphittbar\ spectra in the threshold domain. We note that the kinematic variables introduce an additional suppression in the limit $\betattbar\to0$, \begin{align}\label{eq:kin:asy:diff:pTt_Mtt} \begin{split} % \done^2 \widetilde{P}_{t}^{\perp} &\sim\mathcal{O}(\beta^2_{\ttbar})\,,\qquad\qquad\qquad | \widetilde{P}_{t}^{\perp}|\sim|\widetilde{P}_{t}^{z} |\sim\mathcal{O}(\beta_\ttbar)\,,\\ % \done M^2_{\ttbar} &=2M^2_{\ttbar}\,\left(\frac{ \betattbar }{1-\beta^2_\ttbar}\right)\done \beta_\ttbar=8\, m_t^2\,\beta_\ttbar\,\done \beta_\ttbar +\dots\,. \end{split} \end{align} This yields, \begin{align}\label{eq:asy:obs:qT_dphi} \begin{split} %======================================================== % \frac{\done^3 \sigma^{\rm{res}}_{\ttbar}}{\done \betattbar\done \Yttbar \done\qT} \,\xrightarrow[]{\betattbar\to0} &\, \underbrace{\beta^2_{\ttbar}}_{\rm{kin}}\, \otimes \, \underbrace{ \Big\{ \overbrace{\mathcal{O}(\betattbar^0) }^{\rm{NLL}} + \overbrace{\mathcal{O}(\beta^{-1}_{\ttbar}) }^{\rm{N}^2\rm{LL}} + \dots \Big\}}_{\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}}\, \otimes \, \underbrace{ \Big\{\overbrace{\mathcal{O}(\betattbar^0) }^{\rm{NLL} } + \overbrace{\mathcal{O}(\beta^{-4}_{\ttbar}) }^{\rm{N}^2\rm{LL} } +\dots \Big\}}_{\mathbf{V}^{[\kappa]}_{h}}\, \otimes\dots\\ \sim&\, \underbrace{\mathcal{O}(\beta^2_{\ttbar}) }_{\rm{NLL}} + \underbrace{\mathcal{O}(\beta^{-3}_{\ttbar}) }_{\rm{N}^2\rm{LL}} + \dots\,,\\ %======================================================== % \frac{\done^3 \sigma^{\rm{res}}_{\ttbar}}{\done \betattbar\done \Yttbar \done\dphi_\ttbar} \,\xrightarrow[]{\betattbar\to0} &\, \underbrace{\beta^3_{\ttbar}}_{\rm{kin}}\, \otimes \, \underbrace{ \Big\{ \overbrace{\mathcal{O}(\betattbar^0) }^{\rm{NLL}} + \overbrace{\mathcal{O}(\beta^{-1}_{\ttbar}) }^{\rm{N}^2\rm{LL}} + \dots \Big\}}_{\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}}\, \otimes \, \underbrace{ \Big\{\overbrace{\mathcal{O}(\betattbar^0) }^{\rm{NLL} } + \overbrace{\mathcal{O}(\beta^{-4}_{\ttbar}) }^{\rm{N}^2\rm{LL} } +\dots \Big\}}_{\mathbf{V}^{[\kappa]}_{h}}\, \otimes\dots\\ \sim&\, \underbrace{\mathcal{O}(\beta^3_{\ttbar}) }_{\rm{NLL}} + \underbrace{\mathcal{O}(\beta^{-2}_{\ttbar}) }_{\rm{N}^2\rm{LL}} + \dots\,. %======================================================== \end{split} \end{align} In the first line of each of the equations in Eq.~\eqref{eq:asy:obs:qT_dphi}, the scalings for the kinematic prefactor, the hard sector, and the non-cusp evolution kernel are spelt out, capturing the asymptotic behaviour of the differential spectra $\done^3\sigma^{\rm{res}}_{\ttbar}/(\done\betattbar\done\Yttbar\done\mathcal{Q})$ up to \NNLL\ accuracy. For simplicity, we omit the scalings from the beam functions, the soft sector, and the diagonal resummation kernel, since (at least) up to \NNLL\ all of them approach a constant in the vicinity of the threshold $\betattbar=0$. The second lines then present the resulting asymptotic behaviour of the \qT\ and \dphittbar\ differential distributions at the logarithmic accuracies of our concern. We observe that both the \qT\ and the \dphittbar\ differential spectra at \NLL\ experience significant kinematic suppression near threshold, whereas at \NNLL, thanks to the Coulomb enhancement from the hard sector and the non-cusp evolution kernel, see Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO} and Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, the behaviour of $\done^3\sigma^{\rm{res}}_{\ttbar}/(\done\betattbar\done\Yttbar\done\qT)$ and $\done^3\sigma^{\rm{res}}_{\ttbar}/(\done\betattbar\done\Yttbar\done\dphittbar)$ reverses and they instead develop cubic and quadratic divergences, respectively. % \changed{ Although the existence of such a divergence has been implied in earlier calculations \cite{Kulesza:2017ukk,Zhu:2012ts, Li:2013mia,Ahrens:2010zv,Alioli:2021ggd}, where additional perturbative expansions were applied to the non-cusp kernel $\mathbf{V}^{[\kappa]}_{h}$ in place of the original solution derived in \cite{Buras:1991jm,Buchalla:1995vs}, Eq.~\eqref{eq:asy:obs:qT_dphi} for the first time presents their specific threshold behaviour. In turn, this finding will help to interpret the limitation of a HQET and SCET based analysis, thereby paving the way for the future combined resummation of Coulomb, soft and collinear corrections.% } \changed{ Further, we want to emphasise that for lack of a resummation of the Coulomb interactions, Eq.~\eqref{eq:asy:obs:qT_dphi} should be interpreted as the threshold limit of a HQET and SCET based resummation, testing the integrability in Eq.~\eqref{eq:methods:res:qT_dphi} over the entire $\ttbar$ production phase space, rather than an implication on a full QCD calculation in this limit. An analysis of the threshold behaviour of a full QCD result invariably necessitates the use of pNRQCD or vNRQCD in its derivation. Finally,} we conclude that the resummation formalism in Eq.~\eqref{eq:methods:res:qT_dphi} \textit{cannot} be straightforwardly applied to evaluate the single differential observables $\done\sigma^{\rm{res}}_{\ttbar}/\done\qT$ and $\done\sigma^{\rm{res}}_{\ttbar}/\done\dphittbar$ beyond \NLL, unless a kinematic constraint on $\betattbar$, or equivalently $\Delta E_\ttbar$ or $\Mttbar$, is put in place to remove the threshold regime from the $\betattbar$ integration. Instead, in the following, we will propose two \changed{\textit{ad hoc}} prescriptions to smoothly and consistently match the well-separated domain $\dEttbar\sim\mathcal{O}(m_t)$ to the threshold region $\dEttbar\ll\Mttbar$ for a generic observable $\done^3\sigma^{\rm{res}}_{\ttbar}/({\done\betattbar\done\Yttbar\done\mathcal{Q}})$. % %From this observation, we conclude that the resummation formalism %in Eq.~\eqref{eq:methods:res:qT_dphi} \textit{cannot} be %straightforwardly applied to evaluate the single differential %observables $\done\sigma^{\rm{res}}_{\ttbar}/\done\qT$ and %$\done\sigma^{\rm{res}}_{\ttbar}/\done\dphittbar$ beyond \NLL, %unless a kinematic constraint on $\betattbar$, or equivalently %$\Delta E_\ttbar$ or $\Mttbar$, is put in place to remove the %threshold regime from the $\betattbar$ integration. %Instead, all threshold enhanced terms can be well accommodated %using a combined resummation of the soft, collinear, and Coulomb %corrections, at the price of introducing a second asymptotic %expansion parameter $\betattbar$, by analogy to the threshold %resummation in $\ttbar$~\cite{Beneke:2010da,Beneke:2011mq, % Piclum:2018ndt} and $\ttbar H$~\cite{Ju:2019lwp} production. % %Further, we note that the scale evolution in presence %of Coulomb vertices~\cite{Beneke:2009ye,Pineda:2000gza} %additionally comprises power suppressed contributions. %Hence, such a combined resummation is generally intricate for %$\done^3\sigma^{\rm{res}}_{\ttbar}/(\done\betattbar\done\Yttbar\done\mathcal{Q})$ %beyond the leading logarithmic order, as the kinematic configuration %in the small \qT\ and \dphittbar\ regime allows for novel collimated %modes along the beam directions in comparison with the soft %resummation in~\cite{Beneke:2010da,Beneke:2011mq,Piclum:2018ndt, % Ju:2019lwp} from which additional types of power suppressed %vertices can be introduced. %In recent years, even though some effort %\cite{Balitsky:2017gis,Balitsky:2020jzt,Balitsky:2021fer, % Balitsky:2017flc,Vladimirov:2021hdn,Ebert:2021jhy, % Gamberg:2022lju,Rodini:2022wic,Rodini:2023plb, % Vladimirov:2023aot,Rodini:2023mnh,Ebert:2018gsn, % Inglis-Whalen:2021bea,Inglis-Whalen:2022vyn} has been %devoted to calculate subleading power contributions to the \qT\ spectrum %in colour-singlet hadroproduction and very recently, %focusing on the NLO result of the Higgs production, an all-power %analysis of the rapidity regularisation and zero-bin subtraction %has been delivered in \cite{Ferrera:2023vsw}, their generalisation %to the colourful heavy partons processes, has %not been systematically addressed yet. %To this end, we will refrain from attempting a Coulomb resummation in this paper. %Instead, in the following, we will propose two prescriptions to %smoothly and consistently match the well-separated domain %$\dEttbar\sim\mathcal{O}(m_t)$ to the threshold region %$\dEttbar\ll\Mttbar$ for a generic observable %$\done^3\sigma^{\rm{res}}_{\ttbar}/({\done\betattbar\done\Yttbar\done\mathcal{Q}})$. % % \subsection{\changed{Prescriptions to extend the resummation region}} %\subsection{Prescriptions for the extrapolation} \label{sec:thr:div:extrap} \subsubsection{D-\changed{prescription}: Resummation with a decomposed Sudakov factor} In order to \changed{sufficiently weaken} the threshold divergences in the evolution kernel $\mathbf{V}_h^{[\kappa]}$, which, according to Eqs.~\eqref{eq:asy:obs:qT_dphi}, constitute the main singular contribution at \NNLL, we introduce a first prescription, dubbed D-\changed{prescription} in the following. We start by analysing the elements of $\mathbf{V}_h^{[\kappa]}$ in the well-separated domain, i.e.\ $\dEttbar\sim\mathcal{O}(m_t)$. As defined in Eq.~\eqref{eq:def:Vres:N2LL}, at \NNLL\ accuracy, $\mathbf{V}_h^{[\kappa]}$ includes the \NLL\ resummation kernel sandwiched between the perturbative corrections $\big(1+\alpha_s(\mu_s)\mathbf{J}^{[\kappa]}/(4\pi)\big)$ and $\big(1-\alpha_s(\mu_h)\mathbf{J}^{[\kappa]}/(4\pi)\big)$. In the region $\dEttbar\sim\mathcal{O}(m_t)$, both correction terms are of a similar magnitude to the non-logarithmic contributions in the hard and soft functions. Therefore, the product of them is expected to be numerically comparable with the \NNNLL\ coefficients. In consequence, during our phenomenological investigation, we can truncate all terms proportional to $\alpha_s(\mu_s)\alpha_s(\mu_h)$ in Eq.~\eqref{eq:def:Vres:N2LL}, at the cost of additional non-logarithmic corrections in the well-separated domain, yielding \begin{align}\label{eq:def:Vres:N2LL:Dec} & \mathbf{V}_h^{[\kappa]} (v_t,v_{\tbar}, \mu_s,\mu_h)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}}= \sum_{n_s,n_h=0}^{n_s+n_h=1}\,\left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^{n_s}\left(\frac{\alpha_s(\mu_h)}{4\pi}\right)^{n_h}\mathbf{V}_h^{[\kappa],(n_s,n_h)} (v_t,v_{\tbar}, \mu_s,\mu_h)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}}\,, \end{align} where \begin{align} \label{eq:def:Vres:N2LL:Dec:00:10:01} \begin{split} % \label{eq:def:Vres:N2LL:Dec:00} \mathbf{V}_h^{[\kappa],(0,0)} (v_t,v_{\tbar}, \mu_s,\mu_h)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}} \,=\,&\mathbf{R}^{-1}_{[\kappa]}\, \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\} \mathbf{R}_{[\kappa]}\,=\,\mathbf{V}_h^{[\kappa]} (v_t,v_{\tbar}, \mu_s,\mu_h)\Bigg|_{\mathrm{NLL}},\\ % \label{eq:def:Vres:N2LL:Dec:10} \mathbf{V}_h^{[\kappa],(1,0)} (v_t,v_{\tbar}, \mu_s,\mu_h)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}} \,=\,& \mathbf{R}^{-1}_{[\kappa]}\, \mathbf{J}^{[\kappa]}\, \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \mathbf{R}_{[\kappa]}\,, \\ % \label{eq:def:Vres:N2LL:Dec:01} \mathbf{V}_h^{[\kappa],(0,1)} (v_t,v_{\tbar}, \mu_s,\mu_h)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}} \,=\, &\,-\, \mathbf{R}^{-1}_{[\kappa]}\, \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \mathbf{J}^{[\kappa]}\, \mathbf{R}_{[\kappa]}\,. \end{split} \end{align} Herein, we have decomposed the original evolution kernel of Eq.~\eqref{eq:def:Vres:N2LL} according to their $\alpha_s(\mu_s)$ and $\alpha_s(\mu_h)$ powers. The leading order contribution $\mathbf{V}_h^{[\kappa],(0,0)}$ contains no perturbative corrections and thus coincides with the \NLL\ Sudakov factor in Eq.~\eqref{eq:def:Vres:NLL}, while starting from $\mathbf{V}_h^{[\kappa],(1,0)}$ and $\mathbf{V}_h^{[\kappa],(0,1)}$ perturbative corrections encoded in the $\mathbf{J}^{[\kappa]}$ enter. To facilitate our discussion and comparison below, we will refer to the results in Eq.~\eqref{eq:def:Vres:N2LL:Dec} as the non-cusp evolution kernel evaluated in the decomposed \changed{prescription} (D-\changed{prescription}), i.e.\ \NNLLD. It is worth noting that the non-cusp evolution evaluated in the D-\changed{prescription} cannot precisely satisfy the hard RGE as its original form in Eq.~\eqref{eq:def:Vres:N2LL} did \changed{at \NNLL. This can be confirmed by taking the derivative of Eq.~\eqref{eq:def:Vres:N2LL:Dec} with respect to $\ln\mu_s$. It follows that \begin{equation}\label{eq:diff:Vh:N2LLD} \begin{split} \lefteqn{ \frac{\partial}{\partial \ln\mu_s}\mathbf{V}_h^{[\kappa]} (v_t,v_{\tbar},\mu_s,\mu_h)\Bigg|_{\NNLLD} = \beta\big(\alpha_s(\mu_s)\big)\,\frac{\partial}{\partial \alpha_s(\mu_s)} \mathbf{V}_h^{[\kappa]}(v_t,v_{\tbar},\mu_s,\mu_h)\Bigg|_{\NNLLD} }\\ =&\, \beta\big(\alpha_s(\mu_s)\big)\, \mathbf{R}^{-1}_{[\kappa]} \bigg[ -\frac{1}{\alpha_s(\mu_s)}\frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2 \beta_0}+\frac{ \mathbf{J}^{[\kappa]}}{4\pi}-\frac{ \mathbf{J}^{[\kappa]}}{4\pi}\frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2 \beta_0}\bigg] \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \mathbf{R}_{[\kappa]}\\ & +\,\beta\big(\alpha_s(\mu_s)\big)\, \mathbf{R}^{-1}_{[\kappa]} \bigg[ \frac{1}{\alpha_s(\mu_s)}\frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2 \beta_0}\bigg] \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \frac{\alpha_s(\mu_h)}{4\pi}\mathbf{J}^{[\kappa]}\, \mathbf{R}_{[\kappa]}\,. \end{split} \end{equation} According to the definition in Eq.~\eqref{eq:def:Vres:N2LL:Jmax}, $\mathbf{J}^{[\kappa]}$ fulfills the identity, \begin{align} \label{eq:id:Jh:N2LL} \mathbf{J}^{[\kappa]}\left(\mathbf{I}- \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2 \beta_0}\right)=\frac{\beta_1 }{2\beta_0^2}\mathbf{r}^{[\kappa],(0)}_{h}-\frac{\mathbf{r}^{[\kappa],(1)}_{h}}{2\beta_0}-\frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2 \beta_0}\mathbf{J}^{[\kappa]}\,. \end{align} Reinserting this relation back to Eq.~\eqref{eq:diff:Vh:N2LLD} gives \begin{align}\label{eq:diff:Vh:N2LLD2} &\frac{\partial}{\partial \ln\mu_s}\mathbf{V}_h^{[\kappa]} (v_t,v_{\tbar}, \mu_s,\mu_h)\Bigg|_{\NNLLD}\nnb\\ =&\, \mathbf{R}^{-1}_{[\kappa]} \Bigg\{ \bigg[\frac{\alpha_s(\mu_s)}{4\pi}\mathbf{r}^{[\kappa],(0)}_{h}+\left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^{\!2}\!\!\mathbf{r}^{[\kappa],(1)}_{h}+ \mathcal{O}(\alpha_s^3)\bigg] \bigg[\mathbf{I}+\frac{\alpha_s(\mu_s)}{4\pi}\mathbf{J}^{[\kappa]}\bigg] \Bigg\}\, \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \mathbf{R}_{[\kappa]}\nnb\\ & -\mathbf{R}^{-1}_{[\kappa]} \Bigg\{ \frac{\alpha_s(\mu_s)}{4\pi}\mathbf{r}^{[\kappa],(0)}_{h} + \mathcal{O}(\alpha_s^2) \Bigg\}\, \exp\bigg\{ \frac{\mathbf{r}^{[\kappa],(0)}_{h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\}\, \frac{\alpha_s(\mu_h)}{4\pi}\mathbf{J}^{[\kappa]}\, \mathbf{R}_{[\kappa]}\,, \end{align} where we have expanded the QCD beta function in $\alpha_s(\mu_s)$. In this result we observe that while the expression in the second line meets the \NNLL\ RGE of the hard sector, up to perturbative corrections of $\sim\mathcal{O}(\alpha_s^3)$, which is given by differentiating Eq.~\eqref{eq:def:Vres:N2LL} with respect to $\ln\mu_s$, yielding \begin{align} \label{eq:diff:Vh:N2LL} &\frac{\partial}{\partial \ln\mu_s}\mathbf{V}_h^{[\kappa]} = \mathbf{R}^{-1}_{[\kappa]} \bigg[\frac{\alpha_s(\mu_s)}{4\pi}\mathbf{r}^{[\kappa],(0)}_{h}+\left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^2\mathbf{r}^{[\kappa],(1)}_{h}+ \mathcal{O}(\alpha_s^3)\bigg] \mathbf{R}_{[\kappa]}\, \mathbf{V}_h^{[\kappa]} \,, \end{align} an additional contribution enters in the third line. This additional term takes a form similar to the \NLL\ evolution equation, spoiling the \NNLL\ accuracy of $\mathbf{V}_h^{[\kappa]}|_{\NNLLD}$. In view of this difference, the decomposition of Eq.~\eqref{eq:def:Vres:N2LL:Dec} should be interpreted as an \textit{ad hoc} prescription to diminish the divergence in the threshold limit rather than an exact solution of the hard RGE. } %Hence, the decomposition of Eq.~\eqref{eq:def:Vres:N2LL:Dec} should be only regarded as one possible \changed{prescription} to extrapolate the resummation of Eqs.~\eqref{eq:LP:res:qqbar} and \eqref{eq:LP:res:gg} to the full phase space including the threshold region. An analogous decomposition should also be applied to the other partonic functions in Eqs.~\eqref{eq:LP:res:qqbar} and \eqref{eq:LP:res:gg} to remove the combined contributions from different fixed-order ingredients, giving \begin{align} \label{eq:LP:res:qqbar:gg:Dec} \begin{split} % \label{eq:LP:res:qqbar:Dec} &\hspace*{-5mm} \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[q^i_{n}\qbar^j_{\nbar}]} (\bTvec,\Yttbar, \Mttbar,\Omega_t)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}} \,\\ \,=&\; \left(\frac{1}{2N_c}\right)^2\, \mathcal{D}^{\mathrm{res}}_{[q^i_{n}\qbar^j_{\nbar}]} (\bT,\Mttbar,\mu_h,\mu_b,\mu_s,\nu_b,\nu_s)\\ &\times \sum_{\{n_i,n_i',n_i'',n_i'''\}}\, \left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^{n_s+n'_s+n''_s}\, \left(\frac{\alpha_s(\mu_b)}{4\pi}\right)^{n_b+n_b'}\, \left(\frac{\alpha_s(\mu_h)}{4\pi}\right)^{n_h+n'_h+n''_h+n'''_h}\\ &\hspace*{20mm}\times \mathcal{B}_{n}^{[q_n^i],(n_b)}(\eta_n,\bT,\mu_b,\nu_b)\, \mathcal{B}_{\nbar}^{[\qbar_\nbar^j],(n'_b)}(\eta_{\nbar},\bT,\mu_b,\nu_b) \,\\ &\hspace*{20mm}\times \sum_{\{\alpha,\beta,h\}} \Bigg\{ \mathcal{S}^{\alpha_1\beta_1}_{[q_{n}\qbar_{\nbar}],(n_s)} (\bTvec,v_{t},v_{\tbar},\mu_s,\nu_s) \left[ \mathcal{V}^{[q_{n}\qbar_{\nbar}],(n'_s,n'_h)}_{\alpha_1\alpha_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}^{[q^i_{n}\qbar^j_{\nbar}],(n_h)}_{\alpha_2;h_nh_{\nbar}h_th_{\tbar}} \right]^*\\[-4mm] &\hspace*{80mm}\times \left[ \mathcal{V}^{[q_{n}\qbar_{\nbar}],(n''_s,n''_h)}_{\beta_1\beta_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}_{\beta_2;h_nh_{\nbar}h_th_{\tbar}}^{[q^i_{n}\qbar^j_{\nbar}],(n_h''') }\, \right] \Bigg\}\\ &\hspace*{20mm}\times \theta\Big[1-\left(n_h+n'_h+n''_h+n'''_h\right)-\left(n_s+n'_s+n''_s\right)-\left(n_b+n_b'\right)\Big]\,, \\[2mm] % \label{eq:LP:res:gg:Dec} &\hspace*{-5mm} \widetilde{\Sigma}_{\ttbar }^{\mathrm{res},[g_{n}g_{\nbar}]} (\bTvec,\Yttbar, \Mttbar,\Omega_t)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}} \,\\ \,=&\; \left(\frac{1}{N^2_c-1}\right)^2\, \mathcal{D}^{\mathrm{res}}_{[g_{n}g_{\nbar}]} (\bT,\Mttbar,\mu_h,\mu_b,\mu_s,\nu_b,\nu_s)\\ &\times \sum_{\{n_i,n_i',n_i'',n_i'''\}}\, \left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^{n_s+n'_s+n''_s}\, \left(\frac{\alpha_s(\mu_b)}{4\pi}\right)^{n_b+n_b'}\, \left(\frac{\alpha_s(\mu_h)}{4\pi}\right)^{n_h+n'_h+n''_h+n'''_h}\\ &\hspace*{20mm}\times \sum_{\{\alpha,\beta, h,h'\}} \Bigg\{ \mathcal{S}^{\alpha_1\beta_1}_{[g_ng_{\nbar}],(n_s)}(\bTvec,v_{t},v_{\tbar},\mu_s,\nu_s)\, \mathcal{B}^{[g_n],(n_b)}_{n,h_n'{h_n}}(\eta_n,\bTvec,\mu_b,\nu_b)\, \mathcal{B}^{[g_{\nbar}],(n'_b)}_{\nbar,h_{\nbar}'{h_{\nbar}}}(\eta_{\nbar},\bTvec,\mu_b,\nu_b)\\ &\hspace*{40mm}\times \left[ \mathcal{V}^{[g_{n}g_{\nbar}],(n'_s,n'_h)}_{\alpha_1\alpha_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}^{[g_{n}g_{\nbar}],(n_h)}_{\alpha_2;h'_nh'_{\nbar}h_th_{\tbar}} \right]^*\\ &\hspace*{40mm}\times \left[ \mathcal{V}^{[g_{n}g_{\nbar}],(n''_s,n''_h)}_{\beta_1\beta_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}_{\beta_2;h_nh_{\nbar}h_th_{\tbar}}^{[g_ng_{\nbar}],(n'''_h)} \right] \Bigg\}\\ &\hspace*{20mm}\times \theta\Big[1-\left(n_h+n'_h+n''_h+n'''_h\right)-\left(n_s+n'_s+n''_s\right)-\left(n_b+n_b'\right)\Big], \end{split}\hspace*{-20mm} \end{align} where the Heaviside function $\theta(x)$ is introduced with $\theta(x)=1$ for $x\ge0$ and $\theta(x)=0$ otherwise. The $\mathcal{V}^{[\kappa],(n_s,n_h)}_{\alpha\beta}$ refers to the element in the non-cusp resummation kernel of Eq.~\eqref{eq:def:Vres:N2LL:Dec} at index $\{\alpha,\beta\}$. The perturbative expansion of the fixed-order coefficient functions is defined as, \begin{align} \begin{split} \mathcal{S}^{\alpha\beta}_{[\kappa]}=\sum_{n_s=0}^{\infty}\left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^{n_s}\mathcal{S}^{\alpha\beta}_{[\kappa],(n_s)}\,,\\ \mathcal{C}^{[\kappa]}_{\alpha,\{h\}}=\sum_{n_h=0}^{\infty}\left(\frac{\alpha_s(\mu_h)}{4\pi}\right)^{n_h+1}\mathcal{C}^{[\kappa],(n_h)}_{\alpha,\{h\}}\,,\\ \mathcal{B}_{n(\nbar)}^{[\kappa]}=\sum_{n_b=0}^{\infty}\left(\frac{\alpha_s(\mu_b)}{4\pi}\right)^{n_b}\mathcal{B}_{n(\nbar)}^{[\kappa],(n_b)}\,. \end{split} \end{align} The asymptotic behaviour of Eqs.~\eqref{eq:LP:res:qqbar:gg:Dec} in the threshold limit $\betattbar\to0$ can be obtained by repeating the expansion procedure of Sec.~\ref{sec:sigma:thr:hqet}. Analysing the fixed order constituents, as demonstrated in Eq.~\eqref{eq:bf:asy:thr}, \eqref{eq:chard:asy:thr:qq:gg}, and \eqref{eq:soft:asy:thr:qq:gg}, the soft and beam-collinear functions approach a constant in the limit $\betattbar\to0$ up to \NLO, while a power like divergence of $\order(\betattbar^{-1})$ still emerges from the \NLO\ hard sector as a result of the Coulomb interaction. As for the evolution kernels, the diagonal entries $\mathcal{D}^{\mathrm{res}}_{[\kappa]}$ continue to be regular in the threshold domain, see Eq.~\eqref{eq:Dexp:asy:thr}, while the singular behaviour of the non-cusp kernel $\mathbf{V}_h$ is now reduced by one power of $\betattbar$ after the decomposition in Eq.~\eqref{eq:def:Vres:N2LL:Dec}, according to the scaling rules of Eq.~\eqsref{eq:rh:thr:exp}{eq:Jh:thr:exp:qq_gg}, i.e.\ \begin{align} \label{eq:LP:res:Dec:thr:betam1} \mathbf{V}_h^{[\kappa]}\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}}\sim \mathcal{O}(\beta^{-1}_{\ttbar})\,. \end{align} In summary, we arrive at, \begin{align}\label{eq:LP:res:Dec:thr} \lim_{\betattbar\to0}\widetilde{\Sigma}_{\ttbar }^{\mathrm{res},[\kappa]}\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{D}}}\sim\mathcal{O}\left(\betattbar^{-1}\right)\,. \end{align} In comparison with Eq.~\eqref{eq:def:sigma:res:NLL:N2LL:thr}, the thus defined D-\changed{prescription} reduces the degree of the divergence to $\mathcal{O}(\beta^{-1}_{\ttbar})$, pushing all terms of higher divergence to \NNLLp\ and beyond. Although our resummed cross section still diverges as $\betattbar\to0$, this singularity can be well contained by the kinematical suppression introduced through the phase space element and the observable definition, see Eq.~\eqref{eq:kin:asy:diff:pTt_Mtt}. \changed{Therefore, we can now safely lift the kinematic constraint in Eq.~\eqref{eq:methods:res:qT_dphi} and take into account the full $M_\ttbar$ range in the phase space integral for the single differential observables $\done\sigma^{\rm{res}}_{\ttbar}/\done\qT$ and $\done\sigma^{\rm{res}}_{\ttbar}/\done\Delta\phi_\ttbar$. } At last, we would like to stress that in the previous calculations on the soft \cite{Kulesza:2017ukk} and zero-jettiness \cite{Alioli:2021ggd} resummations, the expansion of the product of the fixed-order contributions and the hard evolution kernels in the strong coupling $\alpha_s$ was already used to remove the Coulomb divergence and thereby accomplish \NNLL\ accurate results. Eqs.~\eqref{eq:LP:res:qqbar:gg:Dec} in our formulation is in fact equivalent to their solution, with the only exception that the soft and beam-collinear sectors were adapted as appropriate to the observables of interest. An analogous \changed{prescription} was also implemented in the \qT\ \cite{Zhu:2012ts, Li:2013mia} and threshold \cite{Ahrens:2010zv} resummation, where, in place of $\alpha_s$, the expansion therein proceeded in the scaling $\lambda_{N}\sim \alpha_s\sim1/\ln(\mu_h/\mu_s)$. This method is equivalent to Eqs.~\eqref{eq:LP:res:qqbar:gg:Dec} of our formulation as well, since, up to \NNLL, the result of the $\lambda_{N}$ expansion can be absorbed into the running of $\alpha_s$. \subsubsection{R-\changed{prescription}: Resummation with a re-exponentiated anomalous dimension} Alternatively, we can also mitigate the threshold singularity of $\mathbf{V}_h^{[\kappa]}$ at \NNLL\ by re-exponentiating the divergent contributions in the anomalous dimension $\gamma^{[\kappa]}_h$. We will call this the R-\changed{prescription} in the following. To accomplish this it is worth noting that, to accommodate the Coulomb enhancement in the threshold domain, it is convenient to organise the perturbative contributions using the parameter $\lambda_{\ttbar}\sim \betattbar\sim\alpha_s$ \cite{Beneke:1999qg,Beneke:1999zr,Pineda:2006ri,Beneke:2011mq}. Even though a systematic resummation of Coulomb, soft, and beam-collinear singularities is not the focus of this paper, in the following we will show that this scaling rule can facilitate the regularisation of the threshold divergence of Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}. Expanding the anomalous dimension $\gamma^{[\kappa]}_h$ up to two-loop level~\cite{Ferroglia:2009ii,Ferroglia:2009ep} in the parameter $\lambda_{\ttbar}$, we arrive at the following power series, \begin{align} \gamma_h^{[\kappa]} \xrightarrow[]{\betattbar\to0} \left(\frac{\alpha_s(\mu)}{4\pi}\right)\gamma_{h,\mathrm{thr}}^{[\kappa],(0)}+\left(\frac{\alpha_s(\mu)}{4\pi}\right)^2\gamma_{h,\mathrm{thr}}^{[\kappa],(1)}+\mathcal{O}(\lambda^2_{\ttbar})\,, \end{align} where \begin{align} \label{eq:def:ad:hard:thr:lo_nlo:qq_gg} \begin{split} % \label{eq:def:ad:hard:thr:lo:qq} \gamma_{h,\mathrm{thr}}^{[q_n\qbar_{\nbar}],(0)}= &\;\gamma_{h,\mathrm{thr}}^{[\qbar_n{q}_{\nbar}],(0)}= \begin{bmatrix} -\frac{8 i \pi }{3 \betattbar} -8& 0 \\ 0& \frac{i \pi }{3 \betattbar}+6 i \pi -14 \end{bmatrix} \,, \\ % \label{eq:def:ad:hard:thr:lo:gg} \gamma_{h,\mathrm{thr}}^{[g_{n}g_{\nbar}],(0)} =& \begin{bmatrix} -\frac{46}{3}-\frac{8 i \pi }{3 \betattbar} & 0&0 \\ 0& \frac{i \pi }{3 \betattbar}+6 i \pi -\frac{64}{3}&0\\ 0&0&\frac{i \pi }{3 \betattbar}+6 i \pi -\frac{64}{3} \end{bmatrix} \,, \\ % \label{eq:def:ad:hard:thr:nlo:qq} \gamma_{h,\mathrm{thr}}^{[q_n\qbar_{\nbar}],(1)}= &\;\gamma_{h,\mathrm{thr}}^{[\qbar_n{q}_{\nbar}],(1)}= \begin{bmatrix} -\frac{344 i \pi }{27 \betattbar}& 0 \\ 0& \frac{43 i \pi }{27 \betattbar} \end{bmatrix} \,, \\ % \label{eq:def:ad:hard:thr:nlo:gg} \gamma_{h,\mathrm{thr}}^{g_{n}g_{\nbar},(1)} =& \begin{bmatrix} -\frac{344 i \pi }{27 \betattbar} & 0&0 \\ 0& \frac{43 i \pi }{27 \betattbar}&0\\ 0&0& \frac{43 i \pi }{27 \betattbar} \end{bmatrix} \,. \end{split} \end{align} Here, while we retain the leading and subleading singular contributions in the one-loop anomalous dimension, only the leading terms are needed in the two loop results, in accordance with our scaling rule. At this point, it is important to note that in the threshold limit all $\gamma^{[\kappa]}_h$ are diagonal up to two-loop order. This allows us to solve the hard RGE for the evolution kernel in the low $\betattbar$ region exactly, \begin{align} \label{eq:def:RGE:ReExp} \frac{\done}{\done\ln\mu}\ln \widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa]} = \gamma_{h,\mathrm{thr}}^{[\kappa]}\,, \end{align} which leads to the results at \NLL\ and \NNLL\ accuracy, \begin{align} \label{eq:def:evo:ReExp:nll_n2ll} \begin{split} % \label{eq:def:evo:ReExp:nll} \widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(0)} \, =&\; \exp\bigg\{ \frac{\gamma^{[\kappa],(0)}_{\mathrm{thr},h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\} \,, \\ % \label{eq:def:evo:ReExp:n2ll} \widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1) } \, =&\; \exp\bigg\{ \frac{\gamma^{[\kappa],(0)}_{\mathrm{thr},h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] -\frac{\alpha_s(\mu_h)-\alpha_s(\mu_s)}{4\pi} \underbrace{ \left(\gamma^{{[\kappa]},(0)}_{h,\mathrm{thr}}\; \frac{\beta_1}{2\beta^2_0} -\frac{ \gamma^{{[\kappa]},(1)}_{h,\mathrm{thr}}} {2\beta_0 }\right)}_{\to\mathbf{J}^{[\kappa]}_{\mathrm{thr}}+\mathcal{O}(\betattbar^0)} \bigg\} \,, \end{split} \end{align} where $\beta_{i}$ stands for the QCD beta function \cite{vanRitbergen:1997va,Czakon:2004bu}. With this result we find that the \NLL\ evolution here can exactly reproduce the leading contributions in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg} which are derived by expanding the analytic expression of Eq.~\eqref{eq:def:Vres:NLL} in the limit $\betattbar\to0$. In particular, at finite \betattbar, where the $\gamma^{[\kappa]}_h$ are in general not diagonal at \NNLL, no closed solutions are available. Hence, approximate solutions are used, for example in Eq.~\eqref{eq:def:Vres:N2LL}, where only the one-loop anomalous dimensions are exponentiated and the logarithmic corrections relevant at \NNLL\ are applied by multiplying $(\mathbf{I}+\frac{\alpha_s(\mu_s)}{4\pi}\mathbf{J}^{[\kappa]})$ and $(\mathbf{I}-\frac{\alpha_s(\mu_h)}{4\pi}\mathbf{J}^{[\kappa]})$, respectively. This structural difference can lead to differences in the asymptotic behaviour between the solutions in Eq.~\eqref{eq:def:evo:ReExp:nll_n2ll} and Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, respectively, in the threshold limit. For instance, the ${\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)}$ of Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg} are directly proportional to the product $\alpha_s(\mu_h)\alpha_s(\mu_s)\big(\mathbf{J}^{[\kappa]}_{\mathrm{thr}}\big)^2$ which, according to Eq.~\eqref{eq:Jh:thr:exp:qq_gg}, develops divergences of $\mathcal{O}(\betattbar^{-2})$ as $\betattbar\to0$. However, as we have now moved all anomalous dimensions into the exponent and owing to the fact that their singular terms reside in the imaginary part only, see Eq.~\eqref{eq:def:ad:hard:thr:lo_nlo:qq_gg}, the $\widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)}$ exhibits oscillatory but finite behaviour in the limit $\betattbar\to0$. We can exploit this improved behaviour to remove the threshold divergences of Eq.~\eqref{eq:def:Vres:N2LL}. Noting that the RGE of Eq.~\eqref{eq:def:RGE:ReExp} is subject to the counting rule $\lambda_{\ttbar}\sim\betattbar\sim\alpha_s$, which is appropriate in the threshold domain but can receive significant power corrections in the well-separated region at large \betattbar, we introduce the following matching procedure, \begin{align} \label{eq:def:Vres:N2LL:Reexp} \mathbf{V}_{h }^{[\kappa] } \Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{R}} } \, =&\; {f}_{\rm{tran}}(\betattbar,c_{\mathrm{thr}} ,r_{\mathrm{thr}})\widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)} \left[ \widetilde{\mathbf{V}}_{h,\mathrm{exp}}^{[\kappa],(1)} \right]^{-1} { \mathbf{V}}_h^{[\kappa]} \Bigg|_{\mathrm{N}^2\mathrm{LL} } +\Big[1-{f}_{\rm{tran}}(\betattbar,c_{\mathrm{thr}} ,r_{\mathrm{thr}})\Big]{ \mathbf{V}}_h^{[\kappa]} \Bigg|_{\mathrm{N}^2\mathrm{LL} }\hspace*{-5mm}, \end{align} where in the first term the matrix $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}^{[\kappa],(1)}$ is used to remove the overlap between $\widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)}$ and $\mathbf{V}_h^{[\kappa]}$. It can be extracted by expanding $\widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)}$ in $\alpha_s(\mu_s)$ and $\alpha_s(\mu_h)$ and retaining all contributions up to \NLO, yielding \begin{align} \label{eq:def:Vres:N2LL:Reexp:exp} \begin{split} \widetilde{\mathbf{V}}_{h,\mathrm{exp}}^{[\kappa],(1)}\,=&\; \bigg[1 +\frac{ \alpha_s(\mu_s)}{4\pi} \left(\gamma^{{[\kappa]},(0)}_{h,\mathrm{thr}}\; \frac{\beta_1}{2\beta^2_0} -\frac{ \gamma^{{[\kappa]},(1)}_{h,\mathrm{thr}}} {2\beta_0 }\right) \bigg]\\ &\hspace*{20mm}\times\, \exp\bigg\{ \frac{\gamma^{[\kappa],(0)}_{\mathrm{thr},h}}{2\beta_0} \ln\bigg[ \frac{\alpha_s(\mu_h)}{\alpha_s(\mu_s)} \bigg] \bigg\} \bigg[1 -\frac{\alpha_s(\mu_h) }{4\pi} \left(\gamma^{{[\kappa]},(0)}_{h,\mathrm{thr}}\; \frac{\beta_1}{2\beta^2_0} -\frac{ \gamma^{{[\kappa]},(1)}_{h,\mathrm{thr}}} {2\beta_0 }\right) \bigg]\,. \end{split} \end{align} Multiplying $\widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)}$ by $[\widetilde{\mathbf{V}}_{h,\mathrm{exp}}^{[\kappa],(1)}]^{-1}$ removes terms of the same perturbative order as those already present in $\mathbf{V}_h^{[\kappa]}$ in Eq.~\eqref{eq:def:Vres:N2LL}, thereby eliminating any double-counting in the matched result. In the limit $\betattbar\to0$, both $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}^{[\kappa],(1)}$ and $\mathbf{V}_h^{[\kappa]}$ approach $\mathbf{V}_{h,\mathrm{thr}}^{[\kappa],(1)}$ of Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, such that the first term of Eq.~\eqref{eq:def:Vres:N2LL:Reexp} is actually dictated by $\widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)}$. Away from the threshold regime, power corrections to Eq.~\eqref{eq:def:RGE:ReExp} become relevant and its solution $\widetilde{\mathbf{V}}_{h,\mathrm{thr}}^{[\kappa],(1)}$ gradually loses its accuracy. Here, we introduce the transition function ${f}_{\rm{tran}}$ to switch off their contribution in the well-separated regime, i.e., \begin{equation} \label{eq:def:ftran} f_{\rm{tran}}({\betattbar},c_{\mathrm{thr}},r_{\mathrm{thr}}) = \begin{cases} 1\,, & \betattbar\le c_{\rm{thr}}-r_{\mathrm{thr}}\,;\\ \displaystyle 1-\frac{(\betattbar-c_{\rm{thr}}+r_{\mathrm{thr}})^2}{2r_{\mathrm{thr}}^2} \,,& c_{\rm{m}}-r_{\mathrm{thr}}<\betattbar\le c_{\rm{thr}}\,;\\ \displaystyle \frac{ (\betattbar-c_{\rm{thr}}-r_{\mathrm{thr}})^2 }{2r_{\mathrm{thr}}^2}\,,& c_{\rm{m}}<\betattbar\le c_{\rm{thr}}+r_{\mathrm{thr}}\,;\\ 0 \,,& c_{\rm{thr}}+r_{\mathrm{thr}}\le \betattbar \,, \end{cases} \end{equation} where the parameters $c_{\rm{thr}}$ and $r_{\mathrm{thr}}$ are introduced to characterize the focal point and the transition radius, respectively. To determine their central values and ranges for the uncertainty estimation for our numerical evaluation in Sec.\ \ref{sec:results}, we compare the numeric values of $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}^{[\kappa],(1)}$ and $\mathbf{V}_h^{[\kappa]}$ to determine the range of validity for the RGE in Eq.~\eqref{eq:def:RGE:ReExp}, for details see App. \ref{app:vali:Vthr}. In consequence, we choose \begin{align}\label{eq:scale:ftran:beta_TT} c^{\mathrm{def}}_{\rm{thr}}&=0.4\,,\quad\quad r^{\mathrm{def}}_{\mathrm{thr}} =0.1\,, \end{align} as our default choices and use the sets \begin{align}\label{eq:scale:ftran:beta_TT:var} \{c_{\rm{thr}},r_{\mathrm{thr}}\}=\{0.35, 0.05\}, \{0.45, 0.15\}\, \end{align} to estimate the theoretical uncertainty associated with our matching procedure. At variance with the D-\changed{prescription} of Eq.~\eqref{eq:def:Vres:N2LL:Dec}, where the Coulomb singular terms are pushed to a higher logarithmic order, Eq.~\eqref{eq:def:Vres:N2LL:Reexp} reduces the threshold divergence by re-exponentiating the \NNLL\ corrections that have been abandoned in the formalism of Eq.~\eqref{eq:def:Vres:N2LL}. To this end, we will call the hereby defined \changed{prescription} the R-\changed{prescription} in the following and label the evolution kernel evaluated via Eq.~\eqref{eq:def:Vres:N2LL:Reexp} with $\mathrm{N}^2\mathrm{LL}_{\mathrm{R}}$. Incorporating Eq.~\eqref{eq:def:Vres:N2LL:Reexp} into Eqs.~\eqref{eq:LP:res:qqbar} and \eqref{eq:LP:res:gg}, we derive the resummed partonic cross section in the R-\changed{prescription}, \begin{align} \label{eq:LP:res:qqbar:gg:Reexp} \begin{split} &\hspace*{-5mm} \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[q^i_{n}\qbar^j_{\nbar}]} (\bTvec,\Yttbar, \Mttbar,\Omega_t)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{R}}} \,\\ \,=&\; \left(\frac{1}{2N_c}\right)^2\, \mathcal{D}^{\mathrm{res}}_{[q^i_{n}\qbar^j_{\nbar}]} (\bT,\Mttbar,\mu_h,\mu_b,\mu_s,\nu_b,\nu_s)\\ &\times \sum_{\{n_i,n_i'\}}\, \left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^{n_s}\, \left(\frac{\alpha_s(\mu_b)}{4\pi}\right)^{n_b+n_b'}\, \left(\frac{\alpha_s(\mu_h)}{4\pi}\right)^{n_h+n'_h}\\ &\hspace*{20mm}\times \mathcal{B}_{n}^{[q_n^i],(n_b)}(\eta_n,\bT,\mu_b,\nu_b)\, \mathcal{B}_{\nbar}^{[\qbar_\nbar^j],(n'_b)}(\eta_{\nbar},\bT,\mu_b,\nu_b) \, \\ &\hspace*{20mm}\times \sum_{\{\alpha,\beta,h\}}\Bigg\{ \mathcal{S}^{\alpha_1\beta_1}_{[q_{n}\qbar_{\nbar}],(n_s)}(\bTvec,v_{t},v_{\tbar},\mu_s,\nu_s) \left[\mathcal{V}^{[q_{n}\qbar_{\nbar}]}_{\alpha_1\alpha_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}^{[q^i_{n}\qbar^j_{\nbar}],(n_h)}_{\alpha_2;h_nh_{\nbar}h_th_{\tbar}} \right]^*\,\\[-4mm] &\hspace*{80mm}{}\times \left[\mathcal{V}^{[q_{n}\qbar_{\nbar}]}_{\beta_1\beta_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}_{\beta_2;h_nh_{\nbar}h_th_{\tbar}}^{[q^i_{n}\qbar^j_{\nbar}],(n_h')}\right] \Bigg\}\\ &\hspace*{20mm}\times \theta\Big(1-n_h\Big)\theta\Big(1-n'_h\Big)\theta\Big(1-n_s\Big)\theta\Big(1-n_b\Big)\theta\Big(1-n_b'\Big)\,, \\[2mm] &\hspace*{-5mm} \widetilde{\Sigma}_{\ttbar }^{\mathrm{res},[g_{n}g_{\nbar}]} (\bTvec,\Yttbar, \Mttbar,\Omega_t)\Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{R}}} \,\\ \,=&\; \left(\frac{1}{N^2_c-1}\right)^2\, \mathcal{D}^{\mathrm{res}}_{[g_{n}g_{\nbar}]} (\bT,\Mttbar,\mu_h,\mu_b,\mu_s,\nu_b,\nu_s)\\ &\times \sum_{\{n_i,n_i'\}}\, \left(\frac{\alpha_s(\mu_s)}{4\pi}\right)^{n_s}\, \left(\frac{\alpha_s(\mu_b)}{4\pi}\right)^{n_b+n_b'}\, \left(\frac{\alpha_s(\mu_h)}{4\pi}\right)^{n_h+n'_h}\\ &\hspace*{20mm}\times \sum_{\{\alpha,\beta, h,h'\}} \Bigg\{ \mathcal{S}^{\alpha_1\beta_1}_{[g_ng_{\nbar}],(n_s)}(\bTvec,v_{t},v_{\tbar},\mu_s,\nu_s)\, \mathcal{B}^{[g_n],(n_b)}_{n,h_n'{h_n}}(\eta_n,\bTvec,\mu_b,\nu_b)\, \mathcal{B}^{[g_{\nbar}],(n'_b)}_{\nbar,h_{\nbar}'{h_{\nbar}}}(\eta_{\nbar},\bTvec,\mu_b,\nu_b)\hspace*{-20mm}\\[-2mm] &\hspace*{40mm}\times\, \left[\mathcal{V}^{[g_{n}g_{\nbar}]}_{\alpha_1\alpha_2}(v_{t},v_{\tbar},\mu_s,\mu_h) \mathcal{C}^{[g_{n}g_{\nbar}],(n_h)}_{\alpha_2;h'_nh'_{\nbar}h_th_{\tbar}}\right]^* \left[\mathcal{V}^{[g_{n}g_{\nbar}]}_{\beta_1\beta_2}(v_{t},v_{\tbar},\mu_s,\mu_h)\, \mathcal{C}_{\beta_2;h_nh_{\nbar}h_th_{\tbar}}^{[g_ng_{\nbar}],(n'_h)}\, \right]\Bigg\}\hspace*{-20mm}\\ &\hspace*{20mm}\times \theta\Big(1-n_h\Big)\theta\Big(1-n'_h\Big)\theta\Big(1-n_s\Big)\theta\Big(1-n_b\Big)\theta\Big(1-n_b'\Big)\,. \end{split} \end{align} Here the perturbative correction in each contribution has been included independently up to NLO, for which the product of the Heaviside step functions $\theta(1-n_i)$ is introduced to impose the boundary condition of the \NNLL-level resummation. Again, $\mathcal{V}^{[\kappa]}_{\alpha\beta}$ denotes the element in the non-cusp resummation kernel of Eq.~\eqref{eq:def:Vres:N2LL:Reexp} at the $\alpha$-th row and $\beta$-th column. Differing from the D-prescription in Eqs.~\eqref{eq:LP:res:qqbar:gg:Dec}, where the product of the NLO fixed-order contributions are pushed to terms of higher logarithmic order, all of those contributions are taken into account in the R-\changed{prescription} of Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}. In principle, if there were no threshold divergences emerging from the NLO non-logarithmic terms, these products could be categorised into the higher logarithmic corrections and should play a numerically minor role in the resummation. However, in light of the Coulomb singularity in Eq.~\eqref{eq:chard:asy:thr:qq:gg} and the threshold enhancement in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg}, the differences in organising the fixed-order correction between the D- and R-\changed{prescription}s can \changed{impact} the \qT\ and \dphittbar\ spectra in the vicinity of $\betattbar=0$ \changed{non-trivially}. \changed{In Sec.~\ref{sec:res:num}, we will make use of this property to test the sensitivity of $\done\sigma_\ttbar/\done\dphi_\ttbar$ and $\done\sigma_\ttbar/\done\qT$ to the treatment of the Coulomb interactions. } Taking the threshold limit $\betattbar\to0$, the only singular contribution in Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp} comes from the perturbative correction to the hard function, Eq.~\eqref{eq:chard:asy:thr:qq:gg}, giving rise to a quadratic divergence in the partonic function, \begin{align} \label{eq:LP:res:Reexp:thr:betam2} \widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]} \Bigg|_{\mathrm{N}^2\mathrm{LL}_{\mathrm{R}}}\xrightarrow[]{\betattbar\to0} \mathcal{O}(\beta^{-2}_{\ttbar})\,. \end{align} In comparison with the corresponding expression in the D-\changed{prescription}, Eq.~\eqref{eq:LP:res:Dec:thr:betam1}, the result in Eq.~\eqref{eq:LP:res:Reexp:thr:betam2} exhibits a stronger divergence in the threshold limit. Nevertheless, this divergence can still be accommodated by the kinematic suppression factors of Eq.~\eqref{eq:kin:asy:diff:pTt_Mtt}, \changed{allowing us to remove the phase space restriction $\Mttbar^\text{min}$ in Eq.~\eqref{eq:methods:res:qT_dphi} when evaluating the single differential observables $\done\sigma^{\rm{res}}_{\ttbar}/\done\qT$ and $\done\sigma^{\rm{res}}_{\ttbar}/\done\dphittbar$. } %extrapolation of $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$ into the threshold domain. %of the leading singular contributions in low $\qT$ $(\dphittbar)$ regime of %Eqs.~\eqref{eq:LP:res:qqbar} and \eqref{eq:LP:res:gg} \subsection{Matching to fixed-order QCD} \label{sec:mat} In the past subsections, we have taken the soft-collinear resummation \changed{for the $\qT$ and $\Delta\phi_\ttbar$ spectra within the well-separated domain $\dEttbar\sim\mathcal{O}(m_t)$ and then extended its coverage over the full $M_\ttbar$ range via two ad hoc prescriptions. During this analysis, we worked at leading-power accuracy, embedding the most singular behaviour as $\qT\to0$ or $\dphittbar\to0$, but systematically neglected higher-power corrections. In the followings, we will restore them in part by matching resummation to a dedicated fixed-order QCD calculation.% } To this end, we introduce a matching procedure between the resummation and the fixed-order QCD calculation, defined through \cite{Banfi:2012jm,Banfi:2012yh,Bizon:2018foh} \begin{equation}\label{eq:def:mat} \begin{split} \cfrac{\done \sigma_{\ttbar}^{\rm{mat}}}{\done \mathcal{Q}} \,\equiv&\; \Bigg\{ \left[ \cfrac{\done\sigma_{\ttbar}^{\rm{res}}}{\done \mathcal{Q}} -\cfrac{\done \sigma_{\ttbar}^{\rm{s}}(\mu_\text{f.o.})} {\done \mathcal{Q}} \right]\, f_{\rm{tran}}({\mathcal{Q}},c_{\mathrm{m}},r_{\mathrm{m}}) +\cfrac{\done \sigma_{\ttbar}^{\rm{s}}(\mu_\text{f.o.})} {\done \mathcal{Q}} \Bigg\}\; \mathcal{R}_{\mathrm{fs}}(\mu_\text{f.o.})\\ =&\; f_{\rm{tran}}({\mathcal{Q}},c_{\mathrm{m}} ,r_{\mathrm{m}})\, \left(\cfrac{\done\sigma_{\ttbar}^{\rm{res}}}{\done \mathcal{Q}}\right)\, \mathcal{R}_{\mathrm{fs}}(\mu_\text{f.o.})\Bigg|_{\mathrm{exp}} +\Big\{ 1-{f}_{\rm{tran}}({\mathcal{Q}},c_{\mathrm{m}} ,r_{\mathrm{m}}) \Big\}\, \cfrac{\done \sigma_{\ttbar}^{\rm{f.o.}}(\mu_\text{f.o.})} {\done \mathcal{Q}} +\dots\,, \end{split} \end{equation} where $\mathcal{Q}\in\{\qT,\Delta\phi_{\ttbar}\}$ stands for the observables of our concern. ${\done\sigma_{\ttbar}^{\rm{res}}}/{\done\mathcal{Q}}$ and ${\done\sigma_{\ttbar}^{\rm{s}}}/{\done\mathcal{Q}}$ represent the resummed differential cross section and its perturbative expansion evaluated at the fixed-order scale $\mu_\text{f.o.}$. The modification factor $\mathcal{R}_{\mathrm{fs}}$ is introduced here to supply the power suppressed contributions that have been discarded in deriving the resummation in Eqs.~\eqref{eq:LP:res:qqbar} and \eqref{eq:LP:res:gg}. It is defined as, \begin{align}\label{eq:def:mat:R} \mathcal{R}_{\mathrm{fs}}(\mu_\text{f.o.}) = \cfrac{{\done\sigma_{\ttbar}^{\mathrm{f.o.}}(\mu_\text{f.o.})}/ {\done\mathcal{Q}}} {{\done\sigma_{\ttbar}^{\mathrm{s}}(\mu_\text{f.o.})}/ {\done\mathcal{Q}}}\,. \end{align} Herein, $\done\sigma_{\ttbar}^{\mathrm{f.o.}}/{\done\mathcal{Q}}$ denotes the fixed-order QCD results at the fixed-order scale $\mu_\text{f.o.}$, which will be appraised by means of the program \Sherpa~\cite{Gleisberg:2003xi,Gleisberg:2008ta, Sherpa:2019gpd,Bothmann:2024wqs}. In calculating $ \mathcal{R}_{\mathrm{fs}}$, it is worth noting that starting from \NNLO, the denominator is not positive definite and exhibits zeros. In this case, we expand $\mathcal{R}_{\mathrm{fs}}$ in $\alpha_s(\mu_\text{f.o.})$ in the second step of Eq.~\eqref{eq:def:mat} following the methodology in \cite{Bizon:2018foh}. Throughout our calculation, we will utilise \begin{align} \label{eq:scale:mat} \mu_\text{f.o.}^{\mathrm{def}}=M_\ttbar \end{align} as our default choice but employ the interval $\mu_\text{f.o.}\in[1/2,2]M_\ttbar$ to estimate the theoretical uncertainty. Again, the transition function $f_{\rm{tran}}$ is employed here to progressively fade out the resummation away from the singular region. $f_{\rm{tran}}$ in Eq.~\eqref{eq:def:mat} formally takes the identical form as in Eq.~\eqref{eq:def:ftran}, only being governed by different arguments $\mathcal{Q}$, $c_{\mathrm{m}}$, and $r_{\mathrm{m}}$ here. The latter two parameters are subject to the range of validity of the leading power approximation, which we determine in Sec.~\ref{sec:results:validation} by comparing ${\done\sigma_{\ttbar}^{\rm{s}}}/{\done\mathcal{Q}}$ and ${\done\sigma_{\ttbar}^{\rm{f.o.}}}/{\done\mathcal{Q}}$. \section{Numerical Results} \label{sec:results} \subsection{Input parameters} \label{sec:results:inputparams} In order to validate and evaluate the expressions for the resummed cross sections of the \qT\ and \dphittbar\ spectra derived in the last section, we need to specify the following input parameters, the top quark mass $m_t$, strong coupling constant $\alpha_s$, and the PDFs. We define the top quark mass in the pole mass scheme, using a value of $m_t=173.4\,\text{GeV}$. This is in line with our adopted UV renormalisation scheme for the hard sector. The strong coupling and the PDFs are evaluated by the \LHAPDF package \cite{Buckley:2014ana,Bothmann:2022thx}, using the \texttt{NNPDF31\_nnlo\_as\_0118}~\cite{NNPDF:2017mvq} PDF set with $\alpha_s(m_Z)=0.118$ in the $n_f=5$ light flavour scheme. The colour- and helicity-dependent amplitudes inherent in the partonic functions of Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}, Eq.~\eqref{eq:LP:res:qqbar:gg:Dec}, and Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}, are evaluated using \Recola~\cite{Actis:2012qn,Actis:2016mpe}, up to \NLO\ accuracy. After their combination with the soft and beam-collinear functions as well as the scale evolution kernels, the resulting resummed cross sections $\widetilde{\Sigma}_{\ttbar}^{\mathrm{res},[\kappa]}$ are integrated over the relevant momentum and impact-parameter spaces using \texttt{Cuba} \cite{Hahn:2004fe,Hahn:2014fua} to give our resummed differential spectra $\done\sigma^{\mathrm{res}}_{\ttbar}/\done\qT$ and $\done\sigma^{\mathrm{res}}_{\ttbar}/\done\dphittbar$. Eventually, we match the resummation onto the fixed-order QCD calculations via Eq.~\eqref{eq:def:mat}. At \NLO, the fixed order contributions comprise only the tree-level amplitudes in the domain $\qT>0$ and $\dphittbar>0$, which can be automatically generated by \Sherpa's \cite{Gleisberg:2003xi,Gleisberg:2008ta,Sherpa:2019gpd,Bothmann:2024wqs} built-in matrix element generator \Amegic~\cite{Krauss:2001iv}. We process its output using \Rivet~\cite{Buckley:2010ar, Bierlich:2019rhm,Bierlich:2024vqo} to extract the observables $\done\sigma^{\mathrm{f.o.}}_{\ttbar}/\done\qT$ and $\done\sigma^{\mathrm{f.o.}}_{\ttbar}/\done\dphittbar$. To calculate the \NNLO\ contributions, \OpenLoops \cite{Cascioli:2011va, Kallweit:2014xda,Buccioni:2017yxi,Buccioni:2019sur} is interfaced with \Sherpa to calculate the renormalised one-loop corrections, which is then combined with the real-emission contribution generated again by~\Amegic within the dipole subtraction framework for single-parton divergences \cite{Catani:1996vz,Catani:2002hc,Gleisberg:2007md, Schonherr:2017qcj}. \subsection{Validation} \label{sec:results:validation} In the following, we confront the fixed-order expansion of the resummation in Eq.~\eqref{eq:methods:res:qT_dphi} with those evaluated in full QCD in order to establish the ability of our approximate calculation to reproduce the exact result in the relevant soft-collinear limits. Before analysing our numerical results in detail, it is worth noting that the expressions in Eq.~\eqref{eq:methods:res:qT_dphi} are applicable in the domain where the top and antitop quarks are well separated from their threshold production region. In this domain we are able to apply SCET$+$HQET to extract the soft and beam-collinear approximation in the low \qT\ and \dphittbar\ regime and thereby exploit the decoupling transformation~\cite{Bauer:2001yt,Beneke:2010da} to accomplish the factorisation in Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}. However, the situation is different in the threshold region where \betattbar\ and $\Delta E_{\ttbar}\to0$. Here, the (Coulomb) potential mode~\cite{Beneke:1997zp} comes into play via virtual gluon exchanges between the heavy partons and therefore Eq.~\eqref{eq:methods:res:qT_dphi} is not directly applicable. To this end, in the analysis below, we divide the phase space into three intervals, the threshold region $\Mttbar\le360\,\text{GeV}$, the transitional region $\Mttbar\in[360,400]\,\text{GeV}$, and the well-separated region $\Mttbar\ge400\,\text{GeV}$. We will use these three regions to examine the quality of the approximate result in the \qT\ and \dphittbar\ spectra, probing into the applicability and limitations of Eq.~\eqref{eq:methods:res:qT_dphi}. %At last, it should be stressed that both schemes to extrapolate %the \qT\ and \dphittbar\ resummations into the threshold regime, %introduced in Eq.~\eqref{eq:LP:res:qqbar:gg:Dec} and %Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}, respectively, %differ, up to \NNLO, from Eq.~\eqref{eq:methods:res:qT_dphi} only %by non-logarithmic contributions and, thus, will not impact the %matching process in Eq.~\eqref{eq:def:mat} and the validation %procedure below. \begin{figure}[t!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_le_360_FixedOrder.pdf} \caption{ } \label{fig:results:val:qT:a} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_360_400_FixedOrder.pdf} \caption{ } \label{fig:results:val:qT:b} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_gtr_400_FixedOrder.pdf} \caption{ } \label{fig:results:val:qT:c} \end{subfigure} \caption{ The transverse momentum spectrum of the \ttbar-pair at fixed-order QCD at \NLO\ and \NNLO\ accuracy in the process $pp\to\ttbar+X$ at $\sqrt{s}=13\,\text{TeV}$ within the intervals $\Mttbar\le 360\,\text{GeV}$ (left), $\Mttbar\in[360,400]\,\text{GeV}$ (centre), and $\Mttbar\ge 400\,\text{GeV}$ (right). The \NLOs\ and \NNLOs\ results encode the leading singular behaviour derived from SCET$+$HQET. } \label{fig:results:val:qT} \end{figure} We begin our analysis with an examination of the transverse momentum spectra of the \ttbar-pair in Fig.~\ref{fig:results:val:qT}, where the differential distributions $\done\sigma_{\ttbar}/\done\qT$ of the SCET$+$HQET approximation are compared to those derived in full QCD. Therein, using cyan and apricot, we show the exact fixed-order full QCD results at \NLO\ and \NNLO, respectively, while the approximations are illustrated in the blue and red, labeled \NLOs\ and \NNLOs\ likewise. During their evaluation, we set the renormalisation and factorisation scales to $\mu_R=\mu_F=\Mttbar$ as our central scale choice and use the interval $\mu_R=\mu_F\in[2,0.5]\,\Mttbar$ to estimate the theoretical uncertainties. We represent the scale uncertainties using corresponding coloured solid and hatched bands. In computing \NNLO\ results, we invariably encounter zeros in both the full QCD and approximate calculations around $\qT\approx3\,\text{to}\,5\,\text{GeV}$, inducing significant Monte-Carlo statistical uncertainties shown via vertical error bars. Please note, that the distributions to the left of the respective zero-crossings are negative and we are therefore showing the absolute values. From the main plots in Fig.~\ref{fig:results:val:qT}, we observe that, up to \NNLO, the asymptotic behaviour of the full QCD calculation is well captured by the leading singular contributions derived using SCET$+$HQET in the low \qT\ domain for all three \Mttbar\ slices, including the scale variations. As \qT\ increases, power corrections progressively corrupt the leading singular approximation and enlarge the discrepancies between \NLO\ and \NLOs, and \NNLO\ and \NNLOs, respectively, with the deviations becoming appreciable only around $\qT\ge 20\,\text{GeV}$. This phenomenon suggests that, up to \NNLO, \changed{the (Coulomb) potential region~\cite{Beneke:1997zp} near the \ttbar\ production threshold does not} incur additional leading singular terms as $\qT\to0$. To make a more quantitative assessment of the leading power approximation, the first (second) subplots of Fig.~\ref{fig:results:val:qT} are devoted to the ratio between \NLOs\ (\NNLOs) and \NLO\ (\NNLO). We observe that with only percent level deviations up to $\qT=20\,\text{GeV}$, the \qT\ spectra derived through SCET$+$HQET manage to describe the asymptotic behaviour of the full QCD results at both \NLO\ and \NNLO\ precisions. Further increase in \qT\ increases the deviations between both approaches as higher-power corrections become increasingly important. Nevertheless, for $\qT\approx50\,\text{GeV}$, the leading power approximation can still account for $80\%$ contribution of the exact differential distributions $\done\sigma_{\ttbar}/\done\qT$. \begin{figure}[t!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_le_360_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:qTwt:a} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_360_400_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:qTwt:b} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_gtr_400_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:qTwt:c} \end{subfigure} \caption{ The weighted transverse momentum spectrum of the \ttbar-pair at fixed-order QCD at \NLO\ and \NNLO\ accuracy in the process $pp\to\ttbar+X$ at $\sqrt{s}=13\,\text{TeV}$ within the intervals $\Mttbar\le 360\,\text{GeV}$ (left), $\Mttbar\in[360,400]\,\text{GeV}$ (centre), and $\Mttbar\ge 400\,\text{GeV}$ (right). The \NLOs\ and \NNLOs\ results encode the leading singular behaviour derived from SCET$+$HQET. } \label{fig:results:val:qTwt} \end{figure} In pursuit of further ascertaining the SCET$+$HQET prediction, we investigate the weighted differential distributions $\done\sigma_{\ttbar}/\done \ln \qT$ in the low $\qT\to 0$ regime, which are expected to observe the power series, \begin{align}\label{eq:AsyExp:qTweighted} \frac{\done{\sigma_{\ttbar}}}{\done \ln \qT} = \qT\,\frac{\done{\sigma_{\ttbar}}}{\done\qT} \,\sim\; \sigma_\ttbar^\text{LO}\, \sum_{m,n}\, \left(\frac{\alpha_s }{4\pi}\right)^m\, \left[\, \underbrace{c^{(0)}_{m,n}\,{\ln^{n}(\qT)}}_{\mathrm{LP}} +\,\underbrace{c^{(1)}_{m,n}\,\qT\ln^{n}(\qT)}_{\mathrm{NLP}} +\,\underbrace{c^{(2)}_{m,n}\,\qT^2 \ln^{n}(\qT)}_{\mathrm{N}^2\mathrm{LP}} +\dots \right]\,, \end{align} where $\sigma_\ttbar^\text{LO}$ is the LO cross section and the $c_{m,n}^{(i)}$ are the coefficients at the respective order of the expansion. The numerical results for $\done\sigma_{\ttbar}/\done\ln\qT$ are presented in Fig.~\ref{fig:results:val:qTwt}. Differing from the findings of Fig.~\ref{fig:results:val:qT}, where acute enhancements are showcased in the low \qT\ region, the asymptotic behaviour in $\done\sigma_{\ttbar}/\done\ln\qT$ is alleviated as compared to that of $\done\sigma_{\ttbar}/\done\qT$ by the application of the weighting factor $\qT$. To examine whether the leading power behaviour can be entirely replicated by Eq.~\eqref{eq:methods:res:qT_dphi}, we exhibit the difference between the full QCD results and the EFT ones in the first and second subgraphs of Fig.~\ref{fig:results:val:qTwt}. At \NLO, their difference declines monotonously as \qT\ decreases in all three \Mttbar\ intervals, demonstrating that the leading power contributions are indeed subtracted by the fixed-order expansion of Eq.~\eqref{eq:methods:res:qT_dphi}. Regarding the interval $\qT\in[0.3,100]~$GeV, analogous scenarios can also be found at \NNLO\ from the bottom subgraphs in Fig.~\ref{fig:results:val:qTwt}, thereby justifying the EFT results from Eq.~\eqref{eq:methods:res:qT_dphi}. However, further decreasing \qT\ incurs non-negligible Monte-Carlo statistical uncertainties, giving rise to deviations between the exact and approximate calculations of up to $\sim\!3$ times the variance estimated there, but still within (sub)percent level relative accuracy w.r.t.\ the magnitude of $\done\sigma_{\ttbar}/\done \ln \qT$. \begin{figure}[t!] \centering \begin{subfigure}{0.42\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_Full_PS_FixedOrder.pdf} \caption{ } \label{fig:results:val:qT:FPS} \end{subfigure} % \begin{subfigure}{0.42\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_qT_tt_Mtt_Full_PS_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:qTwt:FPS} \end{subfigure} \caption{ The transverse momentum (left) and weighted transverse momentum (right) spectra of the \ttbar-pair at fixed-order QCD at \NLO\ and \NNLO\ accuracy in the process $pp\to\ttbar+X$ at $\sqrt{s}=13\,\text{TeV}$ in the full phase space. The \NLOs\ and \NNLOs\ results encode the leading singular behaviour derived from SCET$+$HQET. } \label{fig:results:val:qT:FPS:all} \end{figure} Finally, we exhibit the \qT\ and weighted \qT\ distributions in Fig.~\ref{fig:results:val:qT:FPS:all}, evaluated over the full phase space. Unsurprisingly, the behaviours observed in Fig.~\ref{fig:results:val:qT:FPS} and Fig.~\ref{fig:results:val:qTwt:FPS} closely resemble those found in Fig.~\ref{fig:results:val:qT:c} and Fig.~\ref{fig:results:val:qTwt:c}, respectively, as the slice $\Mttbar\ge400\,\text{GeV}$ accounts for the bulk of contributions in the phase space integrals. With these findings, we are now in a position to determine the coefficients $c_{\mathrm{m}}$ and $r_{\mathrm{m}}$ comprised in the arguments of the transition function $f_{\mathrm{tran}}$ of Eq.~\eqref{eq:def:mat} governing our matching procedure. From the analysis above, we find that for all three invariant-mass slices, the leading power approximation of Eq.~\eqref{eq:methods:res:qT_dphi} is capable of reproducing the asymptotic behaviour of the exact QCD calculation up to $\qT\sim10~$GeV within percent level accuracy. At a level of $\sim\!80\%$ of the full theory, this holds until $\qT\sim50\,\text{GeV}$. In light of this, we will make use of \begin{align}\label{eq:scale:ftran:qT:central} \{c_{\rm{m}},r_{\mathrm{m}}\}&=\{50\,\text{GeV},35\,\text{GeV}\} \end{align} as our default choice during the implementation of the matching procedure. With these parameters, the resummation in Eq.~\eqref{eq:methods:res:qT_dphi} is fully retained until $\qT=15\,\text{GeV}$, after which the transition function $f_{\mathrm{tran}}$ phases out the resummation gradually, reducing it to half its size at $\qT=50\,\text{GeV}$ and completely terminating it at $\qT=85\,\text{GeV}$. In order to estimate the theoretical uncertainties associated with our matching procedure, we adopt the following alternative matching parameters \begin{align} \label{eq:scale:ftran:qT:var} \{c_{\rm{m}},r_{\mathrm{m}}\}&=\{45\,\text{GeV},30\,\text{GeV}\},\;\{55\,\text{GeV},40\,\text{GeV}\} \, \end{align} and construct an envelope of the calculated spectra. \begin{figure}[t!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_le_360_FixedOrder.pdf} \caption{ } \label{fig:results:val:dphi:a} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_360_400_FixedOrder.pdf} \caption{ } \label{fig:results:val:dphi:b} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_gtr_400_FixedOrder.pdf} \caption{ } \label{fig:results:val:dphi:c} \end{subfigure} \caption{ The spectrum of the azimuthal separation of the \ttbar-pair at fixed-order QCD at \NLO\ and \NNLO\ accuracy in the process $pp\to\ttbar+X$ at $\sqrt{s}=13\,\text{TeV}$ within the intervals $\Mttbar\le 360\,\text{GeV}$ (left), $\Mttbar\in[360,400]\,\text{GeV}$ (centre), and $\Mttbar\ge 400\,\text{GeV}$ (right). The \NLOs\ and \NNLOs\ results encode the leading singular behaviour derived from SCET$+$HQET. } \label{fig:results:val:dphi} \end{figure} We now move on to the fixed-order results for the spectra of the azimuthal separation of the top and anti-top, \dphittbar, displayed in Fig.~\ref{fig:results:val:dphi}.\footnote{ It should be noted that the results in Figs.~\ref{fig:results:val:dphi:c} and \ref{fig:results:val:dphiwt:c}, illustrating the region $\Mttbar\ge 400\,\text{GeV}$ have already been evaluated in \cite{Ju:2022wia}. To facilitate the comparison and later discussion, however, we exhibit them here once again.} Akin to the \qT\ spectra in Fig.~\ref{fig:results:val:qT}, the $\done\sigma_{\ttbar}/\done\dphittbar$ in the main plots of Fig.~\ref{fig:results:val:dphi} exhibit a similarly singular behaviour in the low \dphittbar\ domain, at both \NLO\ and \NNLO. However, comparing the exact and approximate results, even though the SCET$+$HQET calculations are able to reproduce the correct asymptotic behaviour in the region $\dphittbar\to 0$ in all three \Mttbar\ slices, the size of the missing power corrections are markedly larger than in the \qT\ case. To be precise, at \NLO, while the SCET$+$HQET approximation agrees with the full QCD result within percent level accuracy below $\qT=10\,\text{GeV}$ in the \qT\ spectra in all three \Mttbar\ regions of Fig.~\ref{fig:results:val:qT}, the \dphittbar\ distributions of Fig.~\ref{fig:results:val:dphi} show a deviation of the EFT-based approximation from the full theory of a few permille around $\dphittbar\sim0.2$ in the $\Mttbar\le 360\,\text{GeV}$ slice, increasing to approximately $5\%$ in $\Mttbar\in[360,400]\,\text{GeV}$, and reaching more than $10\%$ in the interval $\Mttbar\ge 400\,\text{GeV}$. An analogous behaviour can be found in the \NNLO\ results, although the region where the approximate results deviate from the exact one is shifted to slightly higher \dphittbar, around $\dphittbar\sim1$. To interpret this phenomenon, it merits reminding that the derivation of Eq.~\eqref{eq:methods:res:qT_dphi} is subject to an asymptotic expansion of the differential cross section in a given kinematic parameter, for instance, $\lambda_{\mathrm{T}}=\qT/Q_h$ in the $\qT$ spectra and $\lambda_{\tau}=\dphittbar\widetilde{P}_t^{\bot}/Q_h$ in the \dphittbar\ ones, where $Q_h$ represents a hard scale of the similar magnitude to \Mttbar\ and $m_t$. In Fig.~\ref{fig:results:val:qT}, focusing on a constant value of \qT, $\lambda_{\mathrm{T}}$ varies gently as $M_{\ttbar}$ changes when progressing through our three slices since the PDFs effectively suppress contributions from, individually, highly boosted top and antitop quarks. However, the situation for \dphittbar\ in Fig.~\ref{fig:results:val:dphi} is different as $\lambda_{\tau}$ is sensitive to the variable $\widetilde{P}_t^{\bot}$, the transverse momentum of the top quark measured in the rest frame of the \ttbar\ system, and is therefore proportional to \betattbar\ in the threshold domain. In turn, \betattbar\ scales with \Mttbar\ in the left panel, and thus takes the typical values of around $0.2$ for $\Mttbar<360\,\text{GeV}$, rising to values of about $0.5$ for $\Mttbar\in[360,400]\,\text{GeV}$, and ultimately reaching $\betattbar\sim\mathcal{O}(1)$ for $\Mttbar>400\,\text{GeV}$. As a consequence of this additional kinematic suppression upon the expansion parameter $\lambda_{\tau}$, weaker power corrections are observed in Fig.~\ref{fig:results:val:dphi:a} than in Fig.~\ref{fig:results:val:dphi:b}, with the largest power corrections found in Fig.~\ref{fig:results:val:dphi:c}, for constant \dphittbar. \begin{figure}[t!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_le_360_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:dphiwt:a} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_360_400_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:dphiwt:b} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_gtr_400_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:dphiwt:c} \end{subfigure} \caption{ The weighted spectrum of the azimuthal separation of the \ttbar-pair at fixed-order QCD at \NLO\ and \NNLO\ accuracy in the process $pp\to\ttbar+X$ at $\sqrt{s}=13\,\text{TeV}$ within the intervals $\Mttbar\le 360\,\text{GeV}$ (left), $\Mttbar\in[360,400]\,\text{GeV}$ (centre), and $\Mttbar\ge 400\,\text{GeV}$ (right). The \NLOs\ and \NNLOs\ results encode the leading singular behaviour derived from SCET$+$HQET. } \label{fig:results:val:dphiwt} \end{figure} As before, we further assess the quality of the leading power approximation by studying the weighted differential distributions $\done\sigma_{\ttbar}/\done \ln \dphittbar$. They are expected to observe the following power series in the asymptotic domain, \begin{align}\label{eq:AsyExp:dphiweighted} \begin{split} \lefteqn{ \frac{\done{\sigma_{\ttbar}}}{\done \ln \dphittbar} = \dphittbar\,\frac{\done{\sigma_{\ttbar}}}{\done\dphittbar} }\\ & \sim\; \sigma_\ttbar^\text{LO}\, \sum_{m,n}\, \left(\frac{\alpha_s }{4\pi}\right)^m\, \left[\, \underbrace{\tilde{c}^{(0)}_{m,n}\,{\ln^{n}(\dphittbar)}}_{\mathrm{LP}} +\,\underbrace{\tilde{c}^{(1)}_{m,n}\,\dphittbar\ln^{n}(\dphittbar)}_{\mathrm{NLP}} +\,\underbrace{\tilde{c}^{(2)}_{m,n}\,\dphittbar^2 \ln^{n}(\dphittbar)}_{\mathrm{N}^2\mathrm{LP}} +\dots \right]\,, \end{split} \end{align} wherein again $\sigma_\ttbar^\text{LO}$ is the LO cross section and the $\tilde{c}_{m,n}^{(i)}$ are the coefficients at the respective order of the expansion. Numerical results for $\done\sigma_{\ttbar}/\done \ln \dphittbar$ in our three \Mttbar\ slices are displayed in Fig.~\ref{fig:results:val:dphiwt}. From the main plots therein, we find in all three regions that the approximate SCET$+$HQET calculation can reproduce the desired singular behaviour also of the weighted \dphittbar\ spectra of the full QCD calculations at both \NLO\ and \NNLO. Similarly, as illustrated in the middle and bottom subplots of Fig.~\ref{fig:results:val:dphiwt}, their difference progressively decreases as \dphittbar\ decreases from $\dphittbar\sim\mathcal{O}(1)$, until in the $\dphittbar\sim\mathcal{O}(10^{-2})$ non-negligible integration uncertainties are encountered. These observations demonstrate that at least up to \NNLO, the fixed-order expansion of Eq.~\eqref{eq:methods:res:qT_dphi} is able to describe the leading singular contributions of the full theory. \begin{figure}[t!] \centering \begin{subfigure}{0.42\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_Full_PS_FixedOrder.pdf} \caption{ } \label{fig:results:val:dphi:FPS} \end{subfigure} \begin{subfigure}{0.42\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_FO_Mtt_Slice/Diag_pptt_dphi_Mtt_Full_PS_FixedOrder_wt.pdf} \caption{ } \label{fig:results:val:dphiwt:FPS} \end{subfigure} \caption{ The spectrum (left) and weighted spectrum (right) of the azimuthal separation of the \ttbar-pair at fixed-order QCD at \NLO\ and \NNLO\ accuracy in the process $pp\to\ttbar+X$ at $\sqrt{s}=13\,\text{TeV}$ in the full phase space. The \NLOs\ and \NNLOs\ results encode the leading singular behaviour derived from SCET$+$HQET. } \label{fig:results:val:qT:dphi:FPS} \end{figure} Again, in a parallel to our appraisal of the approximate \qT\ spectra, we examine the inclusive \dphittbar\ and weighted \dphittbar\ spectra in Fig.~\ref{fig:results:val:qT:dphi:FPS}. Once again, they effectively reproduce the results for $\Mttbar>400\,\text{GeV}$ as this region carries the bulk of the cross section. With its help we can now determine the coefficients $\tilde{c}_{\mathrm{m}}$ and $\tilde{r}_{\mathrm{m}}$ for the transition function $f_{\mathrm{tran}}$ of Eq.~\eqref{eq:def:mat}, employed to match the resummed \dphittbar\ spectrum to its fixed-order counter-part. Considering that the size of the power corrections in the \dphittbar\ distribution is \Mttbar-dependent, the values of $\tilde{c}_{\mathrm{m}}$ and $\tilde{r}_{\mathrm{m}}$ are chosen differently for each region, i.e., \begin{equation}\label{eq:scale:ftran:dphi:central} \begin{array}{ll} \{\tilde{c}_{\rm{m}},\tilde{r}_{\mathrm{m}}\}&=\{0.5,0.3\}\,, \qquad\qquad \Mttbar\le 360~\mathrm{GeV}\,,\\ \{\tilde{c}_{\rm{m}},\tilde{r}_{\mathrm{m}}\}&=\{0.3,0.2\}\,,\qquad\qquad \Mttbar\ge 360~\mathrm{GeV}\,. \end{array} \end{equation} Therein, in view of the excellent agreement between the approximate and exact results in Fig.~\ref{fig:results:val:dphi:a}, we extend the active range of the soft and collinear resummation in the region $M_{\ttbar}<360\,\text{GeV}$. In consequence, here, the resummation is fully active for $\dphittbar<0.2$ and then will be gradually turned off, being reduced to half its strength at $\dphittbar=0.5$ and eliminated at $\dphittbar=0.8$. Otherwise, a tightened choice of $\tilde{c}_{\mathrm{m}}$ and $\tilde{r}_{\mathrm{m}}$ is made for both other invariant mass domains. Here, the resummation is restricted to the region $\dphittbar<0.1$, reduced to half-value at $\dphittbar=0.3$, and terminated for $\dphittbar>0.5$. To investigate the sensitivity of the final matched \dphittbar\ results to the choice of $f_{\mathrm{tran}}$, we also embed the following alternatives as matching parameters, \begin{equation}\label{eq:scale:ftran:dphi:var} \begin{array}{ll} \{\tilde{c}_{\rm{m}},\tilde{r}_{\mathrm{m}}\}&= \{0.45,0.25\}\,,\{0.55,0.35\}\,, \qquad\qquad \Mttbar\le 360~\mathrm{GeV}\,,\\ \{\tilde{c}_{\rm{m}},\tilde{r}_{\mathrm{m}}\}&= \{0.25,0.15\}\,,\{0.35,0.25\}\,, \qquad\qquad \Mttbar\ge 360~\mathrm{GeV}\,. \end{array} \end{equation} \subsection{Resummation-improved \texorpdfstring{\qT}{qT} and \texorpdfstring{\dphittbar}{dphi} distributions} \label{sec:res:num} In the following, we introduce the resummation-improved \qT\ and \dphittbar\ spectra based on Eq.~\eqref{eq:methods:res:qT_dphi}, including the \changed{threshold region $\betattbar\to0$ by employing two \textit{ad hoc} prescriptions, i.e.\ the D-\changed{prescription} of Eq.~\eqref{eq:LP:res:qqbar:gg:Dec} and the R-\changed{prescription} of Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}. Therein,} as illustrated in Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}, our R(a)GE-based resummation is subject to two sets of auxiliary scales, $\{\mu_h,\mu_b,\mu_s\}$ and $\{\nu_b,\nu_s\}$, characterising the typical scales in the virtuality and rapidity renormalisation, respectively. In addition, the matching procedure of Eq.~\eqref{eq:def:mat}, introduces the fixed-order scale $\mu_\text{f.o.}$. Their default choices are presented in Eq.~\eqref{eq:scale:nat:qT_dphi} and Eq.~\eqref{eq:scale:mat}. To estimate the corresponding theoretical uncertainties, we vary all such scales within the intervals $\mu\in[\tfrac{1}{2},2]\,\mu^{\mathrm{def}}\;(\mu=\mu_h,\mu_s,\mu_b,\mu_\text{f.o})$ and $\nu\in[\tfrac{1}{2},2]\,\nu^{\mathrm{def}}\;(\nu=\nu_s,\nu_b)$. We denote the resulting variation as $\delta_{\mathrm{scale}}$. Furthermore, our matching procedure of Eq.~\eqref{eq:def:mat} also introduces the coefficients $\{c_{\rm{m}},r_{\mathrm{m}}\}$ (for \qT) and $\{\tilde{c}_{\rm{m}},\tilde{r}_{\mathrm{m}}\}$ (for \dphittbar) governing the active range of the soft and beam-collinear resummation. Similarly, while the D-\changed{prescription} does not introduce further parameters, the R-\changed{prescription} involves a second matching, see Eq.~\eqref{eq:def:Vres:N2LL:Reexp}, as it embeds terms to mitigate the threshold singularity in the resummation kernel. Its associated parameters parameters are $\{c_{\rm{thr}},r_{\mathrm{thr}}\}$. Their default choice has been presented in Eqs.~\eqref{eq:scale:ftran:qT:central}, \eqref{eq:scale:ftran:dphi:central}, and \eqref{eq:scale:ftran:beta_TT}, respectively. We estimate the uncertainty of the corresponding matching procedure using alternative matching parameter as defined in Eqs.~\eqref{eq:scale:ftran:qT:var}, \eqref{eq:scale:ftran:dphi:var}, and \eqref{eq:scale:ftran:beta_TT:var}, giving the combined matching uncertainty estimate $\delta_{\mathrm{mat}}$. Finally, both sources of uncertainties, $\delta_{\mathrm{scale}}$ and $\delta_{\mathrm{mat}}$, are combined in quadrature, giving the total uncertainty, \footnote{\changed{% We note here that we have introduced a numerical cutoff into the impact-parameter space integrals of Eq.~\eqref{eq:methods:res:qT_dphi} to evade the QCD Landau divergence \cite{Neill:2015roa}, $\bT^\text{cut}=2\,\text{GeV}^{-1}$. To estimate the uncertainties associated with this choice, we also evaluate \qT\ and \dphittbar\ spectra with the alternatives $\bT^\text{cut}=3\,\text{GeV}^{-1}$ and $\bT^\text{cut}=4\,\text{GeV}^{-1}$. We find the variation generally to be on the permille level, comparable to the statistical error from the Monte-Carlo integration. Therefore, we do not take them into account when calculating $\delta_{\mathrm{tot}}$ here. }} \begin{align} \delta_{\mathrm{tot}}=\sqrt{\delta^2_{\mathrm{mat}}+\delta^2_{\mathrm{scale}}}\;. \end{align} \begin{figure}[t!] \centering \begin{subfigure}{0.42\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_qT_Res_Mul_Mtt_Full_PS.pdf} \caption{ } \label{fig:results:res:qT:dphi:FullPS:a} \end{subfigure} \begin{subfigure}{0.42\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_dphi_Res_Mul_Mtt_Full_PS.pdf} \caption{ } \label{fig:results:res:qT:dphi:FullPS:b} \end{subfigure} \caption{ The resummation-improved \qT\ (left) and \dphittbar\ (right) spectra of the process $pp\to\ttbar+X$ at $\sqrt{s}=13\,\text{TeV}$. } \label{fig:results:res:qT:dphi:FullPS} \end{figure} \changed{With this definition,} we present in Fig.~\ref{fig:results:res:qT:dphi:FullPS} the single differential distributions $\done\sigma_\ttbar/\done\qT$ and $\done\sigma_\ttbar/\done\dphittbar$ over the whole phase space, integrated over all \Mttbar\ values. Therein, the results at \NLLNLO\ \changed{ are calculated from a literal implementation of Eq.~\eqref{eq:methods:res:qT_dphi} since neither the \NLL\ non-cusp evolution kernel $\mathbf{V}_h^{[\kappa]}$ nor the tree-level hard functions $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ induce any singular behaviour in the limit $\betattbar\to0$, and thus no modification of the resummation is required in the threshold regime. These \NLLNLO\ results are depicted in the yellow bands} in Fig.~\ref{fig:results:res:qT:dphi:FullPS:a} (\qT) and \ref{fig:results:res:qT:dphi:FullPS:b} (\dphittbar). \changed{ Comparing the shapes of both distributions, however, we observe that while a classical Sudakov peak is formed in the low \qT\ regime, the \dphittbar\ spectrum grows monotonically as $\dphittbar\to0$. To understand this structural difference, it is worth reminding that although both the \qT\ and \dphittbar\ resummations comprise the same partonic kernels in Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}, which approach constants as \qT\ and \dphittbar\ vanish, the calculation of the \qT\ spectrum invokes an additional factor $\propto\qT$ which is absent in the \dphittbar\ case, see Eq.~\eqref{eq:methods:res:qT_dphi}. In consequence, the resummed \qT\ spectrum experiences kinematical suppression as $\qT\to0$ and in turn develops a Sudakov peak, whereas the \dphittbar\ spectrum does not. } \changed{ At the core of this paper, however, are} the \NNLLDNNLO\ and \NNLLRNNLO\ calculations \changed{shown in the red and cyan in Fig.~\ref{fig:results:res:qT:dphi:FullPS}. They are derived via the \textit{ad hoc} D- and R-prescriptions of Eq.~\eqref{eq:LP:res:qqbar:gg:Dec} and Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}, respectively. It merits recalling that in these prescriptions two fundamentally distinct methods are adopted to address the Coulomb-gluon-induced threshold singularities of Eq.~\eqref{eq:asy:obs:qT_dphi}. While the D-prescription simply shifts them to terms of higher logarithmic order, \NNNLL\ and beyond, see Eq.~\eqref{eq:LP:res:qqbar:gg:Dec}, the R-prescription re-exponentiates the leading Coulomb singularities from the non-cusp kernel $\mathbf{V}_h^{[\kappa]}$ via solving the respective renormalisation group evolution equation in the $\betattbar\to0$ limit, see Eq.~\eqref{eq:def:RGE:ReExp}, and leaves the singularities of the hard scattering amplitudes $\mathcal{C}^{[\kappa]}_{\alpha;\{h\}}$ and their complex conjugate to be cancelled by the respective phase space suppression factors through Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}. Therefore, comparing the results using the D- and R-prescriptions allows us to assess the sensitivity of the \qT\ and \dphittbar\ spectra to the details of how the Coulomb-singular contributions, that are not systematically accommodated by the SCET$+$HQET based resummation in Eq.~\eqref{eq:methods:res:qT_dphi} and can neither be full accessed by scale variations, are addressed. } \changed{ Examining our results in detail, we find that the central value at \NNLLRNNLO\ mostly coincides with that of \NNLLDNNLO\ for the \dphittbar\ spectrum of Fig.\ \ref{fig:results:res:qT:dphi:FullPS:b}, with the uncertainty band of the former being fully contained in that of the latter. Our findings are somewhat different for the \qT\ spectrum of Fig.\ \ref{fig:results:res:qT:dphi:FullPS:a}, however. We observe a difference of around $10\%$ between the \NNLLDNNLO\ and \NNLLRNNLO\ as $\qT\to0$, while both calculations again agree very well for the rest of the spectrum. This difference can be understood from the kinematics in Eqs.~\eqref{eq:methods:res:qT_dphi}, where $\done\sigma_\ttbar/\done\dphittbar$ comprises an additional factor of $|\widetilde{P}_{t}^{\perp}|$ compared to $\done\sigma_\ttbar/\done\qT$. As $\betattbar\to0$, this factor becomes of $\mathcal{O}(\betattbar)$ and effectively removes the threshold contribution that are the main driver of the difference between the D- and R-prescriptions in the phase space integration in the $\dphittbar$ spectrum. Consequently, the well-separated domain, $\Delta E_\ttbar\sim\mathcal{O}(m_t)$ or $\betattbar\sim\order(1)$, dominates the single differential \dphittbar\ spectrum, which leads to the converging uncertainty bands of \NNLLRNNLO\ and \NNLLDNNLO\ and also the proximity of their central values. Nevertheless, the absence of such a dampening factor in \qT\ spectrum emphasises the impact of threshold-enhanced terms in the Coulomb limit, leading to a sizeable dependence on the details of their treatment even after integrating over the entire $\Mttbar$ or $\betattbar$ range.% } \changed{ Given this observation, in order to further improve the description of the \qT\ spectrum, an HQET$+$SCET-only-based analysis will be insufficient to describe the entire phase space for lack of an adequate description of higher-order Coulomb-enhanced terms. To remove any ambiguity caused by the choice of \textit{ad hoc} prescriptions, it will become necessary to develop a combined resummation of the Coulomb, soft, and collinear corrections via SCET$+$pNRQCD (or vNRQCD), at least in the threshold regime. Conversely, the negligible difference between \NNLLRNNLO\ and \NNLLDNNLO\ in the \dphittbar\ spectrum indicates a weaker sensitivity to these Coulomb interactions. Nonetheless, it is worth noting that the inclusion of the threshold regime in Eq.~\eqref{eq:methods:res:qT_dphi} is still subject to \textit{ad hoc} prescriptions to regularise the threshold divergences. We expect that, in this case as well, the introduction of the aforementioned combined resummation will make the application of such prescriptions unnecessary. } % %Ultimately, we present in Fig.~\ref{fig:results:res:qT:dphi:FullPS} %the single differential distributions $\done\sigma_\ttbar/\done\qT$ and %$\done\sigma_\ttbar/\done\dphittbar$ over the whole phase space, integrated %over all \Mttbar\ values. %Therein, the results at \NLLNLO\ in %Fig.~\ref{fig:results:res:qT:dphi:FullPS:a} (\qT) and %\ref{fig:results:res:qT:dphi:FullPS:b} (\dphittbar) are %comparable to those of Fig.~\ref{fig:results:res:qT:cs:c} and %\ref{fig:results:res:dphi:cs:c}, respectively, in both shape %and magnitude, owing to the fact that the interval %$\Mttbar\ge 400\,\text{GeV}$ accounts for the bulk of the cross section. %At \NNLLNNLO\ accuracy, however, whilst the \dphittbar\ distribution %still mostly resembles the one in %Fig.~\ref{fig:results:res:dphi:cs:c}, including the convergence of %both the central value and the uncertainty estimates of the %\NNLLDNNLO\ and \NNLLRNNLO\ calculations in the asymptotic domain, %the \qT\ spectrum exhibits a sensitivity of around $10\%$ to the extrapolation %\changed{prescription} as $\qT\to0$, differing from Fig.~\ref{fig:results:res:qT:cs:c}. %To interpret this, it merits recalling that the threshold limit %$\betattbar\to0$ imposes stronger kinematical restriction on %$\done^2\sigma_\ttbar/(\done\Mttbar\done\dphittbar)$ than on %$\done^2\sigma_\ttbar/(\done\Mttbar\done\qT)$, where the former %experiences an additional kinematic factor of %$|\widetilde{P}_{t}^{\perp}|\sim\mathcal{O}(\betattbar)$ while %there is no such suppression factor for the latter, see %Eqs.~\eqref{eq:methods:res:qT_dphi}. %As a result, during the phase space integration, the contributions %from the threshold region contribute very little to %$\done\sigma_\ttbar/\done\dphittbar$, but still have an %appreciable impact in low \qT\ regime of $\done\sigma_\ttbar/\done\qT$. %% %At last, it is paramount to emphasise that in spite of the %numerical insensitivity of the \dphittbar\ distribution to the %extrapolation prescriptions, implementing the literal resummation %of Eq.~\eqref{eq:methods:res:qT_dphi} onto %$\done\sigma_\ttbar/\done\dphittbar$ is still impossible %without taking care of the divergences in \betattbar\ emerging at \NNLL. %Otherwise, threshold singularities would develop in the limit %$\betattbar\to0$ and in turn leading to a divergent phase space integration, %as elucidated in Eqs.~\eqref{eq:asy:obs:qT_dphi}. % \section{Conclusions} \label{sec:conclusions} % %In this paper we presented the resummation-improved transverse %momentum and, for the first time, azimuthal separation spectra %of the \ttbar-pair at \NNLLNNLO\ accuracy. %In order to include the entire top-antitop production phase space, %ranging from very high invariant $\ttbar$-pair masses, \Mttbar, %down to the production threshold region at $\Mttbar=2m_t$ ($\betattbar=0$), %we isolated the arising threshold singularities at that order %and incorporated them into our resummation formalism. %To address the inherent ambiguities of such a procedure, we %formulated to fundamentally different schemes. %While the D-scheme simply shifts the poles in $1/\betattbar$ to %a higher logarithmic accuracy which is not included here, %the novel R-scheme re-collects such contributions in part and includes them %in the soft-collinear Sudakov form factor. %Their difference is formally of \NNNLL\ %and can be used to estimate %the theoretical uncertainty of the treatment of the %Coulomb singularity. % %In order to analyse the properties and numerical predictions of %our formalism, we investigated the double differential distributions %$\done^2\sigma_\ttbar/(\done\Mttbar\done\qT)$ and %$\done^2\sigma_\ttbar/(\done\Mttbar\done\dphittbar)$. %We found that at large top-pair invariant masses both the D- and %R-scheme give consistent results, agreeing with our expectation %that the \betattbar-dependent non-logarithmic corrections are unimportant %in this region. %Conversely, approaching the threshold region the differences between %both schemes become apparent. %While the D-scheme predicts only slight alterations of the \NLL\ %Sudakov peak in the \qT\ spectrum, the R-scheme shifts the Sudakov %peak to somewhat larger \qT\ at very small \betattbar. %Similar results are found for the \dphittbar\ spectra. %Despite the absence of a Sudakov peak structure, the differences %between both schemes %manifest themselves in lower predicted cross sections in the %R-scheme as both \dphittbar\ and \betattbar\ approach zero. % %Finally, we integrated all invariant mass regions to arrive %at predictions for the single-differential $\done\sigma_\ttbar/\done\qT$ %and $\done\sigma_\ttbar/\done\dphittbar$ distributions. %Their features follow mostly the results calculated far away %from the threshold region, by virtue of their dominance in the %integrated cross section, and show only mild differences between %the D- and R-scheme. %It is noteworthy though, that the \dphittbar\ spectrum experiences %an additional phase space suppression in the threshold limit such %that the Coulomb-gluon affected region plays a smaller role in the %inclusive spectrum than it does for \qT. %Consequently, we found much smaller differences between %both extrapolation schemes in $\done\sigma_\ttbar/\done\dphittbar$. %This suggests that, in comparison to the \qT\ case, the %inclusive \dphittbar\ spectrum is better suited to a pure %soft-collinear resummation, at least up to \NNLLNNLO\ precision. %In bears no mention, though, that $1/\betattbar$ singularities %are present within this integration over the whole invariant %mass range at \NNLLNNLO\ order, and a na\"ive soft-collinear %resummation is not possible without addressing them. %Despite their radical differences, the fact that the predictions %of the D- and R-scheme largely coincide shows the power of %our formalism. % %Ultimately, only a rigorous simultaneous resummation of %both soft-collinear and Coulomb divergences will remove this %scheme dependence and yield reliable predictions throughout %the entire \Mttbar\ range. %We will, however, leave such developments for future work. In this paper we presented the resummation-improved transverse momentum and, for the first time, azimuthal separation spectra of the \ttbar-pair at \NNLLNNLO\ accuracy, \changed{and studied their predictions for top-antitop pair production at the 13\,TeV at the LHC}. \changed{% We based our calculation on the observation that as for such high colliding energies the domain where the top and antitop quarks are kinematically well separated, $\dEttbar\sim\mathcal{O}(m_t)$, dominates the process $pp\to\ttbar+X$ and, therefore, the asymptotic behaviour in the limits $\qT\to0$ and $\dphittbar\to0$ can be mostly captured by the soft and beam-collinear resummation via HQET$+$SCET. We then endeavored to extend this description over the entire phase space, including the threshold regime, $\Delta E_\ttbar\to0$ or $\betattbar\to0$, where the exchange of Coulomb gluons adds new potentially divergent corrections to our process. % Implementing this method at \NLL, however, proved to be straightforward, as the involved functions of the HQET$+$SCET resummation at this accuracy were found to be regular in the threshold limit. Nevertheless, starting from \NNLL, we demonstrated that Coulomb divergences manifest themselves in both the hard function and its non-cusp evolution kernels. This, in turn prohibited a direct application of the soft and collinear resummation result to the entire phase space. } \changed{ In order to address these Coulomb divergences emerging in our soft and collinear resummation, we introduced two \textit{ad hoc} prescriptions, referenced as D- and R-prescriptions, respectively. While the threshold enhanced terms in D-prescription are simply shifted to a higher logarithmic order, they are in part resummed in R-prescription. Here, the leading singular terms induced by the two-loop non-cusp anomalous are re-exponentiated via solving the hard renormalisation group equation as $\betattbar\to0$. %Nonetheless, both prescriptions are, from the viewpoint of the HQET$+$SCET resummation, equivalent, and Comparing their respective predictions allowed us to quantitatively assess the inherent uncertainty of our calculation and the sensitivity of both the \qT\ and \dphittbar\ spectra to Coulomb interactions. } \changed{ Finally, we implemented both prescriptions to calculate $\done\sigma_{t\bar{t}}/\done\dphittbar$ and $\done\sigma_{t\bar{t}}/\done\qT$, with the labelling their predictions \NNLLDNNLO\ and \NNLLRNNLO. We observed that the central values from D- and R-prescriptions mostly coincide in $\done\sigma_{t\bar{t}}/\done\dphittbar$, with the uncertainty band of the latter being fully contained by that of the former. Conversely, we found a deviation of around $10\%$ between both prescriptions as $\qT\to0$ in $\done\sigma_{t\bar{t}}/\done\qT$. This indicates that applying our soft-collinear resummation onto the \qT\ spectrum introduces a non-negligible ambiguity at \NNLL\ in the absence of necessary higher-order contributions from the threshold domain. Therefore, to further improve the theoretical accuracy of the \qT\ spectrum, a combined resummation of Coulomb, soft, and collinear corrections via SCET and pNRQCD (or alternatively vNRQCD) in the threshold regime seems warranted. % Similarly, while the negligible deviation between the D- and R-prescriptions in the \dphittbar\ spectrum indicates a weaker sensitivity to Coulomb interactions, it is worth noting that extending the soft and collinear resummation coverage to the whole \Mttbar\ phase space still necessitates \textit{ad hoc} prescriptions to regularise the arising Coulomb divergences as $\dEttbar\to0$. We expect that a combined resummation will be beneficial in this case as well, removing the need for either prescription. } \subsection*{Acknowledgements} WJ would like to thank Li Lin Yang for sharing valuable details in computing the hard evolution kernel in \cite{Zhu:2012ts,Li:2013mia, Ahrens:2010zv,Ahrens:2011mw}. % WJ is also grateful to Guoxing Wang for the helpful discussion on the threshold soft function in \cite{Wang:2018vgu}. % WJ and MS would also like to express our gratitude to Ben Pecjak for taking the time to respond to our numerous queries. % MS is funded by the Royal Society through a University Research Fellowship (URF\textbackslash{}R1\textbackslash{}180549, URF\textbackslash{}R\textbackslash{}231031) and an Enhancement Award (RGF\textbackslash{}EA\textbackslash{}181033, CEC19\textbackslash{}100349, and RF\textbackslash{}ERE\textbackslash{}210397) as well as the STFC (ST/X003167/1 and ST/X000745/1). \section{\changed{Comparison of D- and R-prescriptions in the double differential distributions}} \begin{figure}[t!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_qT_Res_Mul_Mtt_le_360.pdf} \caption{ } \label{fig:results:res:qT:cs:a} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_qT_Res_Mul_Mtt_360_400.pdf} \caption{ } \label{fig:results:res:qT:cs:b} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_qT_Res_Mul_Mtt_gtr_400.pdf} \caption{ } \label{fig:results:res:qT:cs:c} \end{subfigure} \\ \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_dphi_Res_Mul_Mtt_le_360.pdf} \caption{ } \label{fig:results:res:dphi:cs:a} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_dphi_Res_Mul_Mtt_360_400.pdf} \caption{ } \label{fig:results:res:dphi:cs:b} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.98\linewidth]{Diags_Res_Mtt_Slice/Diag_pptt_dphi_Res_Mul_Mtt_ge_400.pdf} \caption{ } \label{fig:results:res:dphi:cs:c} \end{subfigure} \caption{ Comparison of the D- and R-prescriptions within the intervals $\Mttbar\le 360\,\text{GeV}$ (left), $\Mttbar\in[360,400]\,\text{GeV}$ (centre), and $\Mttbar\ge 400\,\text{GeV}$ (right). } \label{fig:results:res:qT:dphi:cs} \end{figure} \changed{ It is interesting to analyse our results double-differentially, i.e.\ examining both the \qT\ and \dphittbar\ spectra in three different regions of the \ttbar\ invariant mass \Mttbar, $\Mttbar\le 360\,\text{GeV}$, $\Mttbar\in[360,400]\,\text{GeV}$, and $\Mttbar\ge 400\,\text{GeV}$. We can use these three regions, containing the \ttbar\ production threshold and the Coulomb divergences, a transition region, and the well-separated region where $\dEttbar\sim\order(m_t)$, respectively, to investigate the development of the differences between the D- and R-prescriptions as $\Mttbar$ varies. The \qT\ and \dphittbar\ differential distributions within these intervals are presented in Fig.~\ref{fig:results:res:qT:dphi:cs}, including the \NLLNLO, \NNLLDNNLO, and \NNLLRNNLO\ calculations depicted in the yellow, red, and cyan bands, respectively. As to the last two slices, due to the absence of Coulomb divergences, we also add the results evaluated with the original evolution kernels of Eq.~\eqref{eq:def:Vres:N2LL}, labelled \NNLLNNLO\ and shown as a dark-grey hatched band.% }\footnote{ \changed{It should be noted that the \NLLNLO\ and \NNLLNNLO\ results in Fig.~\ref{fig:results:res:dphi:cs:c} have been published in \cite{Ju:2022wia} and are shown here for comparison.} } \changed{ Fig.~\ref{fig:results:res:qT:cs:c} and Fig.~\ref{fig:results:res:dphi:cs:c} illustrate $\done\sigma_{t\bar{t}}/\done\qT$ and $\done\sigma_{t\bar{t}}/\done\dphittbar$, respectively, for $\Mttbar\ge 400\,\text{GeV}$, where the top and antitop quarks are kinematically well separated and our soft-collinear resummation possesses the best predictivity. It is observed that the central values from \NNLL, \NNLLD, and \NNLLR\ coincide to within a few percent of each other and their uncertainty bands marginally overlap with that calculated at \NLL. This phenomenon confirms our derivation in Sec.~\ref{sec:thr:div:extrap} in that the difference amongst D-prescription, R-prescription and the original evolution kernels in Eq.~\eqref{eq:def:Vres:N2LL} is numerically of \NNLLp\ and beyond for the separated domain and therefore the deviations between them can be well captured by the scale variation in this domain. } \changed{ However, lowering $\Mttbar$ leads to distinct scenarios. As exhibited in Fig.~\ref{fig:results:res:qT:cs:b} and Fig.~\ref{fig:results:res:dphi:cs:b}, although the unmodified \NNLL\ result is still in good agreement with \NNLLD, $50\%$ ($20\%$) deviations are observed in the \NNLLR\ calculation in the low \qT\ (\dphittbar) domains. To interpret this, it merits recalling that \NNLLD\ shifts threshold enhanced terms in part from $\mathbf{V}_h^{[\kappa]}$ of \NNLL\ to higher logarithmic orders, while \NNLLR\ re-exponentiates the leading Coulomb singularities from $\mathbf{V}_h^{[\kappa]}$ on top of \NNLL\ and also embeds the NLO corrections from both $\mathcal{C}^{[\kappa]}_{\alpha;\{h\}}$ and its complex conjugate. Nevertheless, the threshold enhancements generated by $\mathbf{V}_h^{[\kappa]}$ are generally weaker than those from the hard sector in the region $\Mttbar\in[360,400]\,\text{GeV}$. For instance, according to Eq.~\eqref{eq:def:Chard:thr:qqb_qbq_gg:NLO} and Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, $\mathbf{V}_h^{[\kappa]}$ entails the leading Coulomb divergence $\sim\frac{\alpha^2_s}{\beta^2_\ttbar}\left\{\left(\frac{55}{4761}\right)^2,\left(\frac{55}{38088}\right)^2 \right\}$ at \NNLO, whereas the product of $\mathcal{C}^{[\kappa]}_{\alpha;\{h\}}$ and its complex conjugate is $\sim\frac{\alpha^2_s}{\beta^2_\ttbar}\left\{\left(\frac{\pi }{3}\right)^2,\left(\frac{\pi }{24}\right)^2\right\}$. Here the first (second) entry refers to the color-singlet (color octet) contributions of the top-antitop quark pair. Given this numerical hierarchy, the interval $\Mttbar\in[360,400]\,\text{GeV}$ is dominated by enhancements in the hard section and therefore gives rise to non-negligible deviation between \NNLLR\ and \NNLLD\ as well as the unmodified \NNLL. } \changed{ Further decreasing $\Mttbar$ focusses on the threshold regime, as shown in Fig.~\ref{fig:results:res:qT:cs:a} and Fig.~\ref{fig:results:res:dphi:cs:a}, where the discrepancies between \NNLLD\ and \NNLLR\ are observed to be up to $\sim 100\%$ in the low \qT\ realm and $\sim60\%$ in the low \dphittbar\ domain, owing to the growth of threshold enhanced contributions. This phenomenon, together with those in Fig.~\ref{fig:results:res:qT:cs:b} and Fig.~\ref{fig:results:res:dphi:cs:b}, demonstrates the origin of the difference between D- and R-prescriptions observed in Fig.~\ref{fig:results:res:qT:dphi:FullPS}. } % %Fig.~\ref{fig:results:res:qT:dphi:cs} %display the resummation-improved \qT\ and \dphittbar\ differential %distributions in the slices $\Mttbar\le 360\,\text{GeV}$, %$\Mttbar\in[360,400]\,\text{GeV}$, and $\Mttbar\ge 400\,\text{GeV}$. %Therein, we display our results at \NLLNLO, \NNLLDNNLO, and \NNLLRNNLO\ %accuracy. %The \NLLNLO\ results are calculated from a literal implementation %of Eq.~\eqref{eq:methods:res:qT_dphi} since neither the \NLL\ %non-cusp evolution kernel $\mathbf{V}_h^{[\kappa]}$ nor the tree-level %hard functions $\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ induce any %singular behaviour in the limit $\betattbar\to0$, see %Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg} and %Eq.~\eqref{eq:chard:asy:thr:qq:gg}, and thus no modification of the %resummation is required in the threshold regime. %Starting from \NNLL, however, both the evolution kernels and hard %functions introduce threshold divergences in the vicinity of %$\betattbar=0$, see Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg} and %Eq.~\eqref{eq:chard:asy:thr:qq:gg}, driven by the exchange of %Coulomb gluons. %To this end, two radically different prescriptions have been proposed %in Sec.~\ref{sec:thr:div:extrap} that modify the resummation as %$\betattbar\to0$ in the resummation of the %respective observable. %The D-\changed{prescription} was formulated in Eq.~\eqref{eq:LP:res:qqbar:gg:Dec} %and shifts the emerging Coulomb singularities to higher logarithmic %order, whereas the %R-\changed{prescription} of Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp} re-exponentiates %such corrections and embeds them in the \NNLL\ evolution kernel. %The results derived by both methods are displayed as \NNLLDNNLO\ %and \NNLLRNNLO, respectively. % %Examining the \qT\ spectra displayed in Fig.~\ref{fig:results:res:qT:cs}, %we observe that the differential cross sections at either large \qT\ or %large \Mttbar\ increase going from \NLLNLO\ to \NNLLNNLO, in %either \changed{prescription}, in line with the dominating effects from higher-order %corrections (both to the resummation and the fixed-order computation) %in these regions. %The magnitude of this increase, however, is strongly non-uniform, %and ranges from a few percent up to a factor of two. %Conversely, at small \Mttbar\ and small \qT\ there also exist regions %where the cross section in fact decreases as a result of a shift of %the Sudakov peak towards higher \qT\ values when the resummation %accuracy is increased, at least in the R-\changed{prescription}. %Generally, the uncertainties of the calculation are reduced when %including the next order in the perturbative expansion, both %in terms of the coupling parameter and the resummed large logarithms. %Unsurprisingly though, the increased convergence is spoiled %in the threshold regime as \qT\ and \betattbar\ vanish simultaneously. % %Among the \NNLLNNLO\ results, the central values of \NNLLDNNLO\ and %\NNLLRNNLO\ nearly coincide throughout the whole \qT\ range for %$\Mttbar>400\,\text{GeV}$, as do their uncertainties, with small %differences being visible in the resummation region. %When moving to smaller \ttbar\ invariant masses, however, differences %between both \changed{prescription}s develop in the low \qT\ region, culminating as %$\Mttbar\to2m_t$ or $\betattbar\to0$. %To interpret this phenomenon, we recall that D- and R-\changed{prescription} employ %distinct methods to organise the perturbative corrections. %More explicitly, the D-\changed{prescription}, see Eq.~\eqref{eq:LP:res:qqbar:gg:Dec}, %shifts the non-logarithmic components of the product of the evolution %kernel $\mathbf{V}_h^{[\kappa]}$ and the fixed-order functions %$\mathcal{C}^{[\kappa]}_{\alpha,\{h\}}$ to \NNNLL\ and beyond (and %therefore does not include them at \NNLLDNNLO), whereas the R-\changed{prescription}, see %Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}, in part re-exponentiates them %in a dedicated Sudakov factor. %In the absence of any asymptotic behavior in \betattbar, the difference %between the \NNLLDNNLO\ and \NNLLRNNLO\ results is of \NNNLL\ order and %beyond. %Hence, we expect it to leave only small residual effects for %$\Mttbar\ge400\,\text{GeV}$. %Lowering $\betattbar$ towards the threshold regime, however, %non-logarithmic contributions in \qT\ can develop power-like divergences %in $1/\betattbar$, see Eqs.~\eqref{eq:chard:asy:thr:qq:gg} and %Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, introducing non-negligible % corrections (in $1/\betattbar$). %This, in turn, induces an increasing divergence between both \changed{prescription}s, %rendering their difference in the resummation region as large as %that to the formally lower-order \NLLNLO\ computation. % %Analogous reasoning can also be employed to analyse the uncertainty %bands in Fig.~\ref{fig:results:res:qT:cs}. %For instance, in the low \qT\ domain of the $\Mttbar\ge 400\,\text{GeV}$ %region, \NNLLRNNLO\ presents the smallest uncertainty due to the %inclusion of higher-order perturbative contributions partially %compensating scale variations in the Sudakov kernels. %It is well contained by \NNLLDNNLO\ band and marginally overlaps %with the \NLLNLO\ one. %This observation demonstrates the perturbative convergences in the %soft and beam-collinear resummation in this regime. %Our findings change, though, as we move towards smaller \Mttbar\ or %\betattbar, towards the threshold region. %Here, a distinct pattern can be found both in %Fig.~\ref{fig:results:res:qT:cs:a} and %Fig.~\ref{fig:results:res:qT:cs:b} where %formally non-logarithmic products of the resummation kernel and the %hard function that are removed in the D-\changed{prescription} but included in the %R-\changed{prescription} can no longer be ignored. %To be precise, focussing on the asymptotic domain of %Fig.~\ref{fig:results:res:qT:cs:a} and %Fig.~\ref{fig:results:res:qT:cs:b}, we find that even though the %uncertainty bands of \NNLLDNNLO\ and \NNLLRNNLO\ still overlap with those %of the \NLLNLO\ computation, significant deviations manifest themselves %in the limit $\qT\to0$ outside their respective uncertainties. %This observation indicates that the perturbative truncation in line %with the logarithmic counting laws of the soft and beam-collinear %resummation invokes substantial higher order corrections in the %domain $\betattbar\to 0$. %Therefore, to deliver precise predictions in this region, a more %systematic re-collection of the threshold enhancements together with %the soft and beam-collinear radiation is still needed. % % % %The resummation-improved distributions $\done\sigma_\ttbar/\done\dphittbar$ %are shown in Fig.~\ref{fig:results:res:dphi:cs} in the three invariant %mass slices $\Mttbar\le 360\,\text{GeV}$, $\Mttbar\in[360,400]\,\text{GeV}$, %and $\Mttbar\ge 400\,\text{GeV}$. %Again, the \NLLNLO\ result in the slice $\Mttbar\ge 400\,\text{GeV}$ %has already been published in \cite{Ju:2022wia}, which is showcased %here for comparison purposes. %We observe that, at variance with the \qT\ spectra of %Fig.~\ref{fig:results:res:qT:cs} where Sudakov peaks are formed in %the asymptotic domain, the \dphittbar\ spectra grow monotonically %as $\dphittbar\to0$. %To understand this structural difference, we remind the reader that %while both the \qT\ and \dphittbar\ resummations comprise the same %partonic kernels in Eqs.~\eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}, %as well as modifications in the D- and R-\changed{prescription}, see %Eq.~\eqref{eq:LP:res:qqbar:gg:Dec} and %Eq.~\eqref{eq:LP:res:qqbar:gg:Reexp}, %which approach constants as \qT\ and \dphittbar\ vanish, %the calculation of the spectra, see Eq.~\eqref{eq:methods:res:qT_dphi}, %invokes an additional kinematic suppression $\propto\qT$ in the \qT\ %spectrum which is absent in the \dphittbar\ case. %In consequence, the \qT\ spectrum develops a Sudakov peak in the vicinity %of $\qT=0$, whereas the \dphittbar\ spectrum does not. %Furthermore, in Fig.~\ref{fig:results:res:dphi:cs} we again compare %our results at \NLLNLO\ and \NNLLNNLO\ accuracy, the latter again both %in the D- and the R-\changed{prescription}. %Akin to the scenario in Fig.~\ref{fig:results:res:qT:cs}, we also %observe perturbative convergence of the resummation in the interval %$\Mttbar\ge 400\,\text{GeV}$ with the increase in the logarithmic %accuracy. %Reducing \Mttbar, as before, leads to a gradual corruption through %the threshold singular terms as $\betattbar\to0$. %This echoes the necessity to re-collect the threshold enhancements %during the soft and beam-collinear resummation for this spectrum %as well, especially when the domain $\dphittbar\to0$ and $\betattbar\to0$ %is of concern. \section{Numerical results of hard-scale evolution kernel} \label{app:vali:Vthr} In this appendix we deliver a numerical comparison amongst the original non-cusp evolution kernel in Eqs.~\eqsref{eq:def:Vres:NLL}{eq:def:Vres:N2LL} as proposed in~\cite{Buras:1991jm,Buchalla:1995vs}, the leading singular approximation from Eqs.~\eqsref{eq:def:Vres:NLL:thr:qq_gg}{eq:def:Vres:N2LL:thr:qq_gg}, and the expansion of the re-exponentiated kernel in Eq.~\eqref{eq:def:Vres:N2LL:Reexp:exp}. During our computation, we fix $\mu_h=M_{\ttbar}$ and $\mu_s=1\,\text{GeV}$ as well as the scattering angle of the top quark $\theta_t={\pi}/{3}$. \begin{figure}[t!] \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudNLLp_qqbar_1_LP.pdf} \caption{ } \label{fig:Suk:Exp:qqbar1:lp:nll} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudNLLp_qbarq_1_LP.pdf} \caption{ } \label{fig:Suk:Exp:qbarq1:lp:nll} \end{subfigure} \\ \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudNLLp_gg_1a_LP.pdf} \caption{ } \label{fig:Suk:Exp:gg1a:lp:nll} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudNLLp_gg_1b_LP.pdf} \caption{ } \label{fig:Suk:Exp:gg1b:lp:nll} \end{subfigure} \caption{ Comparison of the non-cusp evolution kernel $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:NLL} and its leading terms $\mathbf{V}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg} in the threshold regime at \NLL. Therein, $|\mathbf{V}_{h,(\mathrm{thr})}^{(m,n)}|$ denotes the absolute value of the entry of $\mathbf{V}_{h,(\mathrm{thr})}$ in the $m$-th row and $n$-th column from respective partonic process. } \label{fig:Suk:Exp:lp:nll} \end{figure} Fig.~\ref{fig:Suk:Exp:lp:nll} exhibits the \NLL\ results of $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:NLL} and $\mathbf{V}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg} in solid and dashed lines, respectively. Therein, the dependence of all the entries of $\mathbf{V}_h$ is displayed with respect to $\betattbar$. For $\mathbf{V}_{h,\mathrm{thr}}$, we show the non-zero components only. Due to the facts that the leading threshold enhanced terms in the \NLO\ anomalous dimension only manifest themselves in the imaginary parts and that the complete Coulomb singular behaviour has been exponentiated at \NLL\ in both Eq.~\eqref{eq:def:Vres:NLL} and Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg}, the \NLL\ kernel illustrated in Fig.~\ref{fig:Suk:Exp:lp:nll} invokes no divergence as $\betattbar\to0$. Comparing $\mathbf{V}_h$ with $\mathbf{V}_{h,\mathrm{thr}}$, we find that the leading approximation is capable of replicating the correct asymptotic behaviour of all the diagonal entries of $\mathbf{V}_h$, while the non-diagonal elements of $\mathbf{V}_h$ become progressive smaller in the low $\betattbar$ region. This indicates the non-diagonal entries of $\mathbf{V}_h$ are all power suppressed in magnitude and it is thus in agreement with the absence of the off-diagonal contributions in $\mathbf{V}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg}. \begin{figure}[t!] \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudNLLp_qqbar_2_LP.pdf} \caption{ } \label{fig:Suk:Exp:qqbar2:lp:nll:ratio} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudNLLp_qbarq_2_LP.pdf} \caption{ } \label{fig:Suk:Exp:qbarq2:lp:nll:ratio} \end{subfigure} \\ \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudNLLp_gg_2_LP.pdf} \caption{ } \label{fig:Suk:Exp:gg2:lp:nll:ratio} \end{subfigure} \caption{ Product of the non-cusp evolution $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:NLL} and the inverse matrix $\mathbf{V}^{-1}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg} at \NLL. Therein, $|[\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h]_{m,n}|$ denotes the absolute value of the entry of $(\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h)$ in the $m$-th row and $n$-th column from respective partonic process. } \label{fig:Suk:Exp:lp:nll:ratio} \end{figure} In a bid to scrutinise our leading approximation in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg} further, we plot the result of the product $(\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h)$ in Fig.~\ref{fig:Suk:Exp:lp:nll:ratio}. We observe that $(\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h)$ approaches the unity matrix for all three partonic processes of interest. This phenomenon shows that $\mathbf{V}^{-1}_{h,\mathrm{thr}}$ is able to serve as a qualified inverse matrix of $\mathbf{V}_h$ in the vicinity of $\betattbar=0$. Further, it details that the approximation in Eq.~\eqref{eq:def:Vres:NLL:thr:qq_gg} indeed manages to reproduce the leading asymptotic behaviour of Eq.~\eqref{eq:def:Vres:NLL}. \begin{figure}[t!] \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qqbar_1_LP.pdf} \caption{ } \label{fig:Suk:Exp:qqbar1:lp:n2ll} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qbarq_1_LP.pdf} \caption{ } \label{fig:Suk:Exp:qbarq1:lp:n2ll} \end{subfigure} \\ \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_gg_1a_LP.pdf} \caption{ } \label{fig:Suk:Exp:gg1a:lp:n2ll} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_gg_1b_LP.pdf} \caption{ } \label{fig:Suk:Exp:gg1b:lp:n2ll} \end{subfigure} \caption{ Comparison of the non-cusp evolution $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:N2LL} and its leading terms $\mathbf{V}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg} in the threshold regime at \NNLL. Therein, $|\mathbf{V}_{h,(\mathrm{thr})}^{(m,n)}|$ denotes the absolute value of the entry of $\mathbf{V}_{h,(\mathrm{thr})}$ in the $m$-th row and $n$-th column from respective partonic process. } \label{fig:Suk:Exp:lp:n2ll} \end{figure} \begin{figure}[t!] \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qqbar_2_LP.pdf} \caption{ } \label{fig:Suk:Exp:qqbar2:lp:n2ll:ratio} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qbarq_2_LP.pdf} \caption{ } \label{fig:Suk:Exp:qbarq2:lp:n2ll:ratio} \end{subfigure} \\ \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_gg_2_LP.pdf} \caption{ . } \label{fig:Suk:Exp:gg2:lp:n2ll:ratio} \end{subfigure} \caption{ Product of the non-cusp evolution $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:N2LL} and the inverse matrix $\mathbf{V}^{-1}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg} at \NNLL. Therein, $|[\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h]_{m,n}|$ denotes the absolute value of the entry of $(\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h)$ in the $m$-th row and $n$-th column from respective partonic process. } \label{fig:Suk:Exp:lp:n2ll:ratio} \end{figure} In Figs.~\ref{fig:Suk:Exp:lp:n2ll} we confront $\mathbf{V}_h$ of Eq.~\eqref{eq:def:Vres:N2LL} with $\mathbf{V}_{h,\mathrm{thr}}$ of Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg} at \NNLL. At variance with the findings of Figs.~\ref{fig:Suk:Exp:lp:nll} and \ref{fig:Suk:Exp:lp:nll:ratio}, the diagonal entries of $\mathbf{V}_h$ develop divergent behaviour in the threshold domain, as a result of the Coulomb singularity residing in Eq.~\eqref{eq:Jh:thr:exp:qq_gg}, which $\mathbf{V}_{h,\mathrm{thr}}$ is able to replicate at \NNLL. Further, differing from $\mathbf{V}_h$ at \NLL, where all the non-diagonal entries in Fig.~\ref{fig:Suk:Exp:lp:nll} generally decline in magnitude as \betattbar\ reduces, the non-diagonal constituents in Fig.~\ref{fig:Suk:Exp:lp:n2ll} can experience enhancements in the threshold domain, such as $|\mathbf{V}_h^{(3,2)}|$ in Fig.~\ref{fig:Suk:Exp:gg1b:lp:n2ll}. The reason for this phenomenon is that in the expression of Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, only the leading singular terms of Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, which are of $\mathcal{O}(\betattbar^{-2})$, have been taken into account. Divergence of $\mathcal{O}(\betattbar^{-1})$ are, however, still possible. To verify that there is no stronger divergent behaviour in non-diagonal elements other than that of Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, we present the results of $(\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h)$ in Fig.~\ref{fig:Suk:Exp:lp:n2ll:ratio}. It is found that all but the diagonal elements are reduced substantially as $\betattbar\to0$, while all the diagonal elements of the product $(\mathbf{V}^{-1}_{h,\mathrm{thr}}\mathbf{V}_h)$ approach unity. This unambiguously shows that our leading approximation in Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg} can describe the asymptotic behaviour of Eq.~\eqref{eq:def:Vres:N2LL} at \NNLL\ as well. \begin{figure}[t!] \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qqbar_1.pdf} \caption{ } \label{fig:Suk:Exp:qqbar1:n2ll} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qbarq_1.pdf} \caption{ } \label{fig:Suk:Exp:qbarq1:n2ll} \end{subfigure} \\ \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_gg_1a.pdf} \caption{ } \label{fig:Suk:Exp:gg1a:n2ll} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_gg_1b.pdf} \caption{ } \label{fig:Suk:Exp:gg1b:n2ll} \end{subfigure} \caption{ Comparison of the non-cusp evolution $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:N2LL} and $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}$ in Eq.~\eqref{eq:def:Vres:N2LL:Reexp:exp} at \NNLL. Therein, $|\mathbf{V}_{h}^{(m,n)}|$ and $|\widetilde{\mathbf{V}}_{h,\mathrm{exp}}^{(m,n)}|$ denote the absolute values of the entries of $\mathbf{V}_h$ and $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}$ in the $m$-th row and $n$-th column, respectively. } \label{fig:Suk:Exp:n2ll} \end{figure} \begin{figure}[t!] \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qqbar_2.pdf} \caption{ .} \label{fig:Suk:Exp:qqbar2:n2ll:ratio} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_qbarq_2.pdf} \caption{ . } \label{fig:Suk:Exp:qbarq2:n2ll:ratio} \end{subfigure} \\ \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.9\linewidth, height=0.6\linewidth]{Diag_Evo_Hard/Diag_SudN2LLp_gg_2.pdf} \caption{ .} \label{fig:Suk:Exp:gg2:n2ll:ratio} \end{subfigure} \caption{ Product of the non-cusp evolution $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:N2LL} and the inverse matrix $\widetilde{\mathbf{V}}^{-1}_{h,\mathrm{exp}}$ in Eq.~\eqref{eq:def:Vres:N2LL:Reexp:exp} at \NNLL. Therein, $|[\widetilde{\mathbf{V}}^{-1}_{h,\mathrm{exp}}\mathbf{V}_h]_{m,n}|$ denotes the absolute value of the entry of $(\widetilde{\mathbf{V}}^{-1}_{h,\mathrm{exp}}\mathbf{V}_h)$ in the $m$-th row and $n$-th column from respective partonic process. } \label{fig:Suk:Exp:n2ll:ratio} \end{figure} Eventually, Figs.~\ref{fig:Suk:Exp:n2ll} and \ref{fig:Suk:Exp:n2ll:ratio} depict the results of $\mathbf{V}_h$ of Eq.~\eqref{eq:def:Vres:N2LL} and $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}$ in Eq.~\eqref{eq:def:Vres:N2LL:Reexp:exp} at \NNLL, the expansion of the re-exponentiated Sudakov factor. Owing to the fact that in comparison with the leading singular result of $\mathbf{V}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg}, $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}$ is embedded with more power corrections, the agreement between $\mathbf{V}_h$ and $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}$ is considerably improved compared to Figs.~\ref{fig:Suk:Exp:lp:n2ll} and \ref{fig:Suk:Exp:lp:n2ll:ratio}. For instance, focussing on the quark-induced process, while in Fig.~\ref{fig:Suk:Exp:qqbar2:lp:n2ll:ratio}, the deviation between the leading approximation $\mathbf{V}_{h,\mathrm{thr}}$ in Eq.~\eqref{eq:def:Vres:N2LL:thr:qq_gg} and $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:N2LL} rapidly surges above $\betattbar\sim 10^{-3}$, in Fig.~\ref{fig:Suk:Exp:qqbar2:n2ll:ratio}, numerical agreement of $\mathbf{V}_h$ and $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}$ holds up to $\betattbar\sim 10^{-1}$ within around $10\%$. In light of this excellent agreement, in matching the re-exponentiated Sudakov factor onto $\mathbf{V}_h$ in Eq.~\eqref{eq:def:Vres:N2LL:Reexp}, we choose the matching parameters $c^{\mathrm{def}}_{\rm{thr}}=0.4$ and $ r^{\mathrm{def}}_{\mathrm{thr}}=0.1$ as defined in Eq.~\eqref{eq:scale:ftran:beta_TT}. In this way, the re-exponentiation impact is fully switched on in the domain $\betattbar\le0.3$ but then gets gradually faded out until the total shutdown at $\betattbar=0.5$. This choice of this active range brings the difference between $\mathbf{V}_h$ and $\widetilde{\mathbf{V}}_{h,\mathrm{exp}}$ under control, i.e.\ generally below $40\%$ for all three partonic channels, and also steers clear of the tail region in Fig.~\ref{fig:Suk:Exp:n2ll:ratio} where the power correction to the small \betattbar\ expansion escalates dramatically. \section{\changed{Definitions of the color and helicity bases}} \label{app:def:col:spin} \changed{ Here we present the colour bases \cite{Beneke:2009rj} used in calculating $\mathcal{C}_{\alpha;\{h\}}^{[\kappa]}$ and $\mathcal{S}^{\alpha\beta}_{[\kappa]}$ in Eqs.\ \eqsref{eq:LP:res:qqbar}{eq:LP:res:gg}, \begin{equation}\label{eq:def:color:basis:qq_gg} \begin{split} c^{qq,(1)}_{a_1a_2a_3a_4} &= \frac{1}{3}\,\delta_{a_1a_2}\delta_{a_3a_4}\,,\;\; c^{qq,(2)}_{a_1a_2a_3a_4} = \frac{1}{\sqrt{2}}\sum_c T^{c}_{a_1a_2}T^{c}_{a_3a_4}\,,\\ c^{gg,(1)}_{a_1a_2a_3a_4} &= \frac{1}{2\sqrt{6}}\,\delta_{a_1a_2}\delta_{a_3a_4}\,,\;\; c^{gg,(2)}_{a_1a_2a_3a_4} = \frac{i}{2\sqrt{3}}\,\sum_c f^{a_1 c a_2}T^{c}_{a_3a_4}\,,\;\; c^{gg,(3)}_{a_1a_2a_3a_4} = \frac{1}{2}\sqrt{\frac{3}{5}}\sum_cd^{a_1 c a_2}T^{c}_{a_3a_4}\,, \end{split} \end{equation} where $T^{c}_{ab}$ stands for the generator in the fundamental representation of the SU$(3)$ group. $f_{abc}$ and $d_{abc}$ mark the antisymmetric and symmetric structure constants for the SU$(3)$ group, respectively. } \changed{We also specify the helicity bases concerned by the gluon-initialised channel \cite{Actis:2012qn,Actis:2016mpe}, \begin{align} \label{eq:Bgg:def:hel:space} \epsilon^{\mu}_{n,\pm}\equiv \left\{0, \frac{\mp1}{\sqrt{2}},\frac{-\mathrm{i}}{\sqrt{2}},0\right\}\,, \qquad \epsilon^{\mu}_{\nbar,\pm}\equiv \left\{0, \frac{\pm1}{\sqrt{2}},\frac{-\mathrm{i}}{\sqrt{2}},0\right\}\,. \end{align} } \clearpage
